Efficient Multiparty Interactive Coding for Insertions, Deletions and Substitutions

In the field of interactive coding, two or more parties wish to carry out a distributed computation over a communication network that may be noisy. The ultimate goal is to develop efficient coding schemes that can tolerate a high level of noise while increasing the communication by only a constant factor (i.e., constant rate). In this work we consider synchronous communication networks over an arbitrary topology, in the powerful adversarial insertion-deletion noise model. Namely, the noisy channel may adversarially alter the content of any transmitted symbol, as well as completely remove a transmitted symbol or inject a new symbol into the channel. We provide efficient, constant rate schemes that successfully conduct any computation with high probability as long as the adversary corrupts at most $\varepsilon /m$ fraction of the total communication, where $m$ is the number of links in the network and $\varepsilon$ is a small constant. This scheme assumes the parties share a random string to which the adversarial noise is oblivious. We can remove this assumption at the price of being resilient to $\varepsilon / (m\log m)$ adversarial error. While previous work considered the insertion-deletion noise model in the two-party setting, to the best of our knowledge, our scheme is the first multiparty scheme that is resilient to insertions and deletions. Furthermore, our scheme is the first computationally efficient scheme in the multiparty setting that is resilient to adversarial noise.

==> abstract-II.tex <==
%


\begin{abstract}
Interactive coding allows two or more parties 
to carry out a distributed computation
over a communication network that may be noisy.
The ultimate goal is to develop efficient coding schemes that tolerate a high
level of noise while increasing the communication by only a constant factor (i.e., constant rate).

In this work (the second part) we provide computationally efficient, constant rate schemes that conduct any computation on arbitrary networks, and succeed with high probability in the presence of adversarial noise that can
insert, delete, or alter communicated messages. 
Our schemes are non-fully-utilized and incur a polynomial (in the size of the network) blowup in the round complexity.

Our first scheme resists an oblivious adversary that 
corrupts at most a fraction $\frac{\eps}{m}$ of the total communication,
where $m$ is the number of links in the network and $\eps$ is a small constant.
In contrast to the first part of this work, the scheme in this part does not assume that the parties pre-share a long random string.


Our second scheme resists \emph{an arbitrary} (non-oblivious) adversary
that corrupts at most a fraction $\frac{\eps}{m\log m}$ of the communication.
We further improve the resilience to $\frac{\eps}{m\log\log m}$ by assuming the parties pre-share
a long common random string.
\end{abstract}




==> hashes.tex <==
%
\subsection{Hash functions, $\delta$-biased strings}



We use a standard inner-product based hash function. The hash function is seeded with a (usually random) string $S$ such that each bit of the output is an inner product between the input and a certain part of $S$ (using independent parts of $S$ for different output bits). Formally,
%
%
%
%
\gnote{Add concatenated length to Def 2.3, with seed length $2\tauL$. Then footnote saying that we add the length implicitly in our protocol (by sending chunk number and fixed communication pattern).}
\begin{definition}[Inner Product Hash Function]
\label{def:ip-hash}
The inner product hash function 
$h: \{0,1\}^* \times \{0,1\}^* \to \{0,1\}^\tau$ 
is defined for any input $x$ of length $|x|=L$ and seed~$s$ of length $|s|=\tau L$, as the concatenation
of $\tau$ inner products between~$x$ and disjoint parts of~$s$, namely,
\[
 h(x,s) = \langle x, s[1,L] \rangle \circ \cdots \circ  \langle x, s[(\tau-1)L+1,\tau L] \rangle.
\]
We use the shorthand $h_s(x) \eqdef h(x,s)$.
\end{definition}
We sometimes abuse notation and hash a ternary-string $x$ (or a string over a larger alphabet). In this case, assume we first convert $x$ into a binary string in the natural manner (each symbol separately, using $\lceil \log_2 3\rceil =2$ bits) and then hash the binary string. The seed length should increase appropriately (by at most a constant).

The following is a trivial property of the inner product hash function, stating that, given a uniform seed, the output is also uniformly distributed.
\begin{lemma}\label{lem:unifHash}
For any $x\ne 0$, and $r\in\{0,1\}^\tau$
\[
\Pr_{s\sim \Unif} [ h_s(x) = r] = 2^{-\tau}.
\]
\end{lemma}
It is easy to see Lemma~\ref{lem:unifHash} also implies that the collision probability of the inner product hash function with output length $\tau$ is exactly $2^{-\tau}$, since given two strings $x$ and $y$ such that $x \neq y$, the Lemma implies that the probability that $\Pr_{s\sim \Unif} [ h_s(x-y) = \vec{0}] = 2^{-\tau}$.


%
%
%
%


Usually, the hash function is seeded with a uniform string. In order to reduce the amount of randomness needed, we use $\delta$-biased random strings, which are close enough to uniform (for our needs), yet can be constructed from much shorter (uniform) seeds, via a result by Naor and Naor~\cite{NN93}.
\begin{definition}[$\delta$-bias]
\label{def:delta-bias}
Fix $\delta > 0$. A distribution $D$ over $\F_2^n$ is $\delta$-biased if for any $v \in \F_2^n \setminus \{ 0^n\}$, we have that
\[ 
\left| \Pr_{x \sim D}\left[ \sum\limits_{i=1}^{n} v_i x_i = 0 \right] - 1/2 \right| \leq \delta.
\]
\end{definition}
%
%

\begin{lemma}[\cite{NN93,AGHP92}]
\label{lem:delta-bias}
There is a constant $c \in \N$ and an efficiently computable function $G: \{ 0,1\}^* \to \{ 0,1\}^*$ such that the following holds. Fix $\eps > 0$. For any size $k$ and a uniformly random string $S \in \{ 0,1\}^{c\cdot (k+\log(1/\eps))}$, we have that $G(S) \in \{ 0,1\}^{2^k}$ is a $2\eps$-biased distribution over bit strings of length of $2^k$.
\end{lemma}
%
%
%
%
%
%
%
%
%


Finally, we appeal to the following Lemma from~\cite{haeupler14} (which is in turn based on \cite{NN93}) that connects the behaviour of hash function seeded with $\delta$-biased string to hashes seeded with uniformly random string \emph{as long as their input is fixed and independent of the seed}.
\begin{lemma}[Lemma 6.3 from~\cite{haeupler14}]
\label{lem:hashes-delta-bias}
Fix positive integers $k, \tau$, and $L$. Consider $k$ pairs of binary strings $(x_1, y_1), \ldots (x_k, y_k)$ where each string has length at most $L$. Let $\{ h_{Q}\}_{Q \in \{ 0,1\}^{2\tau L}}$ be an inner product hash family with input length $\leq L$, output length $\tau$, and seed length $2\tau L$. Let $S=(s^{(1)}, \ldots, s^{(k)})$ be a random seed of length $k \cdot 2\tau L$.
\begin{enumerate}
\item If $S$ is drawn from a uniform distribution over $\{ 0,1\}^{2\tau L \cdot k}$, then for each $i \in [k]$,
\[
\Pr_{s^{(i)}}[h_{s^{(i)}}(x_i) = h_{s^{(i)}}(y_i)] = 2^{-\tau}
\]
if $x_i \neq y_i$. Note that, trivially, $\Pr_{s^{(i)}}[h_{s^{(i)}}(x_i) = h_{s^{(i)}}(y_i)] = 1$ when $x_i = y_i$. Furthermore, for each $i \in [k]$ the events of hash collisions are independent.
\item If $S$ is drawn from a $\delta$-biased distribution over $\{ 0,1\}^{2\tau L \cdot k}$, then it holds that the distribution
\[ \left( \mathsf{1}_{h_{s^{(1)}}(x_1) = h_{s^{(1)}}(y_1)}, \ldots,  \mathsf{1}_{h_{s^{(k)}}(x_k) = h_{s^{(k)}}(y_k)} \right) \]
is $\delta$-close to the case where $S$ is uniformly random.
\end{enumerate}
\end{lemma}

Recall that $\delta$-closeness means that the statistical difference between two distributions is bounded by~$\delta$.
\begin{definition}[$\delta$-closeness]\label{def:tvd}
We say that distributions $P,Q$ over the probability space~$\Omega$ are $\delta$-close if
\[
\sup_{A\subseteq \Omega} |P(A)-Q(A)|\le \delta.
\]
The above is equivalent to having 
\(
\frac12 \sum_{\omega \in \Omega} \left\vert {P(\omega) -Q(\omega)} \right \vert \le  \delta.
\)
\end{definition}

Note that as a corollary of Lemma~\ref{lem:hashes-delta-bias}, by setting $k$ to 1, $\tau$ to a constant, and using $\delta$-biased randomness with $\delta = 2^{-\tau}$, we can get the hash functions with seed length that is logarithmic in the size of their input, 
by seeding the inner product hash function with $\delta$-biased seeds. This corollary was noted in previous work, e.g. in Naor and Naor~\cite{NN93}.

\begin{corollary}
\label{cor:good-hash} 
There is a hash function family  $\{ h_{Q}\}_{Q \in \{ 0,1\}^{s}}$ with input length $\leq L$, output length~$\tau$, and seed length $s = \Theta(\log L + \tau)$ such that, given any pair of inputs $x$ and $y$ such $x \neq y$, we have that
\[ \Pr_Q[h_Q(x) = h_Q(y)] \leq 2 \cdot 2^{-\tau}\]
\end{corollary}


==> introduction-ii.tex <==
%

\section{Introduction}
\IEEEPARstart{In}{}{} his pioneering work, Schulman~\cite{schulman92,schulman96} introduced and studied the problem of how to perform an interactive two-party computation over a noisy communication
channel. 
Plenty of follow-up work appeared in the recent couple of decades
extending Schulman's work in the two-party setting to a variety of noise and communication models (see~\cite{gelles17} for a survey of these results).
%
In \cite{RS94}, Rajagopalan and Schulman considered interactive coding over 
a network of~$n$ parties that wish to compute some function of their private inputs
by communicating over a 
\emph{noisy} network of arbitrary topology.
The work of~\cite{RS94} shows that if each communication channel
is the binary symmetric channel (BSC$_\eps$) 
that flips every bit with some constant probability~$\eps<1/2$, 
then there exists a \emph{coding scheme}
that takes any protocol $\Pi$ (that assumes noiseless communication), and converts it into
a resilient protocol that computes the same function over the noisy network. 

A coding scheme is measured by its \emph{rate}: the ratio between the amount of communication in the noiseless version of the protocol and
the amount of communication in the resilient protocol. The coding scheme is more efficient (communication-wise) the closer the rate gets to~1. In particular, when the rate remains bounded away from~0 the coding scheme is said to be of \emph{constant rate}. 
The rate of the coding scheme in~\cite{RS94} is given by $O(1/\log (d+1))$ where $d$ is the maximal degree in the network. That is, the rate depends on the network's topology and it decreases as the maximal degree increases. A constant rate is obtained whenever the maximal degree is constant,~$d=O(1)$.
Later, Alon et al.~\cite{ABEGH19} developed coding schemes with a constant rate over a clique and dense $d$-regular networks with $d=n^{\Omega(1)}$ assuming BSC$_\eps$ channels. 
Their result proved that constant rate coding is possible also when the degree is super-constant. Yet, Braverman et al.~\cite{BEGH18} proved that a rate of $\Theta(1/\log n)$ is tight for coding over certain some topologies, e.g., a star. All of these works are in the \emph{fully utilized} model, in which every party sends a single bit to all its neighbors in each round.

Jain et~al.~\cite{JKL15} and Hoza and Schulman~\cite{HS16} developed coding schemes that can deal with a stronger type of noise than the BSC$_\eps$ channel, namely, \emph{adversarial} noise that can corrupt up to a fraction $\eps/n$ of the communication using substitution errors, for a small constant $\eps$. Both these works are computationally inefficient.
%
While \cite{HS16}, like previous work, assumes the fully utilized
model,~\cite{JKL15} uses a non-fully-utilized setting, in which parties may or may not speak in a given round. This is the model of choice in distributed algorithms and cryptography. However,~\cite{JKL15} only works when the network topology is a star.
%


In the first part of this work~\cite{GKR-1}, we developed a coding scheme for \emph{arbitrary} networks that is resilient to a stronger type of adversarial noise than flipping bits, namely, insertion and deletion noise. In addition, unlike previous schemes that consider adversarial error~\cite{JKL15, HS16}, our scheme is \emph{computationally efficient}. Furthermore, it features a constant rate and it is resilient to $\eps / m$ fraction of adversarial errors for a small constant $\eps$, where $m$ is the number of edges in the communication graph.
%
The communication model is the general (non-fully-utilized) model where parties are allowed to either send a bit or remain silent at every round. This holds for both the coding scheme and the underlying noiseless protocol, however, we additionally assume that the order of speaking in the underlying protocol is pre-determined (which was also assumed by~\cite{JKL15}).

The scheme in~\cite{GKR-1} makes two restrictive assumptions that simplify the task of coding over noisy channels. 
The first assumption is that the parties are allowed to pre-share a long common random string (CRS). The second assumption is that this CRS is unknown to the adversary;
in other words, the adversary is assumed to be \emph{oblivious}; in particular, this critically implies that the noise is independent of this CRS. 
In this work we eliminate both these assumptions: our protocol does not require a CRS and works against general adversaries.


\subsection{Our Contributions and Comparison to Previous Work}
We design coding schemes for adversarial errors in the same communication model as~\cite{JKL15,GKR-1}; namely, where parties may or may not speak in a given round, and the underlying protocol is only assumed to have a fixed speaking order, which is assumed by all known schemes in the non-fully-utilized setting. As in \cite{GKR-1}, our coding schemes are for networks with an arbitrary topology, are computationally efficient, and feature a constant rate (i.e., a constant multiplicative blowup in communication). 
Our schemes are randomized, however they \emph{do not} assume the parties pre-share any randomness. 
The schemes succeed with high probability assuming an all-powerful adversary that may insert, delete, and substitute bits up to a restricted fraction of the communication.


Our first coding scheme (\AlgCRS) achieves a constant rate, and is resilient to $\eps / m$-fraction~of adversarial insertion, deletion, and substitution noise.
This scheme assumes a limited type of noise, i.e., an \emph{oblivious adversary} whose corruptions are predetermined and are independent of the parties' randomness.
In our second coding scheme (\AlgNO), we 
remove the restriction of the obliviousness of the adversary, at the price of being resilient to $\eps / (m\log m)$-fraction of errors. 

Finally, if we remove only the assumption that the adversary is oblivious, but retain the assumption that 
the parties pre-share a long random string, then we obtain a scheme that is resilient 
%
to a higher level of noise, namely, 
to $\eps/ m \log\log m$-fraction of insertion and deletion errors (\AlgImpNO). 
See Table~\ref{tbl:comparison} for a comparison of our new results 
%
(Algorithms A, B, and C)
with the state of the art. See \cite{GKR-1} for further discussion on related work.

\begin{table*}[thb]
\caption{Interactive coding schemes in the multiparty setting}
\label{tbl:comparison}
\center
\begin{minipage}{0.8\linewidth}
\setlength\extrarowheight{1.2pt}     
\begin{tabular}{cccccc}
\textbf{scheme} & \textbf{topology} & \textbf{noise level} & \textbf{noise type} & \textbf{rate} & \textbf{efficient} \\
\hline\hline
RS94+GMS14~\cite{RS94,GMS14} & arbitrary & \multicolumn{2}{c}{BSC$_\eps$}  & $1/O(\log (d+1))$ & Yes  \\
ABEGH19~\cite{ABEGH19} & clique & \multicolumn{2}{c}{BSC$_\eps$}  & $\Theta(1)$ & Yes \\
\hline
HS16~\cite{HS16} & arbitrary & $O(1/m)$ & substitution & $\Theta(1)$ & \\
HS16~\cite{HS16} & arbitrary & $O(1/n)$ &substitution & $1/O(m\log (n) / n)$ & \\
JKL15~\cite{JKL15} & star & $O(1/m)$ & substitution\strut & $\Theta(1)$ &  \\
\AlgCRS &  arbitrary & $O(1/m)$ & \parbox[c]{3cm}{\strut\centering\emph{oblivious} insertions\\[-0.65ex] and deletions\strut} & $\Theta(1)$ & Yes \\
\AlgNO & arbitrary & $O(1/m\log m)$ & \parbox[c]{3cm}{\centering insertions and\\[-0.65ex] deletions\strut}\strut & $\Theta(1)$ & Yes \\
\hline\hline
\hspace{-4pt}{\parbox{2.6cm}{\footnotesize pre-shared \\[-3pt] randomness:}}~~\\
\Tstrut\AlgImpNO  & arbitrary & $O(1/m\log\log m)$ & \parbox[c]{3cm}{\centering insertions and\\[-0.65ex] deletions\strut} & $\Theta(1)$ & Yes \\
\hline
\end{tabular}
\footnotetext{The first four schemes are in the \emph{fully-utilized} model (each channel must be utilized in every round), while~\cite{JKL15} and all algorithms in this paper are in the non-fully-utilized model. Recall that $n$ is the number of parties, $m$ is the number of (bi-directional) communication links in the network, and $d$ is the maximal degree of a node in the network}
\end{minipage}
\end{table*}



%



More formally, our result is two-fold. First, we assume that the adversary is oblivious, i.e., the noise is predetermined and is independent of the randomness used by the parties.

\begin{theorem}[Oblivious noise, informal]\label{thm:main}
Let $G=(V,E)$ be an arbitrary synchronous network with $n=|V|$ nodes and $m=|E|$ links.
For any noiseless protocol $\Pi$ over~$G$ with a predetermined order of speaking, 
and for a sufficiently small constant $\eps$,
there exists a computationally efficient coding scheme that simulates $\Pi$
over a noisy network $G$.  The simulated protocol is robust to adversarial insertion, deletion, and substitution noise, assuming at most  $\eps / m$-fraction of the communication is corrupted. The simulated protocol communicates $O(\CC(\Pi))$ bits, takes $O(m\RC(\Pi))$ rounds, and succeeds with probability at least $1-\exp(-\CC(\Pi) /m)$, assuming the noise is oblivious.
\end{theorem}



Next, we remove the restriction to oblivious noise.  Namely, we consider adversaries that may adaptively decide which transmissions to corrupt according to the observed transcript, as well as the parties inputs (however, the noise is unaware of any private coin-tossing a party may perform later in the protocol).
In this case we still obtain an efficient coding scheme with a constant rate, albeit, with slightly smaller noise resilience.
\begin{theorem}[Non-oblivious noise, informal]\label{thm:main2}
Let $G=(V,E)$ be an arbitrary synchronous network with $n=|V|$ nodes and $m=|E|$ links.
For any noiseless protocol $\Pi$ over~$G$ with a predetermined order of speaking, and for a sufficiently small constant $\eps$,
there exists a computationally efficient coding scheme that simulates $\Pi$
over a noisy network $G$.  The simulated protocol is robust to adversarial insertion, deletion, and substituition noise, assuming at most  $(\eps / m\log m)$-fraction of the communication is corrupted. The simulated protocol communicates $O(\CC(\Pi))$ bits, takes $O(m\log m \cdot \RC(\Pi))$ rounds, and succeeds with probability at least $1-\exp(-\CC(\Pi) /m)$.
\end{theorem}




In Appendix~\ref{sec:nonobliv-crs} we consider the case where the adversarial channel is non-oblivious, however, the parties pre-share a long random string. In this case we show a coding scheme (\AlgImpNO) that is resilient to a somewhat higher noise level of $\eps / m\log\log m$-fraction of insertion and deletion noise, while still incurring a constant blowup in the communication. See Appendix~\ref{sec:nonobliv-crs} for the complete details.



We note that, while our schemes feature a constant blowup in their communication rate, the blowup in their round complexity may be up to $O(m\log m)$; furthermore, in all our schemes the round complexity will \emph{not} depend on the noise, and is fixed at the beginning of the scheme. We also note that if there is no bound on the blowup in round complexity, trivial coding schemes exist, e.g., by encoding the input $x\in\{0,1\}^*$ as a single message sent at round~$x$.
%


\subsection{Overview of our Techniques}
\label{sec:overview-intro}
\paragraph{Overview of~\cite{GKR-1}}
Our starting point is the coding scheme presented in~\cite{GKR-1}. 
The scheme works in \emph{iterations}, where every iteration takes the same number of rounds, and approximately the same amount of communication, of $\Theta(m)$ bits. Each iteration consists of the following four phases:
(i) consistency check, (ii) flag passing, (iii) simulation, and (iv) rewind. In phase (i) each pair of parties $u,v$ checks whether or not they agree on the partial transcript communicated on the link~$(u,v)$ so far. In case they do not agree, they initiate a ``meeting points'' mechanism in order to find an agreed prefix of the partial transcript. 
In phase (ii), each party sends a flag to all its neighbors if either it found that its state was inconsistent with one of its neighbors in the previous phase, or it has simulated more chunks with one neighbor than with another neighbor, in which case it wants to truncate the transcript with the neighbor who is ahead before it resumes simulation. These flags are 
propagated throughout the network. 
In phase (iii), if a party received a flag in phase~(ii), the party simply waits and does not simulate until it believes that everything is consistent throughout the network.
In phase (iv), each party $u$ sends a neighbor $v$ a rewind message if $u$ has rewound its transcript due to a meeting points truncation with another neighbor $w$. As mentioned in the description of flag passing, each party wants to make sure it is at the same chunk with all of its neighbors before proceeding with simulation. The rewind phase allows each party to accomplish this goal without relying on the use of hash functions, which are prone to collisions. We elaborate more on this in~\cite{GKR-1}; indeed, the rewind phase was one of the main insights in that work.

In phase (i) (the consistency check phase), the parties send each other a hash of their current transcript. Unfortunately, the description of these hash functions is long---so long that they cannot send each other the desired seed without blowing up the rate of the coding scheme. In~\cite{GKR-1}, we get around this issue by assuming that the descriptions are contained in a common random string (CRS) that the parties share.

For more details, we refer the reader to~\cite{GKR-1}.

%

\paragraph{Removing the Common Random String assumption}
Recall that the parties generate hashes of their partial simulated transcripts in the consistency check phase (phase (i)). The hash function is chosen at random by sampling a (uniformly) random seed. These seeds together constitute the CRS. 

A basic idea for removing the CRS is to
simply have each pair of parties sample this seed and send it across their shared link. 
However, the length of the seed is similar to the length of the information we wish to hash (see Section~\ref{sec:hash} for further details on the hash function we use). 
Hence, sending it will increase the communication complexity by a quadratic factor. Instead, we use an idea from previous work~\cite{GMS11,BK12,haeupler14,GMS14}: the parties
communicate a short random string~$S$ which serves as a seed that generates a longer $\delta$-biased string.  This is done via a well-known technique by Naor and Naor~\cite{NN93}, or Alon et al.~\cite{AGHP92}. This $\delta$-biased randomness is used instead of the shared randomness above.

Intuitively, $\delta$-biased randomness suffices, since the hash function is linear, and thus hashing with a $\delta$-biased seed behaves ``close'' to hashing with a truly uniform seed.  However, this holds only when the input to the hash function is independent of the $\delta$-biased seed.  Unfortunately, in our setting, the input to the hash function may depend on the $\delta$-biased seed. Clearly, if the adversary is non-oblivious, they can look at the $\delta$-biased seed and choose their errors as a function of it, so the partial transcripts may be correlated with the seeds used to hash them. More problematic is that even if the adversary is \emph{oblivious}, the partial transcripts may depend on the seeds being used to hash them. Indeed, this is because the seeds are taken from a long $\delta$-biased seed, and so seeds being used in the current round are correlated with previously-used seeds. Specifically, the previous seeds determined whether there were hash collisions or not, which determines the state of the current partial transcript.

We circumvent this issue in a way similar to~\cite{haeupler14, BKN14}, by showing that a given pattern of hash collisions determines the (partial) transcripts throughout the protocol. Once the transcripts are fixed, the hashes output behave similarly to the case of uniform randomness, up to  a statistical difference proportional to~$\delta$.
Therefore, if $\delta$ is small enough, we can prove robustness for all possible fixed patterns of hash collisions.
Then, we can union bound over all the possible patterns of hash collisions, which bounds the failure probability for the $\delta$-biased case by the failure of the uniform case plus an error term that depends on $\delta$ and the cardinality of the different hash patterns. One cannot take~$\delta$ to be too small, since generating the $\delta$-biased string requires communicating $\approx O(m\log (1/\delta))$ bits, hence the smaller $\delta$ gets, the more communication we need.
Luckily, we can set $\delta$ to be sufficiently small so that the probability of failure is still exponentially small even after the union bound, while keeping a constant rate in the communication.



%
\paragraph{Dealing with a non-oblivious adversary}
Next, we consider the case where the adversary is non-oblivious. 
In particular, we assume that the adversary knows all the randomness of the parties. However, the adversary is still oblivious to any private randomness that a party may have.

Haeupler~\cite{haeupler14} dealt with this same issue in the two-party setting by simply applying a union bound over all the possible oblivious attacks. Unfortunately, as opposed to the two-party case of~\cite{haeupler14}, knowledge of the hash seeds in the multi-party setting gives the adversary too many options for attacks, and the proof fails spectacularly. 

To see why this is, fix an edge $(u,v)$ in the network, and suppose for simplicity that we use truly random functions for our hashes. Since we use constant-length hash outputs\footnote{In order to obtain a constant rate, the length of the hash output must be constant, see~\cite{GKR-1}.}
 and the adversary knows the random seeds ahead of time, with constant probability over the random seed, the adversary can corrupt the simulation on the link $(u,v)$ such that a hash-collision is guaranteed in the following consistency-check phase. In this case, the parties will continue to simulate (incorrectly) since they are not aware of the mismatch in their partial transcripts. 
%
However, note that with some constant probability, this mismatch will not be caught in the next consistency-check as well!
Generalizing the above reasoning, with probability $1/m$, the adversary is able to force hash-collisions on the link $(u,v)$ for $\Theta(\log m)$ consecutive phases, leading to $\Theta(m\log m)$ wasted communication. 
Since there are $m$ links for the adversary to choose from when making an error, with high probability there exists a link on which such an attack is possible, and the adversary who knows the random seeds, the inputs, and the protocol will be able to conduct this attack on it. 
Therefore, the non-oblivious adversary can create $\Theta(m\log m)$ wasted communication with just a single error. 


To overcome this issue, we increase the length of the hash output, so it is no longer constant
but rather $\Theta(\log m)$. Then the hash collision probability drops to $1/\poly(m)$, and
the union bound yields the desired outcome.
However, the length of each hash increased from a constant to $\Theta(\log m)$,
and
the rate of the coding scheme is no longer constant (recall that each iteration in the scheme of~\cite{GKR-1} takes $\Theta(m)$ communication).  
In order to retain a constant rate, we simulate the protocol in larger chunks. Namely, each phase (i)-(iv) now consists of $\Theta(m \log m)$ bits. In particular, instead of sending a hash every $\Theta(m)$ bits of communication of~$\Pi$, parties exchange hashes of length $\Theta(\log m)$ every $\Theta(m\log m)$ bits of simulation, thus increasing the overall communication by just a constant factor. However, as a result, we are resilient to at most $\eps / (m \log m)$ fraction of adversarial error.





==> nonobliv-crs.tex <==
%
\appendix[Improved Coding Scheme 
%
for Non-Oblivious Adversaries Assuming Pre-shared Randomness]
\label{sec:nonobliv-crs}
\subsection{An overview of scheme}
In this section we detail a coding scheme that tolerates fully general (non-oblivious) adversaries with error rate $1/m \log\log m$. This improves the noise rate achieved in Section~\ref{sec:nonobliv-no-crs}, in the setting where the parties can share a common random string. The parties use a common hash function $h_1$ which they agree on via their common random string, in the exact way that they do for the scheme for oblivious adversaries in~\cite{GKR-1}. 
%

In order to make this scheme robust to \emph{non-oblivious} adversaries that get to see the common random string, they need to increase the output size of the shared hash to $\Theta(\log m)$, just like in Section~\ref{sec:nonobliv-no-crs}. In addition, each party generates \emph{fresh} randomness in each iteration for each of its links, and shares these random strings with their neighbors. The parties use this randomness to further hash the outputs of the common hash function $h_1$ down to a constant size. 

Since the randomness used for this second hash is generated fresh in each iteration, the adversary cannot design their errors in previous iterations to cause hash collisions in this second hash, which allows the output size of this hash to be $\Theta(1)$. This technique is also used in the two-party setting by Haeupler~\cite{haeupler14} to improve the rate of the coding scheme.
%
In particular,
we use the construction of a hash-function with small seed length from~\cite{NN93}.\begin{lemma}[{\cite[Section~9]{NN93}}]
\label{cor:good-hash} 
There is a hash function family  $\{ h_{Q}\}_{Q \in \{ 0,1\}^{s}}$ with input length $L$~bits, 
output length~$\tau$ bits, and seed length $s = \Theta(\log L + \tau)$ such that, given any pair of inputs $x$ and $y$ (of length~$L$) where $x \neq y$, 
\[ 
\Pr_Q[h_Q(x) = h_Q(y)] \leq   2^{-\tau}.
\]     
\end{lemma}



\subsection{The protocol}
\begin{algorithm}[htp]
\caption{RobustProtocolV2  (for party $u$) for non-oblivious adversaries}
\label{alg:robust-protocol-2}
\begin{algorithmic}[1]
\small
\State InitializeState()
\State Let $\K := m\log\log m$ (so chunk size is $5m\log\log m$).
\State $S = \{S_{i,u,v} \}_{i,u,v} \gets \left(\{ 0,1\}^{\Theta(|\Pi|\K)}\right)^{100|\Pi| |E|}$ uniform shared randomness.
\For{$i=1$ to $100|\Pi|$}
  \ForAll{$v \in N(u)$ in parallel}	  \Comment{\textbf{meeting points}}
    \State $status_{u,v} \gets MeetingPointsV2(u,v, S_{i,u,v})$
  \EndFor
  \State \textbf{Rest same as in Algorithm \ref{alg:robust-protocol}.}
\EndFor
\end{algorithmic}
\end{algorithm}

\begin{theorem}
\label{thm:nonobliv-adv-crs}
Assume a network $G=(V,E)$ with $n=|V|$ parties and $m=|E|$ links. 
Suppose $\Pi$ is a multiparty protocol over the network~$G$ with communication complexity $\CC(\Pi)$, binary alphabet and fixed order of speaking. Let $|\Pi|  = \frac{\CC(\Pi)}{5m\log\log m}$ 
and let $\eps > 0$ be a sufficiently small constant.
%
\AlgImpNO correctly simulates~$\Pi$ with communication complexity $O(\CC(\Pi))$ with probability at least $1 - \exp(-\Omega(|\Pi|)))$ over the randomness of the parties, in the presence of a non-oblivious adversary limited to a noise fraction at most $\eps / m \log\log m$, as long as the parties are allowed to share a CRS (common random string).
\end{theorem}

\begin{algorithm}
\caption{\textbf{MeetingPointsV2}($u$,$v$, $S_{i,u,v}$) for non-oblivious adversaries with CRS}
\label{alg:meeting-points-2}
\begin{algorithmic}[1]
\small
\State // Initialization
  \State Method called by $u$, with $v \in N(u)$, $S_{i,u,v} \in \{ 0,1\}^{\Theta(|\Pi|\K)}$
  \State $h_1 \gets$ inner product hash function (Definition~\ref{def:ip-hash}) with input length $\Theta(|\Pi|\K)$, $p_1= \frac{1}{m^{\Theta(1)}}$ for a sufficiently small exponent, $o_1 = \Theta(\log m)$, $s = |S_{i,u,v}|$.
  \State $h_2 \gets$ binary hash family from Corollary~\ref{cor:good-hash} with input length $o_1$, $p_2 = \Theta(1)$ sufficiently small, $o_2 = \Theta(1)$, and $s_2 = \Theta(\log\log m)$.
  \State $S_1 \gets S_{i,u,v}$
  \State $S_2 \stackrel{\text{unif}}{\gets} \{ 0,1\}^{s_2}$ are fresh privately generated bits.
  \State $h_S \gets h_{2, S_2}(h_{1,S_1}(\cdot))$
    \State $k,E,mpc1,mpc2 \gets 0$
  
  \Statex
  \Statex // Execute per activation:
  \State $k \gets k+1$
  \State $\widetilde{k} \gets 2^{\lfloor \log k \rfloor}$. Let $c$ be the largest integer such that $c\widetilde{k} \leq |T_{u,v}|$.
  \State $T_1 \gets T_{u,v}[1:c\widetilde{k}], T_2 \gets T_{u,v}[1:(c-1)\widetilde{k}]$
  \State Send $(S_2, h_S(k), h_S(T_1), h_S(T_2))$ to neighbor $v$.
  \State Receive $(S_2', H_k', H_{T_1}', H_{T_2}')$ from our neighbor $v$.
  \State $h'_S \gets h_{2, S_2'}(h_{1,S_1}(\cdot))$ 
  \State $(H_k, H_{T_1}, H_{T_2}) \gets (h'_S(k), h'_S(T_1), h'_S(T_2))$.
  \If {$H_k \neq H_k'$}
    \State {$E \gets E+1$}
  \EndIf
  \If {$k=1, E=0$, and $H_{T_1} = H_{T_1}'$} \label{step:HashesMatch}
    \State {$k \gets 0$}
    \State {$status \gets$ ``simulate''}
    \Return $status$
  \EndIf
  \If {$H_{T_1} = H_{T_1}'$ or $H_{T_1} H_{T_2}'$}
    \State {$mpc1 \gets mpc1 + 1$}
  \ElsIf {$H_{T_2} = H_{T_1}'$ or $H_{T_2} = H_{T_2}'$}
    \State {$mpc2 \gets mpc2 + 1$}
  \EndIf
  \If {$2E \geq k$}~\label{step:resetMP}
    \State {$k \gets 0, E \gets 0, mpc1 \gets 0, mpc2 \gets 0$}
    \State {$status \gets$ ``meeting points''}
  \ElsIf {$k = \widetilde{k}$}
    \If {$mpc1 > 0.4k$}
      \State {$T \gets T_1$}
      \State {$k \gets 0, E \gets 0$}
    \ElsIf {$mpc2 > 0.4k$}
      \State {$T \gets T_2$}
      \State {$k \gets 0, E \gets 0$}
    \EndIf
    \State {$mpc1 \gets 0, mpc2 \gets 0$}
    \State {$status \gets$ ``meeting points''}
  \Else
    \State {$status \gets$ ``meeting points''}
  \EndIf \\
  \Return $status$ 
\end{algorithmic}
\end{algorithm}


\subsection{Bounding hash collisions for non-oblivious adversaries assuming a CRS}
\label{sec:bound-hash-nonoblivious-crs}
We denote the collision probabilities of the hash functions $h_1$ and $h_2$ by $p_{1}$ and $p_2$ respectively, where we note that $p_1 = \frac{1}{m^{\Theta(1)}}$ and $p_2$ is a sufficiently small constant. 
Similar to the analysis in~\cite{GKR-1}, we create a process $\psi_{u,v}$ that upper bounds $\varphi_{u,v}$, but now we take into account hash collisions from both hash functions. We will use the terminology that a hash function $h$ collides in $(i,u,v)$ if there is a hash collision when $u$ and $v$ exchange hashes in iteration $i$.

Similar to the definition in Section~\ref{sec:protocol-obliv-no-crs}, define $X_{i,u,v}$ for iterations when $\varphi_{u,v} > 0$ as 
\[ X_{i,u,v} = 
\begin{cases}
1 &\text{if $h_1$ collides in $(i,u,v)$} \\
0 & \text{otherwise} \\
\end{cases}
\]
and define $Y_{i,u,v}$ for iterations when $\varphi_{u,v} > 0$ as 
\[ Y_{i,u,v} = 
\begin{cases}
1 & \text{if $X_{i,u,v}=0$ and $h_2$ collides in $(i,u,v)$} \\
0 & \text{otherwise}
\end{cases}
\]

Then we define $\psi_{u,v}$ as follows:
\begin{algorithm}[H]
\caption{The process $\psi_{u,v}$}
\small
\begin{algorithmic}
\State $i \gets 1, \psi_{u,v}(1) \gets 0$
\ForAll{iterations $i$ from 1 to $100 |\Pi|$}
  \If {error occurs between $u$ and $v$\\ during iteration $i$, during any phase}
    \State $\psi_{u,v}(i+1) = \psi_{u,v}(i) + 6C_6$
  \ElsIf {$\psi_{u,v}(i) > 0$}
    \State $\begin{aligned}\psi_{u,v}(i+1) = &\psi_{u,v}(i) + (6C_6+5) X_{i,u,v} \\&+ 6C_6 (Y_{i,u,v}) - 5(1-Y_{i,u,v})\end{aligned}$
  \Else
    \State $\psi_{u,v}(i+1) = \psi_{u,v}(i)$ 
  \EndIf
\EndFor
\end{algorithmic}
\end{algorithm}
%
We argue that $\psi_{u,v}$ is an upper bound on $\varphi_{u,v}$ (that is, Lemma~\ref{lem:psi-lb-old} holds with this definition of $\psi_{u,v}$). Indeed, in the case of a hash collision in $h_1$, note that $\psi_{u,v}$ increases by $(6C_6+5) X_{i,u,v} + 6C_6 Y_{i,u,v} - 6(1-Y_{i,u,v}) = 6C_6 + 6 - 5(1) = 5C_6 + 1 \leq 6C_6$, and in the case of a hash collision in $h_2$, which only occurs in the absence of a hash collision in $h_1$, we get that $(6C_6+5) X_{i,u,v} + 6C_6 Y_{i,u,v} - 5(1-Y_{i,u,v}) = 6C_6$. In the absence of a hash collision in either, we have that $X_{i,u,v} = Y_{i,u,v} = 0$, and hence $\psi_{u,v}$ decreases by 5. This was all that was needed to establish Lemma~\ref{lem:psi-lb-old}; the remainder of the argument is identical to the proof of Lemma 4.15 in~\cite{GKR-1}.%
%



We will let $D$ denote the number of triples $(i,u,v)$ such that $\psi_{u,v}(i) > 0$ at the beginning of the iteration. Let $D' \leq D$ denote the number of such triples $(i,u,v)$ where, addititionally, there is no error between $u$ and $v$ in $i$. Let $D_2 \leq D'$ denote the number of triples $(i,u,v)$ where, in addition to this, there is no hash collision in $h_1$ in $(i,u,v)$. These are the triples where it is possible to have a hash collision in $h_2$, but there is no error. We start with the following proposition:
\begin{proposition}
\label{prop:hash2-bounded}
Let $D'$ be defined as above. The number of hash collisions in $h_2$ in triples without errors is at most $2 p_2 D'$ with probability $\geq 1 - \exp(-\Omega(p_2 D'))$.
\end{proposition}
\begin{proof}
Note that hash collisions in $h_2$ can only occur in triples in $D_2$ or in triples $(i,u,v)$ with an error between $u$ and $v$ in iteration $i$. In each of the $D_2$ triples $(i,u,v)$, the event of a hash collision in $h_2$ is either iid Ber($p_2$) or Ber(0), where the latter can happen if $T_{u,v}(i) \neq T_{v,u}(i)$ but $\psi_{u,v}(i) > 0$.

Instead, consider the sum of a sequence of $D'$ Ber($p_2$) random variables. This stochastically dominates the number of hash collisions in $h_2$ in triples without errors, since $D_2 \leq D'$ by definition. The statement follows from a standard Chernoff bound applied to the sum.
\end{proof}

\begin{lemma}
\label{lem:bound-comm-nonobliv-crs}
Let $\Err$ denote the number of errors that the non-oblivious adversary commits in an execution of RobustProtocolV2 (Algorithm \ref{alg:robust-protocol-2}), and let $\CC$ denote the communication complexity in the execution. Then with probability $1 - \exp(- \Omega(|\Pi|))$, we have that either $\CC \leq 200 \alpha |\Pi| m\log\log m$, or that $\Err > \frac{\eps}{m\log\log m} \CC$.
\end{lemma}
\begin{proof}
Recall that we set $\K = m\log\log m$. We will simply bound the upper probability that $\CC > 200 \alpha |\Pi| \K$ and simultaneously $\Err \leq \frac{\eps}{\K} \CC$. 
We invoke Lemma \ref{lem:cc-bound}, which is equivalent to Lemma~4.14 in~\cite{GKR-1}\footnote{Due to an unfortunate error, the last sentence of Lemma 4.14 was ommitted in~\cite{GKR-1}. The complete statement is exactly as appears in the above Lemma~\ref{lem:cc-bound}.},
to establish that these two events happen only if $D > \beta \cdot \Err$, where $\beta = \frac{CC}{3\alpha\K\Err} \geq \frac{1}{3\alpha \eps}$. Note that this holds for any adversary, oblivious or not.
\begin{lemma}[\cite{GKR-1}]
\label{lem:cc-bound}
Consider a run of Algorithm~\ref{alg:robust-protocol-2}.
Denote the number of dangerous triples in this run by~$D$, and the number of errors by~$\Err$. Suppose that the communication complexity in this run satisfies $\CC > 200\alpha |\Pi| \K$, where $\alpha$ is the constant multiplying the communication in Lemma \ref{lem:main-communication-old}, and suppose that $\Err \leq \frac{\eps}{\K} \CC$.

If $\Err > 0$, then $D \geq \beta \cdot \Err$, where $\beta \eqdef \frac{\CC}{3\alpha\K\Err} \geq \frac{1}{3\alpha \eps}$. If $\Err = 0$, then $D=0$ trivially.
\end{lemma}


Now our task is to establish that 
\begin{equation}\label{eq:nonobliv-crs-1}
\Pr[D > \beta \Err] \leq \exp(- \Omega(|\Pi|))
\end{equation}
for any adversary, which will bound the communication complexity of the protocol for any adversary. First, we note that if $D > \beta \Err$, then $D'$, the number of triples that additionally have no error, is at least $(\beta-1)\Err$. Therefore, Proposition \ref{prop:hash2-bounded} tells us that the number of collisions in the hash $h_2$ (in triples without errors) is at most $2p_2 D'$ with probability at least $1 - \exp(-\Omega(p_2 D')) \geq 1 - \exp(-\Omega(p_2 |\Pi|))$, for any adversary, where we use the fact that $D' \geq (\beta-1) \cdot \Err = \Omega(\CC / \K) = \Omega(|\Pi|)$. 

We can use this to condition on the event that the number of hash collisions in $h_2$ is at most~$2p_2D'$, without losing too much in our bound. Formally, Proposition~\ref{prop:hash2-bounded} gives us that
\begin{equation}
\label{eq:nonobliv-crs-2}
\begin{aligned}
\Pr[D > \beta \Err] 
\leq &\Pr[(D > \beta \Err) \mid (\text{\# hash col in $h_2 \leq 2p_2 D'$})] \\
&+ \exp(-\Omega(p_2 |\Pi|))
\end{aligned}
\end{equation}
for any (non-oblivious) adversary. So it suffices to show that, conditioned on the number of hash collisions in $h_2$ being at most $2p_2 D'$, no adversary can make $D > \beta \Err$ except with negligible probability, where the probability is taken over both the CRS and the privately sampled randomness.

This is done by showing this fact for any adversary that additive and \emph{oblivious to collisions in $h_1$}, this occurs with probability at most $\exp(-\Omega(\beta \cdot \Err \cdot \log m))$(shown below in Lemma \ref{lem:bound-dangerous-nonobliv-crs}).

To establish the result for arbitrary adversaries, we union bound the above probability over all possible oblivious, additive adversaries that induce more than errors and show this is $\exp(- \Omega(\eps |\Pi| \log m))$. This is very similar to what we did in Section~\ref{sec:nonobliv-no-crs}. 
The number of oblivious, additive adversaries that induce exactly $\Err$ errors is at most
\begin{equation}
\label{eq:num-adversaries-crs}
\binom{C|\Pi|m^2\log\log m }{\Err} \cdot 2^{\Err}
\end{equation}
for some constant $C$. For a proof of this fact, see the proof of Claim~\ref{claim:num-adversaries}; the proof of this fact is identical, with the $\log m$ replaced by $\log\log m$ due to the fact that we take $K = m\log\log m$ in this section. Now, we separate the remainder of the proof into cases.

\textbf{Case 1: $\Err \leq 200 \alpha \eps |\Pi|$}. In this case, we use the montonicity of binomial coefficients where the bottom is much smaller than the top to upper bound the right-hand side of Eq.~\eqref{eq:num-adversaries-crs} by $\binom{C |\Pi|m^2\log\log m}{200 \alpha \eps |\Pi|}$. Then, we apply the inequality that $\binom{n}{k} \leq \left( \frac{ne}{k}\right)^k$ to get that the number of such adversaries is at most $\exp(O(\eps |\Pi| \cdot \log m))$.

Hence, the probability that there exists an oblivious adversary that makes at most $200 \alpha \eps |\Pi|$ errors and manages to make $D > \beta \Err$  (conditioned on the number of hash collisions in $h_2$ being at most $2 p_2 D'$) is at most
\[\sum_{\Err = 1}^{200 \alpha \eps |\Pi|} \exp(O(\eps |\Pi| \cdot \log m)) \cdot 
\exp(- \Omega(\beta \Err \cdot \log m))\]
Using the fact that $\beta \cdot \Err = \Omega(|\Pi|)$ by the definition of $\beta$, we can simplify the above to 
\[ 
\exp(- \Omega(|\Pi| \log m)),
\]
as desired.

\textbf{Case 2: $\Err > 200 \alpha \eps |\Pi|$}. In this case, we directly apply the inequality that $\binom{n}{k} \leq \left( \frac{ne}{k}\right)^k$ to get that the number of such adversaries is at most $\exp(O(\Err \cdot \log m))$.

Hence, the probability that there exists an oblivious adversary that makes at most $200 \alpha \eps |\Pi|$ errors and manages to make $D > \beta \Err$ (conditioned on the number of hash collisions in $h_2$ being at most $2 p_2 D'$) is at most
\[ \sum_{\Err = 200\alpha \eps |\Pi| + 1}^{C|\Pi|m^2\log\log m} \exp(O(\Err \cdot \log m)) \cdot \exp(- \Omega(\beta \Err \cdot \log m))\]
Using the fact that $\beta \geq 1 / (3 \alpha \eps)$, we can simplify this down to 
\( \exp(- \Omega(- \beta  \Err\cdot \log m)\)
and using the fact that $\beta \cdot \Err = \Omega(|\Pi|)$, we get
\( 
\exp(- \Omega(|\Pi| \log m))
\)
as desired.

Putting the two cases together with Eq.~\eqref{eq:nonobliv-crs-2}, we establish Eq.~\eqref{eq:nonobliv-crs-1}, completing the proof.
\end{proof}

\begin{lemma}
\label{lem:bound-ehc-nonobliv-crs}
Let $\Err$ denote the number of errors that the non-oblivious adversary commits in an execution of RobustProtocolV2 (Algorithm \ref{alg:robust-protocol-2}), let $D$ denote the number of triples $(i,u,v)$ with $\psi_{u,v}(i) > 0$, and let $\eps^*>0$ be a fixed constant larger than $4000 \alpha C_6 \eps$. Then with probability $1 - \exp(- \Omega(|\Pi|))$, we have that $\Err \leq 200 \alpha \eps |\Pi|$ and $D \leq \eps^* |\Pi|$, or that $\Err > \frac{\eps}{m\log\log m} \CC$.
\end{lemma}
We note that the probability in Lemma~\ref{lem:bound-ehc-nonobliv-crs} hides factors of $\eps^*$ in the exponent. However, since $\eps^*$ is not going to 0 with $\eps$, we do not include it in the exponent.
\begin{proof}
First we can bound the probability that $\Err > 200 \alpha \eps |\Pi|$ and simultaneously \\$\Err \leq (\eps / m\log\log m)\CC$. These two events occur simultaneously only if $\CC > 200 \alpha |\Pi| \K$, and we already upper bounded the probability of this event with the desired quantity in Lemma~\ref{lem:bound-comm-nonobliv-crs}. All that remains is to bound the probability that $\Err \leq 200 \alpha \eps |\Pi|$ and simultaneously $D > \eps^* |\Pi|$, which will establish the desired result.

Finally, we consider any adversary and upper bound the probability that it can cause $D > \eps^* |\Pi|$, conditioned on the number of errors being at most $200 \alpha \eps |\Pi|$. This implies that $D' > (19/20) \eps^* |\Pi|$, and so Proposition \ref{prop:hash2-bounded} implies that the number of hash collisions from $h_2$ is at most $2 p_2 D'$ with probability at least $1 - \exp(-\Omega(p_2 \eps^* |\Pi|)) \geq 1 - \exp(-\Omega(|\Pi|))$. 

Then, it remains to show that our nonoblivious adversary cannot cause $D$ to be too large conditioned on this event, as conditioning on this event can add at most $\exp(-\Omega(|\Pi|))$ to the overall probability. Similar to the proof of Lemma~\ref{lem:bound-comm-nonobliv-crs}, we apply Lemma~\ref{lem:bound-dangerous-nonobliv-crs} to get that $\Pr[D > \eps^* |\Pi|] < \exp(-\Omega(\eps^* |\Pi| \log m))$ for any additive adversary that is \emph{oblivious} to collisions in $h_1$ and commits at most $200 \alpha \eps |\Pi|$ errors.  

Doing the same union bound over all oblivious, additive adversaries that make at most $200\alpha \eps|\Pi|$ errors as done in the proof of Lemma~\ref{lem:bound-comm-nonobliv-crs} proves that no adversary can cause $D > \eps^* |\Pi|$ with probability more than $\exp(-\Omega(|\Pi|))$. Formally, there are at most $\exp(O(\eps |\Pi| \cdot \log m))$ adversaries that commit at most $200 \alpha \eps |\Pi|$ errors. Hence, the probability that any nonoblivious adversary that commits at most $200 \alpha \eps |\Pi|$ errors can cause $D > \eps^* |\Pi|$ (conditioned on the number of hash collisions in $h_2$ being at most $2 p_2 D'$) is at most 
\begin{multline*}
\sum_{\Err=1}^{200\alpha\eps|\Pi|} \exp(O(\eps |\Pi| \cdot \log m)) \cdot \exp(-\Omega(\eps^* |\Pi| \log m)) \\
= \exp(-\Omega(|\Pi|\log m)),
\end{multline*}
which completes the proof.
\end{proof}
\begin{lemma}
\label{lem:bound-dangerous-nonobliv-crs}
Suppose that the number of hash collisions in $h_2$ in triples without errors is at most $2 p_2 D'$, where $p_2$ is the hash collision probability of the second hash function. Let $p_1 = \frac{1}{m^{\Theta(1)}}$ be the hash collision probability of $h_1$. Then, fix an arbitrary \emph{oblivious} adversary, and let $k$ be a number larger than $10C_6$. Then 
\[ \Pr[D > k \cdot \Err] \leq \exp(-\Omega(k \cdot \Err \cdot \log m))\]
\end{lemma}
\begin{proof}
Fix the errors that the adversary commits, then consider running RobustProtocolV2 (Algorithm \ref{alg:robust-protocol-2}). Suppose that this run has $D > k \cdot \Err$. Recall that $D' \leq D$ be the set of triples $(i,u,v)$ where $\psi_{u,v}(i) > 0$ and no error occurs between $u$ and $v$ in $i$. Since the number of errors is $\Err$, we get that $D' \geq (k-1) \cdot \Err$. Now we argue that the fraction of hash collisions required to be in $D'$ must be very large, and that this occurs with very low probability. Denote the set of these $D'$ triples as $\wtD$ for concreteness.

Due to the nonnegativity of $\sum \psi_{u,v}$, this implies that 
\begin{multline*}
\sum_{{(i,u,v) \in \wtD}} (6C_6 + 5) X_{i,u,v} + 6C_6 (Y_{i,u,v}) - 5(1-Y_{i,u,v}) \\
\geq -6 C_6 \Err
\end{multline*}
Simplifying and using the fact that $|\wtD| = D' > 6C_6 \Err$, we get that
\[ \sum_{(i,u,v) \in \wtD} (X_{i,u,v} + Y_{i,u,v}) \geq \frac{4}{6C_6 + 5} D'. \]
Finally, using the assumption that $\sum_{S'} Y_{i,u,v} \leq 2 p_2 D'$, and by taking $p_2$ to be a sufficiently small constant such that $p_2 < 1/(10C_6 + 10)$, this implies that
\[ \sum_{(i,u,v) \in \wtD} X_{i,u,v} \geq \frac{3}{6C_6 + 5} D'. \]
So we can upper bound $\Pr[D > k \Err]$ by upper bounding the probability that $\sum_{(i,u,v) \in \wtD} X_{i,u,v} \geq \frac{3}{6C_6 + 5} D'$. Using a Chernoff bound, we get 
\begin{multline*}
\Pr\left[\frac{1}{D'}\sum_{(i,u,v) \in \wtD} X_{i,u,v} \geq p_1 + \frac{2}{6C_6 + 5}\right] 
\\
\leq \exp\left (-\Omega \left(k \Err \log \frac{1}{p_1}\right)\right).
\end{multline*}
By using the fact that $\log(1/p_1) = \Theta(\log m)$, we conclude the result.
\end{proof}

Finally, we can put Lemma~\ref{lem:bound-comm-nonobliv-crs} and~\ref{lem:bound-dangerous-nonobliv-crs} together to prove Theorem~\ref{thm:nonobliv-adv-crs}. 
\begin{proof}[Proof of Theorem~\ref{thm:nonobliv-adv-crs}]
Due to Lemmas~\ref{lem:bound-comm-nonobliv-crs} and~\ref{lem:bound-dangerous-nonobliv-crs}, with probability $1 - \exp(-\Omega(|\Pi|)$, we can conclude that $\CC \leq 200 \alpha \K |\Pi| = O(\CC(\Pi))$ and that the number of errors and hash collisions in the protocol is bounded by $\EHC \leq O(\eps^* |\Pi|)$, where $\eps^* > 0$ is a constant that is larger than $\eps$ but is sufficiently smaller than $C_7$. 

Finally, we recall that the potential $\phi$ rises by at least $\K$ in each iteration, and there are $100 |\Pi|$ iterations (Lemma~\ref{lem:main-communication-old}). Claim~\ref{claim:final-claim} yields the final result.
\end{proof}


==> nonobliv-no-crs.tex <==
%
\section{A Coding Scheme for Non-Oblivious Noise}
\label{sec:nonobliv-no-crs}
\subsection{Overview}
\label{sec:nonobliv-no-crs-overview}
In this section, we generalize the result of the previous section to hold for nonoblivious adversaries. Nonoblivious adversaries have a lot of power: specifically, they can look at the random seeds that will be used in the rest of the protocol and choose their errors as a function of these seeds. The upshot is that we can no longer guarantee that the event of a hash collision is independent of previous hash collisions, or even close to independent. We briefly recall (from the Introduction) the issues that can occur with an adversary that knows the random seeds used ahead of time, even when these seeds are initially sampled from a uniform distribution.

Suppose that the seeds to the hash functions are fixed, and that a randomly selected error creates a hash collision in the next round with probability $p$. Then roughly a $p$ fraction of the possible errors would lead to a hash collision on this link in the next Simulation phase, and hence be undiscovered. Among the errors that caused a collision, roughly a $p$ fraction of them would lead to a hash collision in the proceeding link, and so on. Hence, if the number of error patterns is sufficiently large, the adversary can select a specific error pattern out of them that will not be detected within a large sequence of iterations.
%
In particular, 
since there are $\K = \poly(m)$ bits communicated in a single chunk, the adversary has a choice of $\poly(m)$ errors in any simulation phase, so that there exists an error that is undetectable for 
$\Theta(\log m)$ iterations with high probability. 


To address this issue, we modify our hash function to have a collision probability of~$p = \frac{1}{m^{\Theta(1)}}$, by increasing the output size of our hash to $\Theta(\log m)$~bits. This, however, affects the rate of the coding scheme.
In order to keep the rate constant, we set $\K$ to be $m\log m$, %
i.e., the size of each chunk increases and we effectively send hashes (and other meta-data) less frequently. 
%
We then appeal to the strategy of~\cite{haeupler14}, and show that there is no \emph{oblivious, additive} adversary that sabotages
the simulation with high probability. 
In particular, for any given oblivious, additive adversary, there are exponentially few ``bad'' randomness strings that do not guarantee a correct and constant rate simulation.
Taking a union bound over all possible oblivious, additive adversaries, we show that the union of all the ``bad'' randomness strings is still exponentially small. This means that unless a bad randomness is picked by the parties, \emph{no} oblivious, additive adversary can invalidate the simulation. But the actions of any non-oblivious adversary that makes $\Err$ errors can always be modeled by \emph{some} oblivious, additive adversary that makes $\Err$ errors---simply take the oblivious adversary that miraculously manages to make the same corruptions. Hence, no non-oblivious adversary can invalidate the simulation for the same randomness.


\subsection{A noise-resilient simulation for non-oblivious adversarial noise}
\label{sec:AlgNODef}
Define \AlgNO to be Algorithm~\ref{alg:robust-protocol} combined with the InitializeState() procedure described in Algorithm~\ref{alg:initialize-state-3} below.

\begin{algorithm}[htp]
\caption{InitializeState() for non-oblivious noise without a CRS}
\label{alg:initialize-state-3}
\begin{algorithmic}[1]
\small
\State $\K \gets m\log m$
\ForAll{neighbors $v \in N(u)$ in parallel}
  \State Initialize $T_{u,v} = \emptyset$
  %
  \State $status_{u,v} \gets$ ``simulate''
  \State $alreadyRewound_{u,v} \gets 0$
  \State $\delta := 2^{-\Theta(|\Pi|\K/m)}$
  \State $S := (S_{i,u,v})_{i \in [100|\Pi|]} \gets$ RandomnessExchange($u$, $v$, $\delta$, $\K$)
\EndFor
\State $status_u \gets 1$.
\State $netCorrect_u \gets 1$
\end{algorithmic}
\end{algorithm}
The only difference in InitializeState() from Section~\ref{sec:protocol-obliv-no-crs} is that $\K$ is set to $m\log m$.

%



\subsection{\AlgNO: Analysis}


The main result of this section is the following theorem, arguing that \AlgNO is resilient to non-oblivious adversary that corrupts up to a fraction~$\eps / m \log m$ of the transmissions, with high probability.
\begin{theorem}
\label{thm:nonobliv-adv-no-crs}
Assume a network $G=(V,E)$ with $n=|V|$ parties and $m=|E|$ links.
Suppose $\Pi$ is a multiparty protocol over the network~$G$ with communication complexity $\CC(\Pi)$, binary alphabet and fixed order of speaking. 
Let $|\Pi|  = \frac{\CC(\Pi)}{5m\log m}$ 
and let $\eps > 0$ be a sufficiently small constant.
%
Assume an instance of \AlgNO with a non-oblivious adversary. Denote by $\Err$ the number of error the adversary made in that instance, and let $\CC$ be the communication complexity of that instance.
Then, with probability at least $1 - \exp(-\Omega(|\Pi| \log m))$ over the randomness of the parties
either $\Err > \tfrac{\eps}{m\log m} \CC$ or
\AlgNO correctly simulates~$\Pi$ with communication complexity $O(\CC(\Pi))$.
\end{theorem}



Recall that in \AlgNO we set $\K = m\log m$. We will use $\K$ and $m\log m$ interchangeably throughout this section, often leaving expressions in terms of $\K$ and plugging in $m\log m$ at the end.


As mentioned in the overview in Section~\ref{sec:nonobliv-no-crs-overview}, our general strategy is to union bound over all oblivious additive adversaries to show that the fraction of random strings that lead to bad outcomes is small. We start by showing a simple but useful claim, which provides a bound on the number of different oblivious, additive adversaries that can commit a fixed number of errors.

\begin{claim}
\label{claim:num-adversaries}
Fix a nonnegative integer $\Err$. Assuming a large enough~$m$, 
the number of different oblivious additive adversaries that commit exactly $\Err$ errors is at most 
\[ 
\binom{C|\Pi| m^2\log m}{\Err} \cdot 2^{\Err}
\]
for some constant $C>0$. Furthermore, if $\Err > C\eps m|\Pi|$, then $\Err > \frac{\eps}{m\log m}\CC$
where $\CC$ denotes the communication of the robust protocol.
\end{claim}
\begin{proof}
Each oblivious adversary can be described by a fixed corruption pattern, $\mathsf{cor}\in \{0,1,2\}^{2m\RC}$, where $\RC$ is the (fixed) round complexity of \AlgNO given~$\Pi$. The number of errors is the number of non-zero indices of that string. Therefore, in order to bound the total number of oblivious-adversaries we need to bound the number of different such strings. 


In the randomness exchange part of the protocol, there are $\Theta(\frac{\K}{m}|\Pi|) = \Theta(|\Pi|\log m)$ rounds, and in each of them there are at most $m$ links which the adversary can corrupt. Therefore, there are $\Theta(|\Pi|m\log m) = O(|\Pi|m^2\log m)$ places for the adversary to put errors in the randomness exchange phase.

In the main part of the protocol, each iteration has at most $O(m\log m)$ rounds (see below for a justification) and there are $100 |\Pi|$ iterations. In each round, the adversary can choose which of $2m$ possible (directed) links to put an error. Putting this together, we get that there are at most $O( |\Pi|m^2 \log m)$ places for the adversary to put an error in the main part of the protocol. 
%
To summarize, there are \( 
\binom{C|\Pi| m^2\log m}{\Err} 
\)
ways for the adversary to corrupt exactly $\Err$ places out of the $O(|\Pi| m^2\log m)$ potential communication events, where we let~$C$ be the constant hidden in the big~$O$.

In each place where an oblivious additive adversary commits an error, it can choose one of two possibilities $\mathsf{cor}_{i,(u,v)}\in\{0,1,2\}$, where $\mathsf{cor}_{i,(u,v)}=0$ does not alter the transmission (recall the additive-adversary definition in Section~\ref{sec:preliminaries}).
This yields the $2^{\Err}$~term.


We now justify why there are at most $O(m\log m)$ rounds per iteration. 
Each meeting points phase takes $\Theta(\K/m)$ rounds in which 5 hash values, each of length $\Theta(\K/m)$, are being exchanged between each pair of parties (in parallel). Note that $\Theta(\K/m) = \Theta(\log m) = O(m\log m)$. 
%
The flag passing phase has (at most) $n=O(m\log m)$ rounds. The simulation phase takes $5K+1=5m\log m+1$ rounds (where one round is for the $\perp$ symbols), and the rewind phase takes $n =O(m\log m)$ rounds. 
Putting them all together the round number is at most $O(m\log m)$. 


The second part of the claim follows since there are only $\leq C|\Pi| m^2\log m$ pairs of (round, directed link) where there can possibly be communication during the protocol, and so we get a trivial upper bound on the communication complexity as $C|\Pi|m^2\log m$. 
\end{proof}


Next, we consider the communication complexity of \AlgNO.
Recall that while the round complexity is fixed, the communication complexity depends on the inputs, noise, and randomness.
We now show that the probability that the adversary can make the communication of the robust protocol larger than $O(CC(\Pi))$, if bounded to its allowed budget, is negligible.


Recall that \AlgNO has two parts: the randomness exchange part, which happens in InitializeState(), and the main part, where the actual simulation occurs. Claim~\ref{claim:randomness-exchange-comm} bounds the communication in the randomness exchange by $\Theta(|\Pi|\K) = \Theta(|\Pi|m\log m)$. Therefore, we are only left to show that communication in the main part of \AlgNO is bounded by $\Theta(|\Pi|\K)$, for any non-oblivious adversary.  


We begin with upper bounding the probability that the communication is too large for any specific \emph{oblivious} adversary. This bound
will be sufficiently strong so that we could later union bound over \emph{all} oblivious adversaries and prove the general case (Lemma~\ref{lem:nonobliv-cc-bound-2}).
\begin{proposition}
\label{prop:nonobliv-cc-main-prop}
Fix an oblivious adversary, and denote the number of errors it commits as~$\Err$. Let~$\CC$ denote the communication complexity of the entire protocol, and $\CC'$ denote the communication complexity in the main part. Then
\begin{equation}\begin{multlined}
\label{eq:nonobliv-cc-1}
\Pr \left[(\CC' > 400\alpha|\Pi|\K) \wedge (\Err \leq \tfrac{\eps}{\K} \CC)\right] \\
\leq 
\begin{cases}
\exp(-\Omega(|\Pi| \log m)) &\textup{\small if $\Err \leq 400 \alpha \eps' |\Pi|$} \\
\exp(-\Omega(\log m \cdot \Err / \eps)) &\textup{\small otherwise}
\end{cases},
\end{multlined}
\end{equation}
%
over the randomness of the parties, 
where $\eps' = \Theta(\eps)$ is given by Lemma~\ref{claim:effective-noise}.
\end{proposition}




\begin{proof}
Recall from Section~\ref{sec:protocol-obliv-no-crs} that the adversary can tamper with the randomness exchanges on some links. In line with the notation in Section~\ref{sec:protocol-obliv-no-crs}, denote the set of edges that share randomness successfully as $E' \subseteq E$, and additionally define $J \eqdef |E \setminus E'|$ to be the number of tampered edges, for notational convenience. Recall from Section~\ref{sec:protocol-obliv-no-crs} that when $J \geq 1$, the communication in the rest of the protocol can increase; however we can use Lemma~\ref{lem:main-communication-no-crs} to address this, similarly to how we used it in Section~\ref{sec:protocol-obliv-no-crs}. Note that, since the randomness in the randomness exchange phase is encoded with a code with constant distance, and since $\log(1/\delta) = \Theta(|\Pi|\K / m )$, we have that
\begin{equation}
\label{eq:j-ub}
J \leq %
\Theta \left(\frac{\Err \cdot m}{\K |\Pi|}\right)\text{.}
\end{equation}
This is because it takes $\Theta(\frac{\K}{m} |\Pi|)$ errors to corrupt the randomness exchange on any single edge. 




Furthermore, recall from Claim~\ref{claim:effective-noise} that $\Err \leq \frac{\eps'}{\K} \CC'$ for $\eps' = \Theta(\eps)$, and this implies that the \emph{effective} noise rate
on the main part of the protocol is $\Err' / \CC' \leq \Err / \CC' \leq \eps' / \K$. Hence, we write
\begin{align}
\nonumber
&\Pr\left[\left(\CC' > 400\alpha|\Pi|\K\right) \wedge \left( \Err \leq \frac{\eps}{\K} \CC\right) \right] \\
&\leq \Pr\left [(\CC' > 400\alpha|\Pi|\K) \wedge (\Err \leq \frac{\eps'}{\K} \CC')\right] \nonumber \\
&=\Pr\left[(\CC' > 400\alpha|\Pi|\K) \wedge (\CC' \geq \frac{\K}{\eps'} \Err)\right] \text{,}\label{eq:nonobliv-cc-2}
\end{align}
where in the second line we just rearranged the condition that $\Err \leq \frac{\eps'}{\K} \CC'$.

The fact that $\Err' \leq \frac{\eps'}{\K}\cdot \CC'$ also lets us invoke Lemma~\ref{lem:main-communication-no-crs}, which  will be our main tool here. Recall that the our hash collision probability is $p= 2^{-\Theta(\K / m)}$, then the Lemma gives,
\begin{equation} 
\label{eq:main-communication-obliv-no-crs}
\begin{multlined}
\Pr \left[(\CC' > 100 \gamma \alpha |\Pi|\K(1 + J)) \wedge (\CC' \geq \tfrac{\K}{\eps'} \Err)\right]
\\
 \leq \exp(-\Omega(\gamma |\Pi| \cdot (1 + J) \tfrac{\K}{m}))\text{,}
\end{multlined}
\end{equation}
where $\gamma \geq 2$ is a parameter we can set at our convenience. 





\begin{figure*}[!t]
\begin{equation} 
\Pr\left[\left(\CC' > \gamma' (100 \alpha |\Pi|\K + \Theta(\Err \cdot m))\right) \bigwedge \left(\CC' \geq \frac{\K}{\eps'} \Err\right)\right] 
%
\leq \exp\left(-\Omega \left(\frac{\gamma' |\Pi|\K + \Err \cdot \gamma' \cdot m}{m}\right)\right)
\label{eq:main-communication-obliv-no-crs-newGamma}
\end{equation}
%
\hrulefill
%
\vspace*{4pt}
\end{figure*}




We recall upper bound for $J$ in terms of the number of errors, namely that $J \leq \Theta(\frac{\Err \cdot m}{\K |\Pi|})$. We can ``plug in'' this upper bound into  Eq.~\eqref{eq:main-communication-obliv-no-crs} by absorbing a factor of $\frac{1+J}{1+ \Theta(\Err \cdot m / (K|\Pi|))}$ into $\gamma$.
That is, let $\gamma'>2$ and set $\gamma = \gamma' \cdot \frac{1+ \Theta(\Err \cdot m / (K|\Pi|))}{1+J}\ge \gamma'>2$.
%
Then, 
{\small
\begin{align} 
& \Pr\left[\left(\CC' > \gamma' (100 \alpha |\Pi|\K + \Theta(\Err \cdot m))\right) \bigwedge \left(\CC' \geq \frac{\K}{\eps'} \Err\right)\right] \nonumber \\
&=\Pr \left[\begin{gathered}\left(\CC' > 100 \gamma' \alpha |\Pi|\K\left(1 + \Theta\left(\frac{\Err \cdot m}{K |\Pi|}\right)\right)\right) \\ \bigwedge \left(\CC' \geq \frac{\K}{\eps'} \Err\right)\end{gathered}\right] \nonumber \\
&= \Pr \left[\left(\CC' > 100 \gamma \alpha |\Pi|\K \left(1 + J \right) \right)\bigwedge \left(\CC' \geq \frac{\K}{\eps'} \Err\right)\right] \nonumber \\
&\leq\exp(-\Omega(\gamma |\Pi| \cdot (1 + J) \tfrac{\K}{m})) \nonumber\\
&= \exp(-\Omega(\gamma' (1+\Theta(m\Err/K|\Pi|) |\Pi|  \tfrac{\K}{m}))
\nonumber
\\
&\leq \exp\left(-\Omega \left(\frac{\gamma' |\Pi|\K + \Err \cdot \gamma' \cdot m}{m}\right)\right)\text{.} \label{eq:main-communication-obliv-no-crs-2}
\end{align}
}%
The first inequality is due Eq.~\eqref{eq:main-communication-obliv-no-crs} and the fact that  $\gamma\ge\gamma'\ge2$. We can conclude with Eq.~\eqref{eq:main-communication-obliv-no-crs-newGamma}.
%


We will apply Eq.~\eqref{eq:main-communication-obliv-no-crs-newGamma} to bound the probability on the left-hand side of Eq.~\eqref{eq:nonobliv-cc-1} for the two cases of the statement.

\smallskip\noindent
\textbf{Case 1:} $\Err \leq 400 \alpha \eps' |\Pi|$.

In this case, we note that $\Theta(\Err \cdot m) \leq 100 \alpha |\Pi| \K$ due to the fact that $\eps'$ can be taken to be much smaller than the constant hidden by the $\Theta$. 
Hence, we can select $\gamma' \geq 2$ such that $400\alpha|\Pi|\K \geq \gamma' (100 \alpha |\Pi|\K + \Theta(\Err \cdot m))$. Therefore, Eq.~\eqref{eq:nonobliv-cc-2} becomes as follows:  
\begin{align}
&\Pr\left[(\CC' > 400\alpha|\Pi|\K) \wedge (\CC' \geq \tfrac{\K}{\eps'} \Err)\right] \nonumber \\
&\leq \Pr \left[(\CC' > \gamma' (100 \alpha |\Pi|\K + \Theta(\Err \cdot m))) \wedge (\CC' \geq \tfrac{\K}{\eps'} \Err)\right]\nonumber \\
&\leq \exp(-\Omega(|\Pi|\tfrac{\K}{m})) \nonumber \\
&\leq \exp(-\Omega(|\Pi|\log m))\text{.}
\label{eq:nonobliv-cc-3}
\end{align}
The third line follows from Eq.~\eqref{eq:main-communication-obliv-no-crs-newGamma} with the appropriately selected $\gamma'\ge2$.

\smallskip\noindent
\textbf{Case 2:} $\Err > 400 \alpha \eps' |\Pi|$.

In this case, we claim that $\CC' \geq \frac{\K}{\eps'} \Err$ already implies that $\CC'$ is large enough to apply Eq.~\eqref{eq:main-communication-obliv-no-crs-newGamma} to bound $\Pr[\CC' \geq \frac{\K}{\eps'} \Err]$. To see this, note that $\frac{\CC'}{2} \geq \frac{\K}{2\eps'} \Err \gg \Theta(\Err \cdot m)$ and that $\frac{\CC'}{2} \geq \frac{\K}{2\eps'} \Err \geq 200 \alpha |\Pi| \K$.
Setting $\gamma' \ge \frac{K}{\eps'} \cdot \frac{\Err}{100 \alpha |\Pi| \K + \Theta(\Err \cdot m)} \ge 2$ we get that
$\CC' \ge \gamma' (100 \alpha |\Pi|\K + \Theta(\Err \cdot m))$, and we can apply Eq.~\eqref{eq:main-communication-obliv-no-crs-newGamma} and plug in our choice for~$\gamma'$, to obtain
\begin{align}
\Pr[\CC' \geq \tfrac{\K}{\eps'} \Err] \leq \exp(-\Omega(\tfrac{\K}{m\eps'} \Err)) 
\leq \exp(-\Omega(\tfrac{\log m }{\eps}\Err )), \label{eq:nonobliv-cc-4}
\end{align}
which completes the proof.
\end{proof}

Equipped with Proposition~\ref{prop:nonobliv-cc-main-prop}, we proceed to proving the next lemma that generalizes the communication bound to the case of a general non-oblivious adversary. Towards that goal, we union bound over all the possible oblivious adversaries and show that there are many choices of randomness that work well for all the oblivious adversaries simultaneously.
\begin{lemma}
\label{lem:nonobliv-cc-bound-2}
Let $\K=m\log m$, $|\Pi|= \frac{\CC(\Pi)}{5\K}$ and let $\eps > 0$ be a sufficiently small constant. 
Consider executions of~\AlgNO with a corruption patten~$\mathsf{cor}\in \{0,1,2\}^{2m\RC(\Pi)}$. Denote by $\Err$ the number of non-zero indices in  $\mathsf{cor}$ and 
by $\CC'$ the communication in the main part of the algorithm assuming the corruption~$\mathsf{cor}$. 
It holds that
\begin{multline*}
\Pr \left [
\begin{aligned}
&\exists \mathsf{cor}\in \{0,1,2\}^{2m\RC} : \\
& \left(\CC' > 400\alpha|\Pi|\K\right) \wedge \left(\Err \leq \tfrac{\eps}{\K} \CC\right ) 
\end{aligned}
\right]
\\
\le  \exp(-\Omega(|\Pi| \log m))
\end{multline*}
%
over the randomness of the parties, where $\alpha$ is the constant from Lemma~\ref{lem:main-communication-old}. 
\end{lemma}

\begin{proof}
We will union bound over all possible oblivious additive adversaries to show that none of them can force a large amount of communication. Recall from Claim~\ref{claim:num-adversaries} that the number of adversaries that commit exactly $\Err$ errors is at most 
\begin{equation}
\label{eq:num-adversaries}
\binom{C|\Pi|m^2\log m}{\Err} \cdot 2^{\Err}
\end{equation}
and that we can take $\Err \leq O(\eps m |\Pi|)$ 
without loss of generality when considering adversaries that do not exceed their error budget. 

We continue by considering two cases, namely when $\Err$ is at most $400 \alpha \eps' |\Pi|$ and when it is bigger than that.
%
Suppose that $\Err \leq 400 \alpha \eps' |\Pi|$. 
Since $\eps'$ is sufficiently small, $\Err$ is much smaller than $C|\Pi|m^2\log m$, so we can apply the monotonicity of small binomial coefficients in their bottom argument to upper bound Eq.~\eqref{eq:num-adversaries} by
\begin{align}
%
\nonumber
 &\leq \binom{C|\Pi|m^2\log m}{400 \alpha \eps' |\Pi|} \cdot 2^{400 \alpha \eps' |\Pi|}.\\
 &\leq \left(\frac{Ce |\Pi|m^2\log m}{400 \alpha \eps' |\Pi|}\right)^{400 \alpha \eps' |\Pi|} \cdot 2^{400 \alpha \eps' |\Pi|} \nonumber \\
&\leq \exp(O(\eps |\Pi| \log (m/\eps)))\text{,}
\label{eq:num-adversaries-3}
\end{align}
where the second transition is applying the inequality $\binom{n}{k} \leq \left(\frac{ne}{k}
\right)^k$.
%
Now we can use Proposition~\ref{prop:nonobliv-cc-main-prop} to show that the total fraction of random strings that cause the bad event of the statement
for \emph{any} oblivious adversary that makes at most $400 \alpha \eps' |\Pi|$ 
%
is at most
\begin{align}
\nonumber
&\sum_{\Err = 0}^{400 \alpha \eps' |\Pi|} 
 \#\left\langle \parbox[c]{4cm}{\centering oblivious adversaries \\ with exactly $\Err$ errors} \right\rangle \\
&\qquad\qquad
\cdot \Pr [\CC' > 400\alpha|\Pi|m\log m \  \wedge \ \Err \leq \frac{\eps}{\K}\CC] \nonumber \\
&\le\sum_{\Err = 0}^{400 \alpha \eps' |\Pi|} \binom{C|\Pi|m^2\log m}{\Err} \cdot 2^{\Err} \cdot \exp(-\Omega(|\Pi| \log m)) \nonumber \\
&\leq \sum_{\Err = 0}^{400 \alpha \eps' |\Pi|}  \exp(O(\eps |\Pi| \log (m/\eps))) \cdot \exp(-\Omega(|\Pi| \log m)) \nonumber \\
&\leq  \exp(-\Omega(|\Pi| \log m)),
\label{eq:nonobliv-cc-final-1}
\end{align}
where we substitute Eq.~\eqref{eq:num-adversaries-3} for the second transition, and assume a sufficiently small~$\eps$.

Finally, we suppose that $\Err > 400 \alpha \eps' |\Pi|$. Then we again use the inequality $\binom{n}{k} \leq \left(\frac{ne}{k}\right)^k$ and Claim~\ref{claim:num-adversaries} to upper bound the number of oblivious adversaries that make exactly $\Err$ errors by 
\begin{align}
\binom{C|\Pi|m^2\log m}{\Err} \cdot 2^{\Err}  &\leq \left(\frac{C|\Pi|m^2\log m}{\Err}\right)^{\Err} \cdot 2^{\Err} \nonumber \\
&\leq \left(\frac{C|\Pi|m^2\log m}{400 \alpha \eps' |\Pi|}\right)^{\Err} \cdot 2^{\Err} \nonumber \\
&\leq \exp(\Theta(\Err \cdot \log (m/\eps') )).
\label{eq:num-adversaries-4}
\end{align}
Again, we use Proposition~\ref{prop:nonobliv-cc-main-prop} to show that the total fraction of random strings that can allow \emph{any} oblivious adversary that makes more than $400 \alpha \eps' |\Pi|$ errors to satisfy the statement's event,
%
is at most:
\begin{align}
&\sum_{\Err = 400 \alpha \eps' |\Pi|}^{C\eps m|\Pi|}  \#\left\langle \parbox[c]{4cm}{\centering oblivious adversaries \\ with exactly $\Err$ errors} \right\rangle \nonumber
\\ &\qquad\qquad\qquad \cdot \Pr [\CC' > 400\alpha|\Pi|m\log m \  \wedge \ \Err \leq \frac{\eps}{\K}\CC] \nonumber \\
&\sum_{\Err = 400 \alpha \eps' |\Pi|}^{C\eps m|\Pi|} \binom{C|\Pi|m^2\log m}{\Err} \cdot 2^{\Err} \cdot  \exp(-\Omega(\log m \cdot  \Err / \eps)) \nonumber \\
&\leq \sum_{\Err = 400 \alpha \eps' |\Pi|}^{C\eps m|\Pi|} \exp(O(\log (\frac{m}{\eps'})\Err)) \cdot \exp(-\Omega(\log m\cdot \Err / \eps)) \nonumber \\
&\leq \exp(-\Omega(\log m \cdot\Err / \eps)) \text{.}
\label{eq:nonobliv-cc-final-2} 
\end{align}
Finally, putting together Eqs.~\eqref{eq:nonobliv-cc-final-1} and~\eqref{eq:nonobliv-cc-final-2} yields the desired result:  the fraction of random strings that lead \emph{any} additive oblivious adversary to have too much communication, is low. 
In other words, except for this small fraction of \emph{bad randomness strings}, all the other randomness strings are ``good'' for all the oblivious adversaries simultaneously, in the sense that, for any such good randomness, either it is the case that the protocol has small communication or $\Err > \eps \CC/\K$, regardless of the noise pattern.
%
\end{proof}


The above lemma immediately leads to a bound on the communication of the entire protocol as stated by the following corollary.
\begin{corollary}
\label{cor:nonobliv-cc-bound-1}
Assume the setting of Theorem~\ref{thm:nonobliv-adv-no-crs}.
Then, with probability at least $1 - \exp(-\Omega(|\Pi| \log m))$ over the randomness of the parties, 
either $\Err > \tfrac{\eps}{m\log m}\CC$ or 
the communication blowup of \AlgNO is a constant, 
$\CC = O(|\Pi|m\log m) = O(\CC(\Pi))$.
\end{corollary} 
\begin{proof}%
By Claim~\ref{claim:randomness-exchange-comm}, the communication in the randomness exchange phase is $O(|\Pi|\K) = O(|\Pi|m\log m)$, regardless of the randomness of the parties and corruptions. Lemma~\ref{lem:nonobliv-cc-bound-2} additionally bounds the communication in the main part of the protocol by $O(|\Pi| m\log m)$ with probability $1 - \exp(-\Omega(|\Pi|\log m))$ over the randomness of the parties  
and regardless of the specific corruption made by the non-oblivious adversary.
\end{proof}


Now we are ready to finish the proof of Theorem~\ref{thm:nonobliv-adv-no-crs}.



\begin{proof}[Proof of Theorem~\ref{thm:nonobliv-adv-no-crs}]
We have already showed that with high probability over the randomness of the parties,  and regardless of the adversarial sgtrategy, the communication will be only a constant blowup over $\CC(\Pi)$. Specifically, Corollary~\ref{cor:nonobliv-cc-bound-1} tells us that as long as the adversary did no exceed its budget, 
the communication $\CC$ is $O(|\Pi|m\log m)$ with probability at least $1 - \exp(-\Omega(|\Pi| \log m))$. For the remainder of this proof, we work under the assumption that $\CC$ is bounded by this quantity $\CC_{max} = O(|\Pi|m\log m)$. 

First, note that this means that the adversary cannot corrupt any randomness exchange while having error rate $\frac{\eps}{m\log m}$. Indeed, this is because corrupting even a single randomness exchange costs $\Theta(|\Pi|\log m)$ errors, and the maximum number of errors that the adversary can commit while staying under the error rate is $O(\eps |\Pi|)$. Hence, we can work under the assumption that all the parties exchange randomness successfully, and hence $J = |E \setminus E'| = 0$. 

Now, suppose that the communication complexity is $\CC = O(|\Pi|\K)$ and $\Err \leq \frac{\eps}{\K} \CC \leq O(\eps |\Pi|)$. We show that the probability of the number of errors being this small 
%
yet the number of dangerous rounds $D$ being too large, is exponentially small. Specifically, let $k$ be sufficiently large with respect to~$C_6$, to the constant factors in the hash collision probability~$p = O(1/\poly(m))$, and to $\log(1/\eps)$. Then for any \emph{oblivious} adversary that makes at most $\Err$~errors, we have that 
\begin{equation*}
\begin{multlined}
\Pr\left[\left(D > k \cdot \Err\right) \wedge \left(\Err \leq (\eps / \K) \CC \right)\right] \\
\leq \exp(- \Omega(k \cdot \Err \cdot \log m))\text{,}
\end{multlined}
\end{equation*}
by Corollary~\ref{cor:bound-dangerous-obliv-no-crs}. %
Specifically, if we let $\Err_{max} = \frac{\eps}{\K} \CC_{max}$, then this gives us that the probability that, if the adversary commits $\Err \le \Err_{max}$ errors, 
\begin{equation}
\begin{multlined}
\Pr\left[ D > k \cdot \Err_{max} \right] 
\le \Pr\left[ D > k' \cdot \Err \right] 
\\
\leq \exp(- \Omega(k \cdot \Err_{max} \cdot \log m))\text{, }
\end{multlined}
\label{eq:nonobliv-bound-dangerous} 
\end{equation}
by applying Corollary~\ref{cor:bound-dangerous-obliv-no-crs} with $\Err$ and $k'$ such that $k' \cdot \Err = k \cdot \Err_{max}$ (and hence $k' \geq k$ is sufficiently large to apply the corollary). 
Recall that if $\Err=0$, then $D=0$ so the statement holds in this case as well.


Finally, we union bound Eq.~\eqref{eq:nonobliv-bound-dangerous} over all non-oblivious adversaries that make at most $O(\eps |\Pi|)$ errors to show that, with high probability, no non-oblivious adversary can make $D$ larger than $k \cdot \Err_{max}$, with high probability. This probability is at most 
\begin{align*}
&\sum_{\Err = 0}^{\Err_{max}} \binom{C|\Pi|m^2\log m}{\Err} \cdot 2^{\Err} \cdot \Pr\left[(D > k \cdot \Err_{max})
 %
 \right] \\
&\leq \sum_{\Err = 0}^{\Err_{max}} \binom{C|\Pi|m^2\log m}{\Err_{max}} \cdot 2^{\Err_{max}} \cdot \Pr\left[(D > k \cdot \Err_{max}) 
	%
\right] \\
&\leq \sum_{\Err = 0}^{\Err_{max}} \exp(\Theta(\eps |\Pi| \log (m/\eps))) \cdot \exp(- \Omega(k \cdot \eps |\Pi| \cdot \log m)) \\
&\leq  \exp(- \Omega( k \eps |\Pi| \cdot \log m)). \numberthis
\end{align*}
%
The second line follows from the monotonicity of binomial coefficients with the bottom part much smaller than the top. The third line follows from applying the inequality $\binom{n}{d} \leq \left(\frac{ne}{d}\right)^{d}$ and bringing factors of $m$ and $\eps$ into the exponent, and by Eq.~\eqref{eq:nonobliv-bound-dangerous} and plugging in 
$\Err_{max} = \frac{\eps}{\K} \CC_{max} = O(\eps |\Pi|)$. 
The final line follows from taking the hash sizes (which affect the constants in Eq.~\eqref{eq:nonobliv-bound-dangerous}) and $k$ to be large enough with respect to $\log(1/\eps)$.

We conclude that the probability that a non-oblivious adversary can make $D \geq \eps^* |\Pi|$ 
and $\Err \leq O(\eps |\Pi|)$ simultaneously is at most  $\exp(- \Omega(\eps^* |\Pi| \log m))$ over the randomness of the parties, 
where $\eps^*$ is a fixed constant. Specifically, $\eps^*$ is sufficiently larger than $10C_6 \eps \log(1/\eps)$ and is smaller than a sufficiently small constant multiplied by $1/(4000 \cdot (m/K \log(p^{-1})) \cdot C_7 \cdot C_6 \cdot \alpha)$, where we recall that $m/K \log(p^{-1})$ is the constant in the hash collision probability, and $C_6$ and $C_7$ are constants in the potential function $\phi$ from~\cite{GKR-1} (for details on the exact constant, see Theorem~4.1 in~\cite{GKR-1}). 
%
Combining this with Corollary~\ref{cor:nonobliv-cc-bound-1} and using the fact that $D$ upper bounds the number of hash collisions, we conclude that the non-oblivious adversary cannot make $\EHC$ bigger than $O(\eps^* |\Pi|)$ with probability at least $1 -  \exp(- \Omega(\eps^* |\Pi|  \log m))$. Since $\eps^*$ is a constant that does not go to 0 with $\eps$, we can absorb it into the $\Omega$. Hence, we get that the non-oblivious adversary cannot make $\EHC$ bigger than $O(\eps^* |\Pi|)$ with probability at least $1 -  \exp(- \Omega(|\Pi| \log m))$.

Finally, recall that Lemma~\ref{lem:main-communication-old} shows that the potential $\phi$ rises by at least $\K$ in every iteration. This means that after $100|\Pi|$ iterations, the potential is at least $100|\Pi| \K$. Combining this with the fact that $\EHC \leq O(\eps^* |\Pi|)$, Claim~\ref{claim:final-claim} gives us the desired result. For a fuller treatment of this part of the proof, see the proof of %
Theorem~4.1 in~\cite{GKR-1}. %
\end{proof}


==> prelim-ii.tex <==
%
\section{Preliminaries}
\label{sec:preliminaries}

In this section we set some notations and provide lemmas that we will use in Section~\ref{sec:protocol-obliv-no-crs}. 
We begin by establishing notation and basic properties, and then recalling the communication and noise models from~\cite{GKR-1} for the readers' convenience. 
Readers who are familiar with the setup of~\cite{GKR-1} might wish to skip to Section~\ref{sec:prelim-codes}, which introduces preliminaries that are not covered in~\cite{GKR-1}.


\paragraph{Notations and basic properties}
For $n\in \mathbb{N}$ we denote by $[n]$ the set $\{1,2,\dotsc,n\}$. The $\log(\cdot)$ function is taken to base~2.
For a distribution~$D$ we use $x \sim D$ to denote that $x$ is sampled according to the distribution~$D$.
For a finite set~$\Omega$ we let $\Unif_{\Omega}$ be the uniform distribution over~$\Omega$; we commonly omit~$\Omega$ and write $x\sim\Unif$ when the domain is clear from context.
The indicator function $\Ind_{E}$ is defined to be $1$ if and only if the event~$E$ occurs. We usually use it to indicate an equality of values, e.g., $\Ind_{x=y}$, which equals $1$ if and only if $x=y$.

When analyzing coding schemes,
for any variable $var$ that represents the state of some party or a property of the network as a whole, we let $var(i)$ denote the value of the variable $var$ at the beginning of iteration $i$ of that scheme.

%
\begin{definition}
The Hamming distance $\Hamming(\sigma,\sigma')$ of two strings $\sigma=\sigma_1\ldots\sigma_m$ and
$\sigma'=\sigma'_1\ldots\sigma'_m$ of length $m$ over an alphabet $S$,
is the number of positions $i$ such that $\sigma_i \ne \sigma'_i$.
\end{definition}


\paragraph{Multiparty interactive communication model}
We assume an undirected network $G=(V,E)$ of $n=|V|$ parties, $p_1,\ldots, p_n$, and
$|E| = m$ edges, where $p_i$ is connected to $p_j$ if and only if $(p_i,p_j)\in E$.
We identify parties with nodes, and treat $p_i$ and node~$i$ as one.
%
For $v \in V$, let $N(v)$ denote the neighborhood of $v$ in $G$, i.e. $N(v) = \{u: (u,v) \in E \}$.
The network $G$ is assumed to be a connected simple graph (i.e., without self-loops or multi-edges).



The communication model works in synchronous rounds as follows.
At each round, any subset of parties may decide to speak. Each link is allowed to transmit at most one symbol per round in each direction from a constant-sized alphabet~$\Sigma$. We assume throughout this paper that $\Sigma=\{0,1\}$ (both in the noiseless and noisy settings), however, our results extend to a larger alphabet as well.
At each round, a party is allowed to send multiple (possibly different) symbols over multiple links.
A \emph{transmission} over a certain link at a certain round is the event of a party sending a message on this link at that round (if both parties send messages these are two separate transmissions).

We emphasize that, contrary to most previous work, our communication model is not fully-utilized and does not demand all parties to speak at each round on every communication channel connected to them; in fact we don't demand a certain party to speak at all at any given round.

\paragraph{Multiparty protocol}
Each party $p_i$ is given an input $x_i$, and its desire is to output $f_i(x_1,\ldots,x_n)$ for some predefined function~$f_i$ at the end of the process.
Throughout this work we denote the underlying (i.e., noiseless) interactive protocol that the parties are trying to compute by~$\Pi$. A \emph{protocol} $\Pi$ dictates to each party what is the next symbol to send over which channel (if any), as a function of the party's input, the round number, and all the communication that the party has observed so far. After a fixed and predetermined number of rounds, $\RC(\Pi)$, the protocol terminates and each party outputs a value as a function of its input and observed transcript. The quantity $\RC(\Pi)$ is called 
the \emph{length of the protocol} or its \emph{round complexity}.
The communication complexity of the protocol (in bits), denoted by $\CC(\Pi)$, is the total number of transmissions in the protocol times $\log |\Sigma|$. Since we assume $\Sigma=\{0,1\}$, the communication complexity equals the number of transmissions.


We will usually use the notation $|\Pi|$ to denote the length of the (noiseless) protocol \emph{in chunks} rather than in rounds, where a chunk is 
set of contiguous rounds with total communication complexity exactly $5\K$, for $\K$ to be defined later.
Specifically, we keep adding rounds to a chunk until adding a round would cause the communication to exceed~$5\K$. Note that without the last round, the communication in the chunk is at least $5\K - 2m + 1$ bits. 
We can then add a virtual round that makes the communication in the chunk be exactly~$5\K$ bits.
This addition affects the communication complexity by a constant factor. From this point on, we assume that~$\Pi$ adheres to our required structure.

%
We further assume that the noiseless protocol has the property that the speaking order is independent of the inputs that the parties receive. Note that this assumptions restricts generality.
However,  this requirement does not apply on the coding scheme that simulates~$\Pi$ over the noisy network.






\paragraph{Noise model}
We concern ourselves with simulating multiparty interactive protocols $\Pi$ among $n$ parties over a \emph{noisy} network. To do so, we run a different protocol, $\widetilde \Pi$, whose task is to compute the transcript of~$\Pi$ in the noisy network.

A single communication event over a noisy channel with alphabet $\Sigma$ is defined using a symbol from $\Sigma \cup \{ * \} $ that is sent on the channel, where $*$ is a special symbol that means ``no message''.
%
We say that the communication over some link in a given round is \emph{corrupt} (or noisy) if the received symbol~$y$ differs from the sent symbol~$x$. 
Specifically,
if $x,y \in \Sigma$, this event is called a \emph{substitution noise}, if $x=*$ and $y\in \Sigma$ the event is called an \emph{insertion}, and if $x\in \Sigma$ and $y=*$ the event is called a \emph{deletion}. The amount of such events are called the number of errors in the instance.


We stress that the noise may have a crucial effect on the protocol executed by the parties. Not only its correctness may be harmed, but also its  communication may vary. 
However, as mentioned above, we will only consider protocols whose length, $\RC(\widetilde\Pi)$, is fixed for all the instances, that is, independent of the specific noise pattern and parties inputs.
In the noisy setting we redefine~$\CC(\widetilde\Pi)$ to be the communication complexity of a \emph{given instance} of the protocol (which is determined by the inputs, the randomness, and the noise pattern). Note, that $\CC(\widetilde\Pi)$ counts all the transmissions in rounds $\{1,\ldots,\RC(\widetilde\Pi)\}$, i.e., all the communication events in which the sent symbol is not~$*$, which might differ from all the events in which the received symbol is not~$*$, due to insertions and deletions made by the channel. 



The \emph{fraction of noise} observed in a given instance,
is the fraction of corruptions out of all the transmissions in that instance.
For the binary case the noise fraction can be written as,
\[
\mu = \frac{\#\text{errors}}{\CC(\widetilde\Pi)}.
\]
This is also known as \emph{relative} noise~\cite{AGS16}. %



An \emph{oblivious} adversary is an adversary that pre-determines its noise attack, independently of the randomness of the parties.
In this work we focus on a specific oblivious adversary known as \emph{additive}
adversary initially considered by~\cite{BBT60} (see, e.g., \cite{CDFPW08,GS10,GIPST14} for applications resilient against additive adversaries).
%
Assuming a binary alphabet, an oblivious additive adversary fixes a noise pattern $e=\{0,1,2\}^{2|E| \cdot \RC(\widetilde\Pi)}$ that defines the noise per each link in each round of the protocol (note that $\RC(\widetilde\Pi)$ is fixed for all instances). 
In particular, the entry $e_{i,(u,v)}\in \{0,1,2\}$ determines the noise added to the link $u\to v$ in round $i$. 
Assuming $u$ transmits to $v$ in iteration $i$ the message  $t\in\{0,1,2\}$ (where $2$ denotes the case of no message, i.e., $*$), then $v$ receives the transmission~$t+e_{i,(u,v)}\mod 3$.
The number of errors is the number of non-zero entries in~$e$. 

\begin{remark}\label{rem:additive}
We note that \AlgCRS is also robust against an oblivious \emph{fixing} adversary, which fixes the communication that occurs on a link (see~\cite{GKR-1} for a formal definition). 
While the fixing adversary may be more natural, we note that our end-goal in this result is to extend our result to \emph{non-oblivious} adversaries.
To build towards this goal, we find it is more convenient to prove resilience against oblivious additive adversaries.
\end{remark}

\paragraph{Coding scheme---a noise-resilient protocol} 

A coding scheme is a scheme that converts any protocol~$\Pi$ into a noise-resilient protocol~$\widetilde\Pi$ that simulates~$\Pi$ correctly with high probability on any given input.
We say that a protocol $\widetilde \Pi$ simulates~$\Pi$ correctly on a given input if each party can obtain its output corresponding to~$\Pi$ from the transcript it sees when executing $\widetilde \Pi$.
The protocol $\widetilde \Pi$ is said to be resilient to $\mu$-fraction of noise (with probability~$p$),
if for \emph{any} oblivious adversary and any inputs for the parties, the probability of the event that the adversary commits at most $\mu \CC(\widetilde \Pi)$ errors and $\Pi$ is not simulated correctly, is at most~$1-p$.



\subsection{Codes}
\label{sec:prelim-codes}
We use a standard binary error-correction code (see, e.g.,~\cite{Roth06}) with constant rate and constant distance, which has efficient encoding and decoding procedures.
 Such codes can be constructed by concatenating Reed-Solomon codes with binary linear random codes, or by employing the near-linear codes by Guruswami and Indyk~\cite{GI05}.
\begin{theorem}\label{thm:binary-code}
For every $0<\rho<1$ there exists $\delta>0$ such that the following holds for all sufficiently large $n$.
There exists a binary linear code $C : \{0, 1\}^{k} \to \{0, 1\}^n$  with rate $k/n\ge \rho$ and relative distance at least~$\delta$. Furthermore, $C$ can be encoded and decoded from up to $\delta/2$ fraction of bit-flips in polynomial time in~$n$.
\end{theorem}




\subsection{Hash functions, $\delta$-biased strings}
\label{sec:hash}


We use a standard inner-product based hash function. The hash function is seeded with a random string $S$ such that each bit of the output is an inner product between the input and a certain part of $S$ (using independent parts of $S$ for different output bits). Formally,
\begin{definition}[Inner Product Hash Function]
\label{def:ip-hash}
The inner product hash function 
$h: \{0,1\}^* \times \{0,1\}^* \to \{0,1\}^\tau$ 
is defined for any input $x=x_1x_2\ldots$ of length $|x|=L$ and seed~$s=s_1s_2\ldots$ of length $|s|=\tau (L+1)$ (for $\tau \in \mathbb{N}$), as the concatenation of $\tau$ inner products between~$x$ and disjoint parts of~$s$, namely,
for $i\in[\tau]$ let $s^i = s_{(i-1)(L+1)+1} \cdots s_{ i(L+1)-1}$ and set $h^i(x,s) = \langle x, s^i \rangle + s_{i(L+1)}$. Then,
\[
h(x,s) = h^1(x,s) \circ h^2(x,s) \circ \cdots \circ h^{\tau}(x,s) \text{.}
\]
We use the shorthand $h_s(x) \eqdef h(x,s)$.
\end{definition}
We sometimes abuse notation and hash a ternary-string $x$ (or a string over a larger alphabet). In this case, assume we first convert $x$ into a binary string in the natural manner (each symbol separately, using $\lceil \log_2 3\rceil =2$ bits) and then hash the binary string. The seed length should increase appropriately (by at most a constant).

The following is a trivial property of the inner product hash function, stating that, given a uniform seed, the output is also uniformly distributed and that the hash function is strongly 2-universal. See~\cite[Section~15]{MUbook} for a proof.
\begin{lemma}\label{lem:unifHash}
For any $\tau, L \in \mathbb{N}$, $x, y \in \{0,1\}^{L} \setminus \{0\}$ with $x\ne y$, and any $r,v\in\{0,1\}^\tau$
\[
\Pr_{s\sim \Unif} [ h_s(x) = r] = 2^{-\tau} 
\]
and
\[
\Pr_{s\sim \Unif} [ h_s(x) = r \wedge h_s(y)=v] = (2^{-\tau})^2\text{,}
\]
where $\Unif$ is the uniform distribution over $\{0,1\}^{\tau \cdot (L+1)}$.
\end{lemma}
It is easy to see Lemma~\ref{lem:unifHash} also implies that the collision probability (i.e., $\Pr_{s\sim \Unif}[h_s(x)=h_s(y)]$ when $x\ne y$) 
of the inner product hash function with output length $\tau$ is exactly~$2^{-\tau}$.
%
%

Usually, the hash function is seeded with a uniform string. In order to reduce the amount of randomness needed, we use $\delta$-biased random strings, which are close enough to uniform (for our needs), yet can be constructed from much shorter (uniform) seeds, via a result by Naor and Naor~\cite{NN93}.
\begin{definition}[$\delta$-bias]
\label{def:delta-bias}
Fix $\delta > 0$. A distribution $D$ over $\F_2^n$ is $\delta$-biased if for any $v \in \F_2^n \setminus \{ 0^n\}$, we have that
\[ 
\left| \Pr_{x \sim D}\left[ \sum\limits_{i=1}^{n} v_i x_i = 1 \right] - \Pr_{x \sim D}\left[ \sum\limits_{i=1}^{n} v_i x_i = 0 \right] \right| \leq \delta.
\]
\end{definition}

\begin{lemma}[\cite{NN93,AGHP92}]
\label{lem:delta-bias}
%
For any sufficiently large~$n$, generating $n$  $\{0,1\}$-random variables that are $\delta$-biased requires 
$O(\log n + \log 1/\delta)$ uniform bits, and can be done in polylogarithmic time in~$n$ for each random variable.
\end{lemma}

Evaluating the inner-product hash function seeded with a $\delta$-bias string does not change the properties of the hash function. In particular, the inner-product hash function seeded with a $\delta$-biased string has the same collision probability as the inner-product hash function seeded with a random string, up to~$\delta$. 
This holds, to some extent, to multiple inner-products, as shown by the following lemma by Kushilevitz and Mansour~\cite{KM93}.
\begin{lemma}[\cite{KM93}]
\label{lem:biased-hashes-close-to-uniform}
For any $f:\{0,1\}^n\to\{-1,1\}$ that can be described as a decision tree with $m$ nodes, where the branching of every inner node~$v$ depends on the inner-product (mod 2) of the input with a fixed $v \in \F_2^n \setminus \{ 0^n\}$, and for any $\delta$-biased distribution~$D$, 
it holds that
\[
|E_{x\sim D}[f(x)] - E_{x\sim \Unif}[f(x)]| \le \delta m\text{.}
\]
\end{lemma}
\begin{proof}
Follows directly from Lemma~4.5 and Lemma~5.1 in~\cite{KM93}. 
\end{proof}
Note that the function~$f$ in the above Lemma has the range $\{-1,1\}$. For any $g:\{0,1\}^n\to\{0,1\}$ function, the lemma suggest that $|E_{x\sim D}[g(x)] - E_{x\sim \Unif}[g(x)]| \le \tfrac12 \delta m$ by setting $f(x)=2g(x)-1$ and using the linearity of expectations.







==> protocol.tex <==
%
\section{Coding scheme for oblivious adversarial channels}
\label{sec:protocol-obliv-crs}
\subsection{Overview}
\label{sec:protocol-overview}
The high-level description of the simulation is as follows.
The basic mechanism is the rewind-if-error approach from previous works \cite{schulman92,BK12,haeupler14} (see also~\cite{gelles17}). 
In particular, the parties execute the noiseless protocol~$\Pi$ for some rounds and then exchange some information to verify if there were any errors. If everything seems consistent, the simulation proceeds to the next part; otherwise, the parties rewind to a previous (hopefully consistent) point in $\Pi$ and proceed from there.

Note that since multiple parties are involved, it may be that some parties believe the simulation so far is correct while others believe it is not.
Yet, even if one party notices some inconsistency, the entire network should rewind. Hence, we need a mechanism that allows propagating the local view of each party to the entire network.


Our simulation algorithm consists of repeatedly executing the following four phases:
(i) consistency check,
(ii) flag passing,
(iii) simulation,
and (iv) rewind.
The simulation protocol cycles through these four phases in a fixed manner, and each such cycle is referred to as an  {\em iteration}.  Each phase consists of a fixed number of rounds (independent of the parties' inputs and the content of the messages exchanged).  Therefore, there is never an ambiguity as to which phase (and which iteration) is being executed. 
We next describe each phase (not in the order they are preformed in the protocol).



\begin{itemize}
\item [(i)] \textbf{Simulation:}
In this phase the parties simulate \emph{a single chunk} of the protocol $\Pi$. Specifically,
we split $\Pi$ into chunks---consecutive sets of rounds---where at each chunk $5\K$ bits are being communicated, for some $\K \geq m$ that is fixed throughout the simulation 
and such that $\K$ is divisible by $m$.  Jumping ahead, we note that $\K$ is set to be $\Theta(m)$ in the first protocol we construct, that is robust to oblivious adversaries, and is set to $\Theta(m\log m)$ in the final protocol that considers arbitrary (non-oblivious) adversaries.
Note that since the speaking order in~$\Pi$ is fixed and predetermined, the partition into chunks can be done in advance and is independent of the inputs. We assume without loss of generality that each party speaks at least once in each chunk (this is without loss of generality since one can preprocess $\Pi$ to achieve this property while increasing the communication complexity by only a constant factor).

In this phase, the parties ``execute'' the next chunk of $\Pi$, sending and receiving messages as dictated by the protocol~$\Pi$.

This phase \emph{always} takes $5\K$ rounds, which is the maximal number of rounds required to simulate $5\K$ transmissions of~$\Pi$. It may be that the simulation of a specific chunk takes less rounds; in this case, the phase still takes $5\K$ rounds where all the parties remain silent after the chunk's simulation has completed until $5\K$ rounds have passed.


We note that some parties may be aware that the simulation so far contains errors that were not corrected yet (jumping ahead, this information can be obtained via local consistency checks that failed or via the global flag-passing phase, described below).
When we reach the simulation phase, these parties will send a dummy message~$\bot$ to their neighbors and remain silent for $5\K$ rounds until the simulation phase completes.

\item [(ii)] \textbf{Consistency check:}
The main purpose of this phase is to check whether each two \emph{neighboring parties} $u,v\in V$
have consistent transcripts and can continue to simulate, or whether instead they need to correct prior errors.
This phase is based on the \emph{meeting points} mechanism~\cite{schulman92,haeupler14},
which allows the parties to efficiently find the highest chunk number up to which they both agree.

Roughly speaking, every time the parties enter this phase, they exchange a hash of their current transcripts with each other. If the hashes agree, the parties believe that everything is consistent and effectively continue with simulating $\Pi$.
%
If the hashes do not agree, the parties try to figure out the longest point in their transcript where they do agree.
To this end, they send hashes of prefixes of their transcript until the hashes agree. In our setting, each time the parties
enter the ``consistency check'' phase they perform a \emph{single} iteration of the meeting-points mechanism~\cite{haeupler14}, which consists of sending two hash values. If the hashes mismatch, they will send the next two hash values (of some prefixes of the transcript, as instructed by the meeting-points mechanism) \emph{next time they enter the consistency check phase}.\footnote{In addition to exchanging two hash values corresponding to prefixes of the transcript, the parties also exchange a hash indicating how long they have been running the meeting-points mechanism; see Section~\ref{sec:meeting-points} for a full description.}


Note that the above is performed between
each pair of adjacent parties, in parallel over the entire network.

\item [(iii)] \textbf{Flag passing:}
In the flag passing phase, the parties attempt to synchronize whether or not they should continue the simulation of $\Pi$ in the next simulation phase. As mentioned, it may be that some parties believe that the simulation so far is flawless while other may notice that there are some inconsistencies. In this phase the information about (2-party) inconsistencies is propagated to all the parties.

Roughly, if any party believes it shouldn't continue with the simulation, it notifies all its neighbors, which propagate the message to the rest of the network, and no party will simulate in the upcoming simulation phase.
However, if all parties believe everything is consistent then no such message will be sent, and all the parties will continue simulating the next chunk of~$\Pi$.

Technically speaking, the parties accomplish this synchronization step by passing a ``flag'' (i.e., a stop/continue bit) along a spanning tree $\mathcal{T}$ of~$G$. Namely, each party receives flags from each of its children in~$\mathcal{T}$. A party $u$ will receive a bit from each of its children in $\mathcal{T}$. If one of the flags is stop, or if the party sees inconsistency with one of its neighbors, it sends a stop flag to its parent in the tree. Otherwise, it sends its parent the continue flag.
After this phase ends and the root of $\mathcal{T}$ receives all the flags, the root propagates the computed flag in the opposite direction back to the leafs. If there is no channel noise in this phase, it is clear that all parties are synchronized regarding whether the simulation should continue or not (recall that a party sends a dummy message during the simulation phase if its flag is set to stop).


\item [(iv)] \textbf{Rewind:}
In the rewind phase, each party tries to correct any obvious (i.e., length-wise) inconsistencies with their neighbors.
Recall that the meeting-points mechanism allows two neighboring parties to truncate their mis-matching transcripts to a prefix  on which both parties agree. However, this may cause inconsistencies with all their other neighbors.
Indeed, if $u$ and $v$ rewind several chunks off their transcript with each-other, then $u$ must inform any other party $z\in N(u)$ to rewind the same amount of chunks. This rewinding happens \emph{even if the transcripts on the link $(u,z)$ are consistent} at both ends. Therefore, this discrepancy is not necessarily revealed by the meeting-point mechanism between $u$ and $z$, and must be solved in a different manner.


Technically, if  the transcript of $u$ and $v$ consists of $k$ chunks, then
$u$ will send a ``rewind'' message to any neighbor $z$ for which the transcript of $u$ and $z$ contains more than $k$ chunks.
%
However, there are a few caveats. Any party $z$ that is currently trying to find agreement with $u$ via the meeting-points mechanism should not rewind the transcript with~$u$. Intuitively, we can see that any such rewind seems unnecessary, since $z$ is already going to truncate its transcript when it eventually finds agreement with $u$ in the meeting-points subroutine.
Furthermore, an underlying assumption of the meeting-points protocol is that, until the parties decide to truncate their transcripts in the protocol, their transcripts do not change.

Additionally, we restrict each party to rewinding at most one chunk in each of its pairwise transcripts. This is primarily for ease of analysis: it means that no matter what kind of errors the adversary induces, there is only so much harm that can be done during the rewind phase. The upshot of this is that it is not necessarily true that after the rewind phase, $u$ sees exactly the same amount of simulated chunks with all $z\in N(u)$.


Once a party $u$ sends a rewind message to a neighbor $z$, party~$z$ will truncate one chunk of the transcript that corresponds to the link~$(u,z)$, and might then want to send rewind messages to its own neighbors.
These rewinds could trigger more rewinds, leading to a wave of rewinds going through the network.
By providing $n$ rounds in the rewind phase, we make sure that this wave has enough time to go through the entire network.\footnote{Alternatively, we could have fixed the rewind phase to consist of $D$ rounds (rather than~$n$ rounds), where $D$ is the the diameter of the grahp~$G$.} This is critical to guaranteeing that we fix errors quickly enough to simulate $\Pi$ with constant overhead.
\end{itemize}

%

\begin{comment}
\paragraph{Randomness Exchange.}
Our coding scheme is randomized. The only usage of randomness in our scheme is for the consistency check phase, where hash values are exchanged. Since both parties must use the same hash function they must agree on the seed of the hash function, which can be thought of as a random string.  
In the description of the protocol below, we will assume that any pair of neighboring parties share a long random string of polynomial length in the communication of the protocol, and this random string determines the seeds to the hash functions used in the protocol.

In Section~\ref{sec:protocol-obliv-no-crs} we show how to remove the need for a long shared random string.  The basic approach is from previous works~\cite{BK12,haeupler14}:  First make the common randomness short, by having the randomness consist of a (short) seed for $\delta$-biased randomness.  Then, in the protocol, use the $\delta$-bias randomness, as opposed to the true randomness.  Once the random string is short, the parties can simply send it over the network using a standard error-correcting code\footnote{The reason a standard error-correcting code suffices is that this ``randomness sharing'' step of the protocol fully utilizes the network; hence, insertions are nonexistent, and deletions are equivalent to erasures.}, without blowing up the communication complexity by more than a constant factor.

Unfortunately, this approach doesn't work in a straightforward manner.
The reason is that our assumption, that hashes seeded with a $\delta$-biased string behave ``close to'' hashes seeded with a uniform hash, no longer holds when the inputs to the hash depend on the seed itself. Indeed, in our case the inputs depend on which hash collisions occurred in previous rounds, which is a function of the $\delta$-biased string. Showing that replacing a uniform seed with a $\delta$-biased, despite the dependency of the inputs on the seed, is a technicality that is addressed in Section~\ref{sec:protocol-obliv-no-crs}.
\end{comment}




%

\begin{algorithm}[htp]
\caption{A noise-resilient simulation of $\Pi$ (for party $u$)}
\label{alg:robust-protocol}
\begin{algorithmic}[1]
\small
\Statex 
Let $T_{u,v}$ denote the partial, pairwise transcript between $u$ and $v$ \emph{according to $u$}, and let $|T_{u,v}|$ denote the number of \emph{chunks} simulated so far in $T_{u,v}$.
\Statex
\State \Call{InitializeState}{\,}
\Statex
\For{$i=1$ to $100|\Pi|$}
  \ForAll{$v \in N(u)$ in parallel}	  \Comment{\textbf{meeting points}}
    \State $status_{u,v} \gets \Call{MeetingPoints}{u,v, S_{i,u,v}}$
  \EndFor
  \State $minChunk \gets \min_{v \in N(u)} |T_{u,v}|$
  \If{exists $v$ such that $status_{u,v} = \text{``meeting points''}$}
    \State{$status_u \gets 0$}
  \ElsIf{exists $v$ such that $|T_{u,v}| > minChunk$}\label{step:minChunkCheck}
    \State{$status_u \gets 0$}
  \Else
    \State{$status_u \gets 1$}
  \EndIf
  \Statex
  \State $netCorrect_u \gets \Call{FlagPassing}{u, status_u}$  \Comment{\textbf{flag passing}}
  \Statex
  \If{$netCorrect_u = 1$} \Comment{\textbf{simulation}}
    \State Listen for one round. \label{step:listen-bot}
    %
    \State \parbox[t]{0.7\columnwidth}{Simulate chunk $|T_{u,v}|+1$ with each party $v \in N(u)$ from whom we have not received $\perp$ at the first round. The simulation is based on the partial transcript $T_{u,w}$ for each $w \in N(u)$, as well as the input to $u$. \strut \rule[-.4\baselineskip]{0pt}{\baselineskip}}
     \State If the above step took less than $5\K$ rounds, wait until $5\K$ rounds have passed
    \If{received no $\perp$'s in Line~\ref{step:listen-bot} in this iteration}
      \State $minChunk \gets minChunk + 1$
    \EndIf
  \Else
    \State Send a single $\perp$ to each neighbor, and wait $5\K$ rounds.
  \EndIf
  \Statex
  \For{round $r=1$ to $n$} \Comment{\textbf{rewind}}
    \ForAll{$v \in N(u)$ in parallel}
      \If{$status_{u,v} \neq \text{``meeting points''}$ AND $alreadyRewound_{u,v}=0$}
        \If{$|T_{u,v}| > minChunk$} \label{step:truncate}
          \State{Send a rewind message to $v$ and truncate $T_{u,v}$ by one chunk}
          \State{$alreadyRewound_{u,v} \gets 1$}
        \EndIf
      \EndIf
      \If{a rewind message is received from $v$}
        \If{$status_{u,v} \neq$ ``meeting points'' AND $alreadyRewound_{u,v}=0$}
          \State{Truncate $T_{u,v}$ by one chunk}
          \State{$alreadyRewound_{u,v} \gets 1$}
        \EndIf
      \EndIf
    \EndFor
  \EndFor
\EndFor
\end{algorithmic}
\end{algorithm}


%


\begin{algorithm}[htp]
\caption{InitializeState()}
\label{alg:initialize-state}
\begin{algorithmic}[1]
\small
\State $\K \gets m$
\ForAll{neighbors $v \in N(u)$}
  \State Initialize $T_{u,v} = \emptyset$
  \State Initialize $k_{u,v}, E_{u,v}, mpc1_{u,v}, mpc2_{u,v} \gets 0$
  \State $status_{u,v} \gets$ ``simulate''
  \State $alreadyRewound_{u,v} \gets 0$
  \State $S_{u,v} := (S_{i,u,v})_{i \in [100|\Pi|]} \stackrel{\text{unif}}{\gets}  \left(\{ 0,1\}^{\Theta(|\Pi|\K)}\right)^{100|\Pi|}$ uniform bits of randomness.
\EndFor
\State $status_u \gets 1$.
\State $netCorrect_u \gets 1$
\end{algorithmic}
\end{algorithm}


%



\begin{algorithm}[htp]
\caption{FlagPassing($u$, $status$)}
\label{alg:flag-passing}
\begin{algorithmic}[1]
\small
\Statex
 Let $\rho \in V$ be a specific node known by all the parties.
 Let $\mathcal{T}$ be a spanning tree generated by a breadth-first-search starting from $\rho$.
 Denote the depth of $\mathcal{T}$ as $d(\mathcal{T})$, where the depth of a single vertex is~1. Finally, let the \emph{level} of a vertex be defined as $\ell(v) := \ell(u) + 1$, where $u$ is the parent of $v$ in $\mathcal{T}$, and $\ell(\rho) = 1$.

 \Statex
\State $netCorrect \gets status$
\If{$u$ is a leaf in $\mathcal{T}$}
  \State Send $netCorrect$ to parent vertex in $\mathcal{T}$.
  \State Sleep for $\ell(u)-1$ rounds.
\Else
  \State Sleep for $d(\mathcal{T}) - \ell(u)$ rounds. Ignore any messages received in these rounds.
  \State Receive $b_1, \ldots, b_k$, one symbol from each child in $\mathcal{T}$.
  \State $netCorrect \gets \bigwedge\limits_{i=1}^{k} b_i \wedge status$
  \If{$u \neq \rho$}
    \State Send $netCorrect$ to parent.
    \State Sleep for $\ell(u) - 1$ rounds. Ignore any messages received in these rounds.
  \EndIf
\EndIf
\If{$u = \rho$}
  \State Send $netCorrect$ to children.
\Else
  \State Sleep for $\ell(u) - 1$ rounds. Ignore any messages received in these rounds.
  \State Receive $b$ from parent.
  \State $netCorrect \gets b \wedge status$
  \If{$u$ is not a leaf in $\mathcal{T}$}
    \State Send $netCorrect$ to children.
    \State Sleep for $d(\mathcal{T}) - \ell(u)$ rounds. Ignore any messages received in these rounds.
  \EndIf
\EndIf \\
\Return $netCorrect$
\end{algorithmic}
\end{algorithm}


%




\subsection{The coding scheme}
We now formally describe the coding scheme assuming a common random string (CRS) and oblivious noise (Algorithm~\ref{alg:robust-protocol}).
%
Let $\Pi$ be a noiseless protocol over $G=(V,E)$, with $R$ rounds and $C$ transmissions  throughout.
Assume that the communication pattern and amount is predetermined, and independent of parties' inputs and the transcript.
%
Namely, let $T_\Pi = (m_1 m_2 \cdots m_{C})$ be the noiseless transcript of $\Pi$; the content of the messages $m_i$ depend on the specific inputs, however their order, source and destination are fixed for~$\Pi$.

We partition $T_\Pi$ into rounds according to $\Pi$, and group the rounds into \emph{chunks}, where each chunk is a 
set of contiguous rounds with total communication complexity exactly $5\K$.
Specifically, we keep adding rounds to a chunk until adding a round would cause the communication to exceed~$5\K$. Note that without the last round, the communication in the chunk is at least $5\K - 2m + 1$ bits. 
We can then add a virtual round that makes the communication in the chunk be exactly~$5\K$ bits.
This addition affects the communication complexity by a constant factor. From this point on, we assume that~$\Pi$ adheres to our required structure.

We number the chunks in order, starting from 1.
For any (possibly partial) transcript $T$, we let $|T|$ denote the \emph{number of chunks} contained in the transcript~$T$. In particular, $|\Pi|$ is the maximal number of chunks in~$\Pi$.
\label{sec:chunks}  %
%
 We assume without loss of generality that in each chunk, each party sends at least one bit to each of its neighbors (again, this can easily be achieved by pre-processing~$\Pi$ while increasing its communication by a constant factor).  In addition, we assume that the protocol $\Pi$ is padded with enough dummy chunks where parties simply send zeros.  This padding is standard in the literature on interactive coding, and is added to deal with the case that the adversary behaves honestly in all the rounds until the last few rounds, and fully corrupts the last few rounds.

%



The parties simulate $\Pi$ one chunk at a time, by cycling through the following phases in the following order:
consistency check, flag passing, simulation, and rewind.
Each phase takes a number of rounds that is a priori fixed, and since our model is synchronous, the parties are always in agreement regarding which phase is being executed.


Let $T_{u,v}$ denote the pairwise transcript of the link $(u,v)$ as seen by~$u$, where $v \in N(u)$; Similarly,
$T_{v,u}$ is the transcript of the same link as seen by~$v$ (which may differ from $T_{u,v}$ due to channel noise).
In more detail, $T_{u,v}$ is the concatenation of the transcripts generated at each chunk, where the transcript of chunk~$i$
consists of two parts: 
(1) the simulated communication of chunk~$i$, and (2) the chunk number~$i$.\footnote{It is important to add the chunk number since the inner-product hash function we use (Lemma~\ref{def:ip-hash}) has the property that for any string $x$, $h(x)=h(x\circ 0)$.}
The structure of the part (1) is as follows.
Assume that in the $i$-th chunk in $\Pi$,  $j$ bits are exchanged over the $(u,v)$ link in rounds $t_1,\ldots, t_j$.
Then $T_{u,v}$ holds a string of length $j$ over $\{0,1,*\}$ describing the communication
at times $t_1,\ldots, t_j$, \emph{as observed by $u$}. 
The symbol $*$ denotes the event of not receiving a bit at the specific round (i.e., due to a deletion). 
%
The transcript $T_{v,u}$ is defined analogously from $v$'s point of view. 
Note that restricted to the substrings that belongs to chunk~$i$, $T_{u,v}=T_{v,u}$ if and only if there where no errors
at rounds $t_1,\ldots,t_j$ in the simulation phase; insertions and deletions at other rounds are ignored.
%
We abuse notation and define $|T_{u,v}|$ to be the number of \emph{chunks} that appear in~$T_{u,v}$.




\medskip



In Algorithm~\ref{alg:robust-protocol} we describe the noise-resilient protocol for a fixed party $u$.
%
The parties start by initializing their state with a call to InitializeState()  (Algorithm~\ref{alg:initialize-state}).
Much of this state is used for keeping state across iterations of the meeting-points mechanism, described in Algorithm~\ref{alg:meeting-points} (in Appendix~\ref{sec:meeting-points}).







Next, the parties perform a single iteration of the meeting-points mechanism  (Algorithm~\ref{alg:meeting-points}).
%
Given a pair of adjacent parties $u$ and $v$, the meeting-points mechanism outputs a variable $status_{u,v}$, which indicates whether the parties want to simulate (in which case $status_{u,v} = \text{``simulate''}$) or continue with the meeting-points mechanism (in which case $status_{u,v} = \text{``meeting points''}$).

Then, according to the output of the meeting-point mechanism and according to any apparent inconsistencies in the simulated transcripts with its neighbors,
each party sets its ``flag'' $status_u$ to denote whether it should continue with the simulation or not.
This status is used as an input to the flag-passing phase, described in Algorithm~\ref{alg:flag-passing}.
%

Each party ends the flag-passing phase with a flag denoted $netCorrect_u$ that is set to~$1$ if the network as a whole seems to be correct.
Then, the parties perform a simulation phase. If the $netCorrect$ flag is set to~$1$, they execute $\Pi$ for one additional chunk, according to the place they believe they are at. Otherwise, they send a special symbol~$\bot$ to indicate they are not participating in the current  simulation  phase.

Finally, the rewind phase begins, where any party $u$ that sees an obvious discrepancy in the lengths of the transcripts in its neighborhood, sends a single rewind request to any neighbor $v$ which is ahead of the rest, conditioned that $u$ and $v$ are not currently in the middle of a meeting-points process.






==> remove-crs.tex <==
%
\section{A Coding Scheme for Oblivious Noise without Pre-shared Randomness}
\label{sec:protocol-obliv-no-crs}
In this section we modify our protocol from~\cite{GKR-1} to not require a (preshared) common random string (CRS) between the parties. This will involve the parties generating randomness privately and sharing this randomness with their neighbors. 
In this section we will still assume that the adversary is oblivious, which in particular means that the adversary cannot plan his errors after seeing the random strings communicated in the network. 

Let us recall the scheme of~\cite{GKR-1}. As mentioned in Section~\ref{sec:overview-intro}, this protocol works in iterations, where each iteration consists of four phases: (i) consistency check, (ii) flag passing, (iii) simulation, and (iv) rewind. In each consistency check, every two neighboring parties $u$ and $v$ exchange hashes of $T_{u,v}$ (and $T_{v,u}$) to verify that their transcripts so far are consistent. If their hashes are inconsistent, they initiate a meeting points mechanism to find the last point they were in agreement. In addition, in phase (ii), they send a flag to all the parties in the network indicating that the simulation should be temporarily stopped. If their hashes are consistent and they do not receive a flag from other parties, then they simulate in phase (iii).


Note that the pairwise transcripts $T_{u,v}$ are extremely long, potentially $O(|\Pi|\K)$ bits, where $|\Pi|$ denotes the number of chunks in the underlying protocol
and $\K$ is such that the amount of communication in any single chunk is $O(\K)$.
In particular, in our first protocol against oblivious adversaries (\AlgCRS) we set $\K = m$, in our second protocol against 
any (general) adversary we set $\K = m\log m$ (\AlgNO), and in our third protocol (\AlgImpNO, in Appendix~\ref{sec:nonobliv-crs}), we set $\K = m \log\log m$.
This means that 
if we use the inner product hash function of Definition~\ref{def:ip-hash}  and assume a uniformly random seed, the seed's length will be $\Theta(|\Pi|\K)$ bits per output bit. Since the parties do not pre-share randomness, they must communicate these seeds in order to agree on the seeds to be used. However, if they all send each other $|\Pi|$ uniformly random seeds each of length $\Omega(|\Pi|\K)$, this would cost $\Omega(|\Pi|\cdot m \cdot \CC(\Pi))$ in communication throughout the protocol, and the rate of the coding scheme would not be constant.

Our way around this, much like the solution employed by previous work~\cite{GMS11,BK12,haeupler14}, is to use $\delta$-biased seeds for the inner product hash function. Specifically, recall that the lemma of Naor and Naor~\cite{NN93} (Lemma \ref{lem:delta-bias}) states that we can efficiently generate $\delta$-biased distributions over strings of length $\ell$ using just $\Theta(\log(1/\delta) + \log \ell)$ bits of uniform randomness. Hence, the parties can share small amounts of uniform randomness that they will expand to a common $\delta$-biased random seed, which they can then use for the consistency checks.


\subsection{The coding scheme construction}
\label{sec:mod-protocol-oblivious-noCRS}
We now define our first interactive coding scheme, which does not assume a CRS, but does assume that the adversary is oblivious, which we call \emph{\AlgCRS}. This algorithm will be resilient to a fraction $\eps / m$ of (oblivious) adversarial error.

The protocol consists of several parts depicted in Algorithms~\ref{alg:robust-protocol}--\ref{alg:meeting-points}.
In Algorithm~\ref{alg:robust-protocol} we recall the blueprint of the~\cite{GKR-1} scheme. The blueprint of \AlgCRS is identical to~\cite{GKR-1}, the only difference being the implementation of the subroutine InitializeState(), which is replaced with Algorithm~\ref{alg:initialize-state-2}. This new subroutine initiates a randomness exchange routine (Algorithm~\ref{alg:randomness-exchange}), where the parties exchange a small amount of uniform randomness in order to generate a larger (shared) $\delta$-biased seed, which replaces the pre-shared uniform random string assumed in~\cite{GKR-1}.
The other subroutines in \AlgCRS, namely, the flag-passing mechanism (Algorithm~\ref{alg:flag-passing}) and the meeting-points mechanism (Algorithm~\ref{alg:meeting-points}), remain as defined in~\cite{GKR-1}. 
%


\begin{algorithm}[htp]
\caption{A noise-resilient simulation of $\Pi$ (for party $u$) \cite{GKR-1}}
\label{alg:robust-protocol}
\begin{algorithmic}[1]
\small
\Statex 
Let $T_{u,v}$ denote the partial, pairwise transcript between $u$ and $v$ \emph{according to $u$}, and let $|T_{u,v}|$ denote the number of \emph{chunks} simulated so far in $T_{u,v}$. 
Assume the part in $T_{u,v}$ for chunk $i$ consists of the simulated communication of chunk~$i$, and the chunk number~$i$.
\Statex
\State \Call{InitializeState}{\,} 
\Statex
\For{$i=1$ to $100|\Pi|$}
  \ForAll{$v \in N(u)$ in parallel}	  \Comment{\textbf{meeting points}}
    \State $status_{u,v} \gets \Call{MeetingPoints}{u,v, S_{i,u,v}}$
  \EndFor
  \State $minChunk \gets \min_{v \in N(u)} |T_{u,v}|$
  \If{exists $v$ such that $status_{u,v} = \text{``meeting points''}$}
    \State{$status_u \gets 0$}
  \ElsIf{exists $v$ such that $|T_{u,v}| > minChunk$}\label{step:minChunkCheck}
    \State{$status_u \gets 0$}
  \Else
    \State{$status_u \gets 1$}
  \EndIf
  \Statex
  \State $netCorrect_u \gets \Call{FlagPassing}{u, status_u}$  \Comment{\textbf{flag passing}}
  \Statex
  \If{$netCorrect_u = 1$} \Comment{\textbf{simulation}}
    \State Listen for one round. \label{step:listen-bot}
    %
    \State \parbox[t]{0.7\columnwidth}{Simulate chunk $|T_{u,v}|+1$ with each party $v \in N(u)$ from whom we have not received $\perp$ at the first round. The simulation is based on the partial transcript $T_{u,w}$ for each $w \in N(u)$, as well as the input to $u$. \strut \rule[-.4\baselineskip]{0pt}{\baselineskip}}
     \State \parbox[t]{0.7\columnwidth}{If the above step took less than $5\K$ rounds, wait until $5\K$ rounds have passed}\strut
    \If{received no $\perp$'s in Line~\ref{step:listen-bot} in this iteration\strut}
      \State $minChunk \gets minChunk + 1$
    \EndIf
  \Else
    \State Send a single $\perp$ to each neighbor, and wait $5\K$ rounds.
  \EndIf
  \Statex
  \For{round $r=1$ to $n$} \Comment{\textbf{rewind}}
    \ForAll{$v \in N(u)$ in parallel}
      \If{$status_{u,v} \neq $ ``meeting points'' \\ and $alreadyRewound_{u,v}=0$}
        \If{$|T_{u,v}| > minChunk$} \label{step:truncate}
          \State{\parbox[t]{0.7\columnwidth}{Send a rewind message to $v$ and truncate $T_{u,v}$ by one chunk}}
          \State{\strut$minChunk \gets \min_{v\in N(u)} |T_{u,v}|$}
          \State{$alreadyRewound_{u,v} \gets 1$}
        \EndIf
      \EndIf
      \If{a rewind message is received from $v$}
        \If{$status_{u,v} \neq$ ``meeting points'' \\ and  $alreadyRewound_{u,v}=0$}
          \State{Truncate $T_{u,v}$ by one chunk}
          \State{$minChunk \gets \min_{v\in N(u)} |T_{u,v}|$}
          \State{$alreadyRewound_{u,v} \gets 1$}
%
%
%
%
        \EndIf
      \EndIf
    \EndFor
  \EndFor
\EndFor
\end{algorithmic}
\end{algorithm}





\begin{algorithm}[htp]
\caption{InitializeState() \quad   (for party~$u$, simulation against oblivious noise without a CRS)}
\label{alg:initialize-state-2}
\begin{algorithmic}[1]
\small
\State $\K \gets m$
\ForAll{neighbors $v \in N(u)$ in parallel}
  \State Initialize $T_{u,v} = \emptyset$
  \State $status_{u,v} \gets$ ``simulate''
  \State $alreadyRewound_{u,v} \gets 0$
  \State $\delta := 2^{-\Theta(|\Pi|\K/m)}$
  \State $S := (S_{i,u,v})_{i \in [100|\Pi|]} \gets$ RandomnessExchange($u$, $v$, $\delta$, $\K$)
\EndFor
\State $status_u \gets 1$.
\State $netCorrect_u \gets 1$
\end{algorithmic}
\end{algorithm}

The randomness exchange procedure is depicted in Algorithm~\ref{alg:randomness-exchange}.
On every link $(u,v)$, one of the parties $u$ (chosen according to some global total ordering of the parties)
uniformly samples a seed~$L$, encodes it against errors, and sends it to~$v$. Then, both parties expand $L$ to a larger $\delta$-biased string~$S_{u,v}$. Note that $v$ decodes the communication from $u$ and gets a seed $L'$ which may differ from $L$ due to noise. In this case the string $S_{u,v}$ generated by $u$ will differ from $S_{v,u}$ generated by~$v$.
However, we will argue that, with high probability, the adversary will not have enough noise budget to corrupt any~$S_{v,u}$.

\begin{algorithm}[htp]
\caption{RandomnessExchange($u$, $v$, $\delta$, $\K$)}
\label{alg:randomness-exchange}
\begin{algorithmic}[1]
\small
\Statex \textbf{input:} $u$ calling party, $v \in N(u)$. $\delta > 0$ is a parameter that specifies the bias we desire from our random string.
%
%
\Statex
\State Fix an arbitrary total order on the vertices in~$V$ (common for all instantiations of this procedure).
\State $\ell \gets \Theta(|\Pi|\K) \cdot \Theta(\K/m) \cdot 100|\Pi|$
\State $r \gets \Theta(\log(1/\delta) + \log \ell)$, large enough to generate a string of length at least $\ell$ and bias at most $\delta$ via Lemma~\ref{lem:delta-bias}.
\State $C \gets$ error correcting code with block length $\Theta(r)$, constant rate and constant distance  (e.g., the code from Theorem~\ref{thm:binary-code}) \label{alg:CodeRand}
%
\If{$u < v$ in the ordering of~$V$}

\State Sample a uniformly random string $L \in \{0,1\}^{r}$
  \State Send $C(L)$ to $v$
\Else
  \State Receive ${W}$ from $v$
  \State $L \gets C^{-1}(W)$, the decoding of~$W$ with respect to~$C$.
\EndIf
\State $S_{u,v} \gets \left(\{ 0,1\}^{\Theta(|\Pi|\K^2/m)}\right)^{100|\Pi|}$ gets the $\delta$-biased string of length~$\ell$ generated from $L$ by Lemma~\ref{lem:delta-bias}.
\State  \textbf{Output} $S_{u,v}$.
\end{algorithmic}
\end{algorithm}

We note that the randomness exchange uses a standard error correcting code in order to protect the seeds from being shared incorrectly
unless the adversary commits a large number of errors. We do not need an insertion-deletion code because that the rounds where the seeds are shared 
are fully utilized, and so deletions are equivalent to erasures.



We now give the FlagPassing procedure (Algorithm~\ref{alg:flag-passing}), which is identical to the one in~\cite{GKR-1}. This part assumes that all the parties share a spanning tree of the network graph, rooted at some node~$\rho$. If we don't assume that all the parties know the topology of the network, then such a tree can be constructed in a resilient manner using the techniques in~\cite{CGH19}.




%


\begin{algorithm}[htp]
\caption{FlagPassing($u$, $status$) \cite{GKR-1}}
\label{alg:flag-passing}
\begin{algorithmic}[1]
\small
\Statex
Let $\mathcal{T}$ be a spanning tree of~$G=(V,E)$ with a root $\rho\in V$, known to all parties. 
Denote by $d(v)$ the distance (in edges) of $v\in V$ from~$\rho$.  
Let $\depth(\mathcal{T})=\max_v d(v)$ be the depth of $\mathcal{T}$. 


 \Statex
\Statex  // convergecasting the status to the root~$\rho$
\State Wait until round $r= \depth(\mathcal{T})-d(u)+1$  
\State $netCorrect \gets status \wedge \left( \bigwedge_i s_i \right)$, where $\{s_i\}$ are messages received in round $r-1$ from $u$'s children (if any)
\State Send $netCorrect$ to parent


 \Statex
\Statex  // downcasting the result to the entire~$\mathcal{T} $
\State Wait until round $r'=r+2d(u)$
\State $netCorrect \gets status \wedge s_p$, where $s_p $ is the message received in round $r'-1$ from parent (if any)
\State Send $netCorrect$ to children
\Statex
\State \Return $netCorrect$
\end{algorithmic}
\end{algorithm}



%
Finally, we give the MeetingPoints procedure (Algorithm~\ref{alg:meeting-points}), which is also identical to the one in~\cite{GKR-1}. In all variables below, we will drop the subscript of $(u,v)$ but it is implied. Specifically, $k$ below denotes $k_{u,v}$, and the same is true for $E$, $T$, $mpc1$, $mpc2$, and $status$.

\begin{algorithm}[htp]
\caption{{MeetingPoints}($u$,$v$, $S_{i,u,v}$, $\K$) \cite{GKR-1}}
\label{alg:meeting-points}
\begin{algorithmic}[1]
\small
\Statex // Initialization:
  \State Method called by $u$, with $v \in N(u)$. $S_{i,u,v} \in \{ 0,1\}^{\Theta(|\Pi|\K)}$ is a large random seed to be split up and used for hashing. $\Pi \gets$ protocol to be simulated.
  \State $h \gets$ inner product hash family (Definition~\ref{def:ip-hash}) with input length 
  $\Theta(|\Pi|\K)$, collision probability $p= 2^{-\Theta(\K / m)}$ sufficiently small, output length $o = \Theta(\K / m)$, and seed size $s = |S_{i,u,v}|/10$.
  \State $(S_1, S_2, \ldots, S_{10}) \gets S_{i,u,v}$. $S_{i,u,v}$ is split into ten seeds. Without loss of generality we assume that $S_1, \ldots, S_5$ are for the hashes it sends, and $S_6, \ldots, S_{10}$ are for the hashes it uses for comparisons (so $v$ is using $S_6, \ldots S_{10}$ for the hashes it sends, and $S_1, \ldots, S_5$ for comparisons, respectively).
  \State $k,E,mpc1,mpc2 \gets 0$
  
  \Statex
  \Statex // Execute per activation:
  \State $k \gets k+1$
  \State $\widetilde{k} \gets 2^{\lfloor \log k \rfloor}$. Let $c$ be the largest integer such that $c\widetilde{k} \leq |T_{u,v}|$.
  \State $T_1 \gets T_{u,v}[1:c\widetilde{k}], T_2 \gets T_{u,v}[1:(c-1)\widetilde{k}]$
  \State Send $(h_{S_1}(k), h_{S_2}(T_1), h_{S_3}(T_1), h_{S_4}(T_2), h_{S_5}(T_2))$ to neighbor $v$.
  \State \strut $(H_k, H_{T_1}^{(1)}, H_{T_2}^{(1)}, H_{T_1}^{(2)}, H_{T_2}^{(2)}) \gets$ 
  \Statex $\quad (h_{S_6}(k), h_{S_7}(T_1), h_{S_8}(T_2), h_{S_9}(T_1), h_{S_{10}}(T_2))$
  \State Receive $(H_k', H_{T_1}^{(1)'}, H_{T_1}^{(2)'}, H_{T_2}^{(1)'}, H_{T_2}^{(2)'})$ from our neighbor $v$. \label{step:recHash}
  \If {$H_k \neq H_k'$}
    \State {$E \gets E+1$}
  \EndIf
  \If {$k=1, E=0$, and $H_{T_1}^{(1)} = H_{T_1}^{(1)'}$} \label{step:HashesMatch}
    \State {$k \gets 0$}
    \State {$status \gets$ ``simulate''}
    \Return $status$
  \EndIf
  \If {$H_{T_1}^{(1)} = H_{T_1}^{(1)'}$ or $H_{T_1}^{(2)} = H_{T_2}^{(1)'}$}
    \State {$mpc1 \gets mpc1 + 1$}
  \ElsIf {$H_{T_2}^{(1)} = H_{T_1}^{(2)'}$ or $H_{T_2}^{(2)} = H_{T_2}^{(2)'}$}
    \State {$mpc2 \gets mpc2 + 1$}
  \EndIf
  \If {$2E \geq k$}~\label{step:resetMP}
    \State {$k \gets 0, E \gets 0, mpc1 \gets 0, mpc2 \gets 0$}
    \State {$status \gets$ ``meeting points''}
  \ElsIf {$k = \widetilde{k}$}
    \If {$mpc1 > 0.4k$}
      \State {$T \gets T_1$}
      \State {$k \gets 0, E \gets 0$}
    \ElsIf {$mpc2 > 0.4k$}
      \State {$T \gets T_2$}
      \State {$k \gets 0, E \gets 0$}
    \EndIf
    \State {$mpc1 \gets 0, mpc2 \gets 0$}
    \State {$status \gets$ ``meeting points''}
  \Else
    \State {$status \gets$ ``meeting points''}
  \EndIf \\
  \Return $status$
\end{algorithmic}
\end{algorithm}


%
%
%


\subsection{\AlgCRS: Analysis}

We now analyze \AlgCRS and show that for any oblivious adversary that corrupts at most $\eps/m$ fraction of the communication, the parties correctly simulate~$\Pi$ with high probability.

\smallskip
The main  theorem of this section is as follows. Its proof will also be useful in Section~\ref{sec:nonobliv-no-crs}.

\begin{theorem}
\label{thm:oblivious-adv-no-crs}
Assume a network $G=(V,E)$ with $n=|V|$ parties and $m=|E|$ links.
There exists a sufficiently small constant~$\eps>0$ and sufficiently large constant~$c$ such that the following holds.

Suppose $\Pi$ is a multiparty protocol over the network~$G$ with communication complexity $\CC(\Pi)$, binary alphabet and fixed order of speaking; let $|\Pi| = \frac{\CC(\Pi)}{5m}$ 
Consider an instance of \AlgCRS with an oblivious adversary that makes $\Err$ corruptions, 
and let $\CC$ denote the communication complexity of that instance.
Then, the probability that the total number of errors satisfies $\Err \leq \frac{\eps}{m} \cdot \CC$ and yet  \AlgCRS either simulates $\Pi$ incorrectly or has 
%
$\CC > c \cdot \CC(\Pi)$ is at most $\exp(-\Omega(|\Pi|))$. 
\end{theorem}


\subsubsection{Overview}

The analysis we perform resembles the one of the original Algorithm~1, that we analyze in~\cite{GKR-1}.
We start by providing an overview of the parts of our analysis from~\cite{GKR-1} that remain exactly the same; 
for full details, see Sections 4.1--4.3 in~\cite{GKR-1}.

We recall the potential function used to track the progress
of the parties in~\cite{GKR-1}:
\begin{equation}\label{eqn:potential}
\phi \eqdef \sum_{(u,v) \in E} \left( \frac{\K}{m}G_{u,v} - \K \cdot \varphi_{u,v}\right) - C_1 \K B^* + C_7 \K \cdot \EHC,
\end{equation}
where $G_{u,v}$ measures how much party $u$ and $v$ have simulated without error between them (in chunks). 
%
$\varphi_{u,v}$ measures the ``meeting points potential'' between parties $u$ and $v$; intuitively, this 
measures how many iterations parties $u$ and $v$ will need to spend with $status_{u,v} = \text{``Meeting Points''}$ 
(which prevents the rest of the network from simulating). 
%
$B^*$ measures the gap between the \emph{highest} chunk number simulated in the protocol and the 
highest chunk number that the network as a whole has simulated without any errors (this is equal to 
$\min_{u,v} G_{u,v}$). 
%
$\EHC$ measures the number of (adversarial) errors and hash collisions that have occurred so far in the protocol.
%
$C_1,\ldots,C_7$ are constants set in~\cite{GKR-1}.


Analogous to~\cite{GKR-1}, Theorem~\ref{thm:oblivious-adv-no-crs} effectively follows from two lemmas about the potential function $\phi$. The first lemma says that the value of~$\phi$ increases by at least $\Omega(\K)$ in every iteration. This lemma was written for the robust protocol in~\cite{GKR-1}, but does not rely on the implementation of InitializeState(), so it applies to \AlgCRS with an identical proof.
\begin{lemma}[Lemma 4.2 from~\cite{GKR-1}]
\label{lem:main-communication-old}
Fix any iteration of \AlgCRS and let $b$ be the number of links with errors or hash collisions in this iteration. Then the following holds.
\begin{enumerate}
\item The potential $\phi$ increases by at least $\K$ in this iteration.
\item The amount of communication in the entire network during this iteration ($\CC$) satisfies
\( \CC \leq \alpha (1 + b) \K\),
where $\alpha$ is a sufficiently large constant.
\end{enumerate}
\end{lemma}
The second lemma we need bounds the parameter~$\EHC$, that is, bounds the total amount of errors and hash collisions, assuming that the adversary follows its budget.
This lemma is required in order to show that when the potential function is sufficiently large, the protocol has been simulated correctly (i.e., the high potential doesn't stem from high~$\EHC$). 
%
%
Unfortunately, we cannot bound the number of hash collisions the same way we did in~\cite{GKR-1}.
The reason is that we used uniformly random seeds in Algorithm 1 from~\cite{GKR-1}, whereas in \AlgCRS they come from a $\delta$-biased distribution.




We develop a new bound on the hash collisions in this setting by relating the number of hash collisions that occur when the parties share $\delta$-biased seeds to the case where the parties share uniformly random seeds. More specifically, we consider an arbitrary fixed pattern of hash agreements and misses throughout the entire protocol (and throughout the entire network). Fixing the pattern of hash agreements and misses additionally fixes the transcripts throughout the entire protocol, as this is the only randomness in the protocol. This allows us to apply %
Lemma~\ref{lem:biased-hashes-close-to-uniform}
to relate the probability of this pattern of hash agreements and misses when the parties share uniformly random seeds to the corresponding probability of the same pattern with $\delta$-biased seeds. The formal proof is in Sections~\ref{sec:bounding-collisions-delta-bias} and~\ref{sec:bounding-collisions-delta-bias:proof}.

Finally, we will need to establish that the adversary cannot meaningfully corrupt the randomness exchange protocol. That is, the adversary cannot make parties use mis-matching $\delta$-biased strings. Since the adversary has a limited budget of corrupting $\eps/m$-fraction of the communication, the randomness exchange succeeds if the budget does not suffice to corrupt a single coded message (Line~\ref{alg:CodeRand} in Algorithm~\ref{alg:randomness-exchange}).

To this end we need to bound the communication of \AlgCRS, and thus, the budget of the adversary. Note that the communication depends on the randomness exchange, that is, it is possible that corrupting this part and making parties use 
mis-matching $\delta$-biased strings will lead to a large amount of communication, which will allow this corruption. Hence, we need to bound the communication of \AlgCRS \emph{assuming that some of the $\delta$-biased strings are adversarially chosen}. 

We show that despite the fact that the adversary controls some of these seeds, the communication does not increase too much, and the increase is proportional to the number of seeds controlled by the adversary. This bound on the communication effectively bounds the budget of the adversary. By choosing the right parameters, we establish that a noise level of $\eps/m$-fraction of the communication is insufficient to corrupt the $\delta$-biased string of even a single link. The communication-related bounds appear in Section~\ref{sec:noCSR:comm-bound}.

We put the results above together to prove the desired bound on the number of hash collisions in Corollary~\ref{cor:remove-crs-ehc}. We use this to prove Theorem~\ref{thm:oblivious-adv-no-crs} in Section~\ref{sec:thm:oblivious-adv-no-crs:proof}, which follows with a proof identical to that of Theorem 4.1 in~\cite{GKR-1}.

\subsubsection{Bounding hash collisions---Goal and Relevant Notations}
\label{sec:bounding-collisions-delta-bias}


As mentioned in the overview, the adversary has two types of errors it can place: it can use errors to tamper with the randomness exchange phase (and make two adjacent parties fail to share a random seed, by making so many errors that the seed is incorrectly decoded), and it can use errors to corrupt the ``main'' part of \AlgCRS (i.e. after InitializeState() is completed). Let $E'$ be the set of edges on which the parties successfully share $\delta$-biased randomness after InitializeState() is completed; intuitively, only edges in $E'$ can simulate correctly, since edges in $E \setminus E'$ will be comparing hashes computed with different seeds, and will get nonsensical results. We let $\CC$ and $\Err$ denote the \emph{total} amount of communication and number of errors respectively in the entire protocol, and we define $\CC'$ and $\Err'$ be the amount of communication and number of errors during the main part of \AlgCRS. 
Note that while $\CC$ is a random variable, the round complexity $\RC$ of the coding scheme is fixed (given $\Pi$) to be $\Theta(r)=\Theta(|\Pi|K/m)$ rounds in the randomness exchange part and $100|\Pi| \cdot \Theta (K/m + n + 5K + n)$ in the main part. 
The quantity $\Err$ is a then deterministic function of the  
noise-pattern $e \in \{0, 1, 2\}^{2|E|\cdot \RC}$ fixed by the oblivious adversary before the protocol begins.


Our main goal in this section is to bound the number of hash collisions that occur even when the parties use $\delta$-biased randomness. Towards this end, 
we recall the following proposition about $\varphi_{u,v}$ from Appendix A of~\cite{GKR-1}, slightly rephrased.
\begin{proposition}[Proposition A.2 in~\cite{GKR-1}]
\label{prop:phi-nonnegative}
$\varphi_{u,v}(i)$ is non-negative. 
If $\varphi_{u,v}(i)=0$ then $u$ and $v$ have consistent transcripts at the beginning of iteration $i$.
\end{proposition}
%
Note that the other direction does not necessarily hold, i.e., $u$ and $v$ might have consistent views while $\varphi_{u,v}(i)>0$.

\begin{definition}[Dangerous triple]
Given an iteration $i \in [100|\Pi|]$ and an edge $(u,v) \in E$, we say that the triple $(i,u,v)$ is \emph{dangerous} if $\varphi_{u,v}(i) > 0$ and $(u,v) \in E'$. 
\end{definition}
Intuitively, a dangerous triple denotes an iteration $i$ and edge $(u,v) \in E'$ in which the transcripts of $u$ and $v$ differ. 
We let $D$ denote the total number of dangerous triples throughout the execution of~\AlgCRS.

A bound on~$D$ implies a bound on the number of possible hash-collisions (recall, that a hash collision can happen only when the partial transcripts $T_{u,v}$ and $T_{v,u}$ differ, which is indicated by a positive $\varphi_{u,v}(i)$).\footnote{It turns out that $u$ and $v$ can have consistent transcripts while $\varphi_{u,v}(i)>0$; hence, the number of dangerous triples $D$ overcounts the number of potential hash collisions. %
}
%

In~\cite{GKR-1}, we proved that if the parties share a (long) \emph{uniform} random string, then the probability that $D$ is much larger than $\Err'$ is extremely small. However, in this part of the work, the parties instead share a short seed that is locally expanded into a long $\delta$-biased random string via Lemma~\ref{lem:delta-bias}. We need to show that this has no effect on the correctness of the coding scheme.

Below, we state our main lemma of this section, which proves exactly the above. 
Namely, we consider the (bad) event that $D$ is much larger than $\Err'$,
and bound its probability in the $\delta$-biased setting via its probability the uniform randomness setting.

\begin{lemma}
\label{lem:bound-dangerous-obliv-no-crs}
Assume $|\Pi| \K \geq m\log m$. 
Consider an instance of \AlgCRS  and let $p$ denote the collision probability of the inner product hash function used by the protocol under uniformly random seeds.
Suppose the adversary is oblivious, and let $k > 1$ be a real number. 
%
 Then
\[ 
\Pr_S[D > k\cdot \Err' ] \leq e \cdot p^{-O(\Err')} \cdot \Pr_{R}[D > k\cdot \Err']\text{,}
\]
where $S= (S_{i,u,v}, S_{i,v,u})_{i \in [100|\Pi|], (u,v) \in E}$ is the strings shared by each party after Algorithm~\ref{alg:randomness-exchange}, and 
%
where $R = (R_{i,u,v}, R_{i,v,u})_{i \in [100|\Pi|], (u,v) \in E}$ is sampled from a distribution such that
for every $(u,v) \in E'$ the parties share a uniform string, and for any  $(u,v) \not\in E'$
the seeds are sampled identically to the distribution of~$S$ on the corresponding links.
\end{lemma}


In order to use the lemma above in a meaningful way, we need to limit the number of errors $\Err'$ that the adversary can commit in the main part of the protocol. We show below that the ratio of errors to communication within the \emph{main part} of the protocol is always within a constant factor of the ratio of errors to communication in the protocol \emph{overall}. In order to do this, we use Claim~\ref{claim:randomness-exchange-comm} to bound the communication in the randomness exchange phase; we leave the formal statement and simple proof to Section~\ref{sec:noCSR:comm-bound}, where we address the randomness exchange phase in greater detail.
\begin{claim}
\label{claim:effective-noise}
Let $\CC$ be the communication complexity of an execution of \AlgCRS and let $\eps > 0$ be a sufficiently small constant. Assume that $|\Pi|\K \geq m\log m$. If $\Err \leq \frac{\eps}{\K} \cdot \CC$, then $\Err \leq \frac{\eps'}{\K} \cdot \CC'$, where $\eps' = \Theta(\eps)$.
\end{claim}
\begin{proof}
Claim~\ref{claim:randomness-exchange-comm} shows that the communication in the randomness exchange is $\Theta(|\Pi|\K)$ as long as $|\Pi|\K \geq m\log m$. Furthermore, the communication in the main part of the protocol is always at least $\Omega(|\Pi| \K)$: there are $100|\Pi|$ iterations, and the communication in each meeting-points phase is at least $\Theta(\K)$, since the parties pass hashes of size $\Theta(\K/m)$ to each other and there are $m$ links.
\end{proof}
Due to Claim~\ref{claim:effective-noise}, we can consider the main part of the protocol in isolation when bounding the number of dangerous triples, despite the fact that there is extra communication in the randomness exchange phase.


We now make a definition that is critical to our proof of Lemma~\ref{lem:bound-dangerous-obliv-no-crs}.
\begin{definition}[Agreement patterns]\label{def:agreement-pattern}
An agreement pattern $a\in \{0,1\}^{100|\Pi| \cdot (2|E|)}$ consists of a pair of elements $(a_{i,u,v}, a_{i,v,u})$ for each iteration $i \in [100|\Pi|]$ and each edge $(u,v) \in E$, where
 $a_{i,u,v}=1$ if and only if  
 party~$u$ \textbf{believes} that $u$ and $v$ have matching hashes in iteration~$i$.
%
The term $a_{i,v,u}$ is defined analogously.
\end{definition}
Note that $a_{i,u,v}=1$ does not imply that the hashes \emph{actually} match. Indeed, in the presence of channel noise the parties may believe that their hashes match (or mismatch) while the real hashes do not.

To be precise, multiple hashes are passed by $u$ and $v$ in iteration $i$, and an agreement pattern should account for misses/matches in all of them.  To ease the readability of the analysis, we will assume that the parties exchange only \emph{a single} hash, and that they make all their decisions according to whether this hash missed or matched.
This will not affect the validity of the analysis, yet it will somewhat simplify it.
We elaborate on this simplifying assumption in Remark~\ref{rmk:agreements} in the proof of Lemma~\ref{lem:bound-dangerous-obliv-no-crs}.



%

%

Given an agreement pattern $a$, let $a_{u,v} \in \{0,1\}^{200|\Pi|}$ denote the vector 
\[
a_{u,v} \eqdef ((a_{1,u,v}, a_{1,v,u}), \ldots, (a_{100|\Pi|, u, v}, a_{100|\Pi|, v,u})),\]
 which is the pattern of hash misses and matches that both $u$ and $v$ see along a single link $(u,v)$ throughout the protocol. Similarly, let 
 \[
 a_i \eqdef (a_{i, u, v}, a_{i,v,u})_{(u,v) \in E} \in \{ 0,1\}^{2|E|}
 \]
  denote the vector of hash misses and matches for every party and every link in an iteration $i$, and let $a_{\leq i} \eqdef (a_1, \ldots, a_i)$. Call $a_i, a_{u,v}$, and $a_{\leq i}$ \emph{sub-patterns} of~$a$. 

Note that, since we fix the oblivious adversary's errors ahead of time, the agreement pattern $a$ observed in a given instance of \AlgCRS is a function of the random seed $S$ that the algorithm samples. Let $A$ denote the random variable over agreement patterns $a$, where $\Pr_S[A=a]$ 
is the probability, over the random string $S$, %
that the protocol gets agreement pattern $a$, where $S$ is the concatenation of the randomness used by each party for each link. Similar to previous notation, let $A_{i}$ denote the random variable $A$ restricted to sub-patterns $a_{i}$, and $A_{\leq i}$ denote the restriction to sub-patterns $a_{\leq i}$.

\subsubsection{Bounding hash collisions---detailed proof}
\label{sec:bounding-collisions-delta-bias:proof}
In this section, we prove Lemma~\ref{lem:bound-dangerous-obliv-no-crs}. First, we state a simple but vital claim regarding agreement (sub-)patterns.
\begin{claim}
\label{claim:agreement-pattern-transcripts}
Fix the inputs to the protocol and an oblivious adversary, let $i$ be an iteration of \AlgCRS, and fix an agreement sub-pattern $a_{\leq i}$ for the protocol. Then for all $(u,v) \in E$ and all $j = 1, \ldots, i+1$, the partial transcripts $T_{u,v}(j)$ and $T_{v,u}(j)$ are fixed. 
\end{claim}
\begin{proof}
We will prove this by induction on $j$. In fact, we prove something stronger: for every party $u$ and every variable $\var$ that $u$ keeps in its state, $\var(j)$ is fixed.

For $j=1$, it is clear the statement holds, as no communication has happened yet.

Now assume that the claim holds for $j < i+1$. In iteration $j$, the parties exchange hashes of the partial transcripts $T_{u,v}(j)$ and $T_{v,u}(j)$. Since $j \leq i$, we have fixed $a_j$, which means we have already fixed whether or not $u$ and/or $v$ observe hash collisions for \emph{every} pair of adjacent parties $(u,v) \in E$. Noting that the \emph{only randomness in \AlgCRS comes from hashing}, we can conclude that this fixes \emph{every action of each party} in iteration $j$.

Therefore, the values of every state variable (including the partial transcripts $T_{u,v}$ and $T_{v,u}$) at the beginning of iteration $j+1$ are fixed.
\end{proof}
The following corollary follows by taking $i = 100|\Pi|$.
\begin{corollary}
\label{cor:agreements-transcript}
Fix the inputs to the protocol and an oblivious adversary, and fix an agreement pattern $a$. For all $(u,v) \in E$ and all iterations $i$, $T_{u,v}(i)$ and $T_{v,u}(i)$ are fixed.
\end{corollary}
\begin{remark}[Remark on Hash Agreements]
\label{rmk:agreements} 
The situation is actually somewhat more complex than just whether or not the hashes of the transcript $T_{u,v}(i)$ matches the (possibly corrupted) hash of $T_{v,u}(i)$ in iteration $i$. In the meeting-points protocol, the parties send each other \emph{two} hashes of transcripts, one for each of their current ``meeting points.'' Party $u$ compares these two received hashes to her own two hashes, and takes different outcomes depending on how these received hashes match with her hashes. The parties also send each other hashes of their meeting-point iteration $k$, and compare these. Hence, the actions of party $u$ are actually a function of these 5 hash comparisons, and the agreement pattern should be defined over $2^5$-ary symbols rather than bits. For simplicity, we pretend as if the action is a function of just one hash comparison for this proof. This only affects the constant in the exponent of $p$ in Lemma~\ref{lem:bound-dangerous-obliv-no-crs}.
\end{remark}
Now we can prove Lemma~\ref{lem:bound-dangerous-obliv-no-crs}.
\begin{proof}[Proof of Lemma~\ref{lem:bound-dangerous-obliv-no-crs}]
Fix the inputs to the parties and the adversary's errors. By Corollary~\ref{cor:agreements-transcript}, fixing the agreement pattern throughout the entire protocol fixes all the partial transcripts $T_{u,v}(i), T_{v,u}(i)$ for each link $(u,v) \in E$ and iteration $i$. In other words, as long as the agreement pattern for two runs of the \AlgCRS are the same, the actions of the parties in each phase of the two instances are identical as well, \emph{even if} the random seeds sampled in the two runs are different. In other words, every random seed that leads to agreement pattern $a$ \emph{also} leads to the exact same set of pairs of transcripts $\{(T_{u,v}(i), T_{v,u}(i))\}_{i,u,v}$ for every iteration $i$ and edge $(u,v) \in E$. 

We briefly note that it is possible that an agreement pattern $a$ never occurs in \AlgCRS (i.e., $\Pr[A=a] = 0$ for any distribution of randomness). As a simple example,
consider the cases where no noise occurs at all, and yet $a_{i,u,v}=0$ for some $i$ and $(u,v)\in E$. This is obviously impossible since the absence of noise implies that the transcripts at both sides are the same, and hence their hashes must be the same. Since no noise is present, both parties receive the correct hash values and the agreement must be $a_{i,u,v}=1$ in all iterations.

We call an agreement pattern~$a$ \emph{consistent} with respect to a distribution $\mathcal{D}$ if there is some random seed $S \in \text{supp}(\mathcal{D})$ that leads to the agreement pattern $a$. If $a$ is consistent with the uniform distribution, then we simply say $a$ is consistent. Given a consistent agreement pattern $a$, denote the unique set of pairs of transcripts that can coexist with it in the protocol as $\{(T_{u,v}^{(a)}(i), T_{v,u}^{(a)}(i))\}_{i,u,v}$. We have already argued that $a$ can coexist with at most one set of pairs of transcripts, since fixing $a$ fixes the behavior of all the parties in the protocol.

Now we prove the key proposition for this proof, which roughly says that the probability that we see a consistent agreement pattern $a$ in \AlgCRS is equal to the probability of the following event:
\[
h_u(T_{u,v}^{(a)}) = h_v(T_{v,u}^{(a)}) \text{ if and only if }a_{i,u,v}=1 \text{ for all }(i,u,v),
\]
where $h_u$ denotes the hash function that $u$ uses during $i$ with seed $S_{i,u,v}$, $h_v$ denotes the hash function that $v$ uses with seed $S_{i,v,u}$, and $\{(T_{u,v}^{(a)}(i), T_{v,u}^{(a)}(i)\}$ denotes the unique set of pairs of transcripts that is consistent with $a$ given the specific oblivious noise.

This alone is not quite accurate, since $u$'s actions are not determined by whether the hashes of $T_{u,v}^{(a)}$ and $T_{v,u}^{(a)}$ \emph{actually} match, but rather by whether $u$ \emph{thinks} they matched. These two events can be different when the adversary corrupts the hash that $v$ sends to $u$, which is why we defined $a_{i,u,v}$ and $a_{i,v,u}$ separately. Hence, instead of comparing $a_{i,u,v}$ to the event that $h(T_{u,v}^{(a)}(i)) = h(T_{v,u}^{(a)}(i))$, we actually compare $a_{i,u,v}$ to the event that 
$h(T_{u,v}^{(a)}(i)) = \widetilde{h}(T_{v,u}^{(a)}(i))$, where $\widetilde{h}(\cdot)$ is the function that first applies the hash $h$ to the input and then induces errors from the adversary.

For notational convenience, let $Z(S, i, u, v, a)$ denote the event that the hash agreement between $u$ and $v$ in iteration $i$ is consistent with $a$, when seeded by~$S$. Namely, $Z(S, i, u, v, a)$ is the following event
\begin{multline}
\label{eqn:z-def}
Z(S, i, u, v, a) \eqdef \\
\bigg \{
	\left(\mathsf{1}_{h_{S,i,u,v}(T_{u,v}^{(a)}(i)) = \widetilde{h}_{S,i,v,u}(T_{v,u}^{(a)}(i))} = a_{i,u,v}\right) \qquad\quad \\
	\bigwedge 
	\left(\mathsf{1}_{\widetilde{h}_{S,i,u,v}(T_{u,v}^{(a)}(i)) = h_{S,i,v,u}(T_{v,u}^{(a)}(i))} = a_{i,v,u}\right)
\bigg \}\text{,}
\end{multline}
where $h_{S,i,u,v}$ denotes the hash function $h$ used in  \AlgCRS when given the seed $S_{i,u,v}$,  and $\widetilde{h}_{S,i,u,v}(\cdot)$ is defined by applying $h_{S,i,u,v}$ to its input, then modifying the output with the errors that the adversary commits on the transmission from $u$ to $v$ in iteration $i$.

\begin{proposition}
\label{prop:key}
Fix a distribution $\mathcal{D}$ and a consistent agreement pattern $a$ (with respect to the uniform distribution). Fix $\{(T_{u,v}^{(a)}(i), T_{v,u}^{(a)}(i))\}_{i,u,v}$ to the unique transcripts forced in the protocol by fixing~$a$. 
Let $S = ( S_{i,u,v}, S_{i,v,u})_{i \in [100|\Pi|, (u,v) \in E]}$ denote the tuple of random strings used by the main part of the protocol. 
Then,
\begin{equation}
\label{eq:key-prop}
\Pr_{S \sim \mathcal{D}}[A=a] = 
\Pr_{S \sim \mathcal{D}}\left[\bigwedge_{i,u,v} Z(S, i, u, v, a) \right].
\end{equation}
Furthermore, if $a$ is not consistent with $\mathcal{D}$, then Eq.~\eqref{eq:key-prop} is equal to 0.
\end{proposition} 

\begin{proof}
We show that the set~$\mathcal{S}$ of randomly sampled strings that gives rise to the agreement pattern~$a$ in the protocol is the same set of strings that gives rise to $\mathsf{1}_{h_{S,i,u,v}(T_{u,v}^{(a)}(i)) = \widetilde{h}_{S,i,v,u}(T_{v,u}^{(a)}(i))} = a_{i,u,v}$ and $\mathsf{1}_{\widetilde{h}_{S,i,u,v}(T_{u,v}^{(a)}(i)) = h_{S,i,v,u}(T_{v,u}^{(a)}(i))} = a_{i,v,u}$ for all $(i,u,v)$. Therefore, the probability on both sides of Eq.~\eqref{eq:key-prop} is simply the measure of $\mathcal{S}$ under the distribution $\mathcal{D}$, and the result follows as a corollary.

We proceed by induction on $i$, the iteration of the protocol. For $i=1$, note that all pairs of transcripts match at the beginning of the first iteration, as no communication has occurred yet. Hence, the transcripts at the beginning of the protocol between $u$ and $v$ are trivially exactly $T_{u,v}^{(a)}(1)$ and $T_{v,u}^{(a)}(1)$. Hence, $A_{\leq 1} = a_{\leq 1}$ if and only if the strings $S_{1,u,v}, S_{1,v,u}$ used to hash the transcripts in the first iteration satisfy that $\mathsf{1}_{h_{S,1,u,v}(T_{u,v}^{(a)}(1)) = \widetilde{h}_{S,1,v,u}(T_{v,u}^{(a)}(1))} = a_{1,u,v}$ and $\mathsf{1}_{\widetilde{h}_{S,1,u,v}(T_{u,v}^{(a)}(1)) = h_{S,1,v,u}(T_{v,u}^{(a)}(1))} = a_{1,v,u}$ for all $(u,v) \in E$.
I.e.,  
\[
\Pr_{S \sim \mathcal{D}}[A_{\leq 1} = a_{\leq 1}]=\Pr_{S \sim \mathcal{D}}\left[\bigwedge_{(u,v)\in E}Z(S,1,u,v,a)\right].
\] 

Now suppose inductively that the set of random strings $\mathcal{S}_{i-1}$ that lead to $A_{\leq i-1} = a_{\leq i-1}$ is the same as the set of strings that lead to 
\[
\mathsf{1}_{h_{S,j,u,v}(T_{u,v}^{(a)}(j)) = \widetilde{h}_{S,j,v,u}(T_{v,u}^{(a)}(j))} = a_{j,u,v}\] 
and 
\[
\mathsf{1}_{\widetilde{h}_{S,j,u,v}(T_{u,v}^{(a)}(j)) = h_{S,j,v,u}(T_{v,u}^{(a)}(j))} = a_{j,v,u}
\] 
for all $(j,u,v)$ s.t. $j \leq i-1$. Note that, since all $S \in \mathcal{S}_{i-1}$ lead to the same agreement sub-pattern $a_{\leq i-1}$, they also all lead the protocol to the pairs of transcripts $(T_{u,v}^{(a)}(i), T_{v,u}^{(a)}(i))$ at iteration $i$, since fixing the $a_{\leq i-1}$ fixes the behavior of all the parties up until the $i$th iteration of the protocol. Hence, the random strings that lead to $A_{\leq i} = a_{\leq i}$ are precisely the strings in $\mathcal{S}_{i-1}$ that additionally lead to $\mathsf{1}_{h_{S,i,u,v}(T_{u,v}^{(a)}(i)) = \widetilde{h}_{S,i,v,u}(T_{v,u}^{(a)}(i))} = a_{i,u,v}$ and  $\mathsf{1}_{\widetilde{h}_{S,i,u,v}(T_{u,v}^{(a)}(i)) = h_{S,i,v,u}(T_{v,u}^{(a)}(i))} = a_{i,v,u}$ for all $(u,v)$. 

Applying the inductive hypothesis, $\mathcal{S}_{i-1}$ is exactly the set of strings that lead to \\$\mathsf{1}_{h_{S,j,u,v}(T_{u,v}^{(a)}(j)) = \widetilde{h}_{S,j,v,u}(T_{v,u}^{(a)}(j))} = a_{j,u,v}$ and $\mathsf{1}_{\widetilde{h}_{S,j,u,v}(T_{u,v}^{(a)}(j)) = h_{S,j,v,u}(T_{v,u}^{(a)}(j))} = a_{j,v,u}$ for all $(u,v) \in E$ and all $j \leq i-1$. Hence we conclude that the the set of strings that lead to $A_{\leq i} = a_{\leq i}$ is the same as the set of strings that lead to $\mathsf{1}_{h_{S,i,u,v}(T_{u,v}^{(a)}(i)) = \widetilde{h}_{S,i,v,u}(T_{v,u}^{(a)}(i))} = a_{i,u,v}$ and  $\mathsf{1}_{\widetilde{h}_{S,i,u,v}(T_{u,v}^{(a)}(i)) = h_{S,i,v,u}(T_{v,u}^{(a)}(i))} = a_{i,v,u}$ for all $(u,v)$ and $j \leq i$.

Finally, the last claim of the Proposition follows trivially, since if $a$ is not consistent with $\mathcal{D}$, then no $S\in \text{supp}(\mathcal{D})$ leads to~$a$, and we have $\Pr_{S \sim \mathcal{D}}[A=a] = 0$ by definition.
\end{proof}

Now we can bound the probability of getting too many dangerous triples with $\delta$-biased randomness from the randomness exchange (Algorithm~\ref{alg:randomness-exchange}) in terms of the probability of getting too many dangerous triples with uniform randomness. Recall that, after fixing a consistent agreement pattern~$a$, there is exactly one possible setting to all pairs of transcripts $(T_{u,v}(i), T_{v,u}(i))$ for each link and iteration that complies with this agreement pattern. Given such a setting of pairs of transcripts, it is easy to read off an upper bound on the number of dangerous triples, since in every dangerous triple $(i,u,v)$, we have that $T_{u,v}(i) \neq T_{v,u}(i)$ and $(u,v) \in E'$. 
Recall that we are interested in the probability there where more than $k\Err'$ dangerous triples, where $k$ is a real number given by the lemma's statement.
\begin{definition}
A consistent agreement pattern $a$ is called  \emph{bad} if it leads to having more than $k \Err'$ dangerous triples in the considered instance. 
\end{definition}
We let $\Bad = \{ a\in \{0,1\}^{100|\Pi| \cdot (2|E|)} \mid a \text{ is bad and consistent}\}$ be the set of all bad consistent agreement patterns (given the fixed inputs, fixed error pattern, and $k$). 
Then, for any distribution~$D$ we can write
\begin{equation}
\Pr_{S \sim \mathcal{D}}[D > k \Err'] = \sum_{a \in \Bad} \Pr_{S \sim \mathcal{D}}[A=a]. 
\end{equation}
Hence, to prove Lemma~\ref{lem:bound-dangerous-obliv-no-crs}, it suffices to show that
\begin{equation}
\label{eqn:sum-patterns-1}
\sum_{a \in \Bad} \Pr_{S \sim \mathcal{D}_S}[A=a] \leq e \cdot p^{-4\Err'} \cdot \sum_{a \in \Bad} \Pr_{R \sim \mathcal{D}_R}[A=a]\text{,}
\end{equation}
where we recall that $\mathcal{D}_S$ is the distribution where the $\{S_{u,v}\}$ are drawn i.i.d from a $\delta$-biased distribution for $(u,v) \in E'$ 
%
while for $(u,v) \in E \setminus E'$ the string $\{S_{u,v}, S_{v,u}\}$ are adversarially chosen by the fixed noise. The distribution $\mathcal{D}_R$ is the same for $(u,v) \in E \setminus E'$ and uniform for $(u,v) \in E'$, as described in the statement of the lemma. 

Since $\Pr_{R\sim\mathcal{D}_R}[A=a] = 0$ for any agreement pattern $a$ that is not consistent w.r.t $\mathcal{D}_R$, we can sum the right-hand side Eq.~\eqref{eqn:sum-patterns-1} only over $a$'s that are bad and consistent w.r.t $\mathcal{D}_R$. Denote these by the set 
\[
\Bad_{\mathcal{D}_R} = \{ a \mid a\in \Bad \text{ and is consistent with respect to } \mathcal{D}_R\}.
\]
Noting that the uniform distribution trivially contains the support of $\mathcal{D}_R$, which  itself contains the support of $\mathcal{D}_S$, Proving Eq.~\eqref{eqn:sum-patterns-1} amounts to proving
\begin{align}
%
\sum_{a \in \Bad_{\mathcal{D}_R}} \Pr_{S \sim \mathcal{D}_S}[A=a] 
\leq e \cdot p^{-4\Err'} 
\cdot 
\sum_{a \in \Bad_{\mathcal{D}_R}} \Pr_{R \sim \mathcal{D}_R}[A=a]\text{.}
\label{eqn:sum-patterns-2}
\end{align}


For ease of notation in the proof below, let $Q(a)$ denote the probability of seeing the agreement sub-pattern $a_{u,v}$ for all $(u,v) \in E \setminus E'$. Formally,

\begin{equation}
\label{eqn:q-def}
Q(a) \eqdef \Pr_{S \sim \mathcal{D}_S}\left[\bigwedge_{i,(u,v) \in E \setminus E'} Z(S, i, u, v, a)\right]\text{,}
\end{equation}
where the events $Z(S,i,u,v,a)$ are as defined in Eq.~\eqref{eqn:z-def}.

%
We upper bound the left-hand side of Eq.~\eqref{eqn:sum-patterns-2}, as depicted in Eq.~\eqref{eq:delta-bias-simplification-1}.
%
%
%
%
%
\begin{figure*}[!t]
\begin{align}
 &\sum_{a \in \Bad_{\mathcal{D}_R}} \Pr_{S \sim \mathcal{D}_S}[A=a] \nonumber\\
 &=  \sum_{a \in \Bad_{\mathcal{D}_R}} \Pr_{S \sim \mathcal{D}_S}\left[\bigwedge_{i,(u,v) \in E} Z(S, i, u, v, a) \right] \nonumber \\
&= \sum_{a \in \Bad_{\mathcal{D}_R}} \left(\prod_{(u,v) \in E'}\Pr_{S \sim \mathcal{D}_S}\left[\bigwedge_{i} Z(S, i, u, v, a)\right]\right) \cdot Q(a) 
%
 \label{eq:delta-bias-simplification-1}
 \\
&\leq  \sum_{a \in \Bad_{\mathcal{D}_R}} \left(\prod_{(u,v) \in E'}\Pr_{S \sim \mathcal{D}_S}\left[\bigwedge_{i:\text{no err on $(i,u,v)$}} Z(S, i, u, v, a)\right]\right) \cdot Q(a) \nonumber \\
&=  \sum_{a \in \Bad_{\mathcal{D}_R}} \left(\prod_{(u,v) \in E'}\Pr_{S \sim \mathcal{D}_S}\left[\bigwedge_{i:\text{no err on $(i,u,v)$}} \mathsf{1}_{h_{S,i,u,v}(T_{u,v}^{(a)}(i)) = h_{S,i,u,v}(T_{v,u}^{(a)}(i))} = a_{i,u,v}\right]\right) \cdot Q(a)
\nonumber
\end{align}
%
\hrulefill
%
\vspace*{4pt}
\end{figure*}
%
The first equality is Proposition~\ref{prop:key}. 
%
The second equality is due to the fact that, given a specific~$a$ and fixing the adversary's errors, the event $\bigwedge_{i} Z(S, i, u, v, a)$ for $(u,v) \in E'$ is independent from $\bigwedge_{i} Z(S, i, u', v', a)$ for all $(u',v') \in E$ such that $(u',v') \neq (u,v)$, since $S_{u,v}$ is sampled independently from $S_{u', v'}$.
To elaborate, since $a$ is fixed, all the transcripts $\{T^{(a)}_{u,v}(i)\}$ are fixed as well (Claim~\ref{claim:agreement-pattern-transcripts}), and since the channel's noise is fixed we get that, 
for any $(i',u',v')$, the event $Z(S, i', u', v', a)$ depends only on the seed $S_{u',v'}$.
 

The inequality in the third line follows from the fact that the event $\bigwedge_{i:\text{no err on $(i,u,v)$}} Z(S, i, u, v, a)$ contains the event $\bigwedge_{i} Z(S, i, u, v, a)$, since we perform AND over fewer random variables. Note that, by $i:\text{no err on $(i,u,v)$}$, we mean that there is no adversarial error between $u$ and $v$ in the entire iteration~$i$. 

The last equality follows from the following facts: (1) the parties successfully share a seed on the edges in $E'$, so $S_{i,u,v} = S_{i,v,u}$ for all $(u,v) \in E'$, (2) $h_{S,i,u,v} = \widetilde{h}_{S,i,u,v}$ and there is no adversarial error between $u$ and $v$ in iteration $i$, and (3) $a_{i,u,v} = a_{i,v,u}$ when $a$ is consistent and there is no error on $(i,u,v)$, because the hashes are transmitted properly, and so either $u$ and $v$ will both have a hash match or both have a hash miss, and so if $a_{i,u,v} \neq a_{i,v,u}$ then $a$ would not be consistent. 

Now we can apply Lemma~\ref{lem:biased-hashes-close-to-uniform} to the right-hand side of Eq.~\eqref{eq:delta-bias-simplification-1}. Note that 
\begin{equation}
 \bigwedge_{i:\text{no err on $(i,u,v)$}} \mathsf{1}_{h_{S,i,u,v}(T_{u,v}^{(a)}(i)) = h_{S,i,u,v}(T_{v,u}^{(a)}(i))} = a_{i,u,v} 
\label{eqn:event:i-no-err}
\end{equation}
is an event about a sequence of hash misses and matches on a fixed input when using a seed that is chopped up from a string $S_{u,v}$ sampled from a $\delta$-biased source. 
For a single iteration~$i$, the equality or inequality of $h_{S,i,u,v}(T_{u,v}^{(a)}(i))$ and $h_{S,i,u,v}(T_{v,u}^{(a)}(i))$
can be decided by a decision tree (according to the their definition in Lemma~\ref{lem:biased-hashes-close-to-uniform}) of size $\Theta(K/m)$. 
%
It is easy to verify that, for inner-product hash~$h$ with output size~$\Theta(K/m)$ and any~$g$, 
deciding the conjunction $(h(x)=h(y)) \wedge g(z)$ requires $O(K/m + \mathsf{Tree}(g))$ nodes, where $\mathsf{Tree}(g)$ is size of the decision tree for~$g$. 
Yet, the number of nodes required for a decision tree for  
$(h(x) \ne h(y)) \wedge g(z)$ is $O( (\mathsf{Tree}(g)+1) \cdot K/m)$. 
Putting these two together, the size of a decision tree for the event in Eq.~\eqref{eqn:event:i-no-err} is bounded by $(c K/m)^{100|\Pi|}$ for some constant $c\ge 1$, since it is a conjunction of size at most $100|\Pi|$ of functions of the form $(h(x) \ne h(y))$ or $(h(x) = h(y))$.


With the above observation, Lemma~\ref{lem:biased-hashes-close-to-uniform} gives that
the probability of the event in Eq.~\eqref{eqn:event:i-no-err} 
does not differ by much from the probability of the same event given the seed is uniform.
\begin{align*}
&\left |\Pr_{S \sim \mathcal{D}_S} \left[ \bigwedge_{\substack{i:\\ \text{no err on} \\ (i,u,v)}} \!\!\! \mathsf{1}_{h_{S,i,u,v}(T_{u,v}^{(a)}(i)) = h_{S,i,u,v}(T_{v,u}^{(a)}(i))} = a_{i,u,v} \right ] \right. 
\\ 
&\left.
\quad - \Pr_{R \sim \mathcal{D}_R} \left [ \bigwedge_{\substack{i:\\ \text{no err on} \\ (i,u,v)}} \!\!\! \mathsf{1}_{h_{R,i,u,v}(T_{u,v}^{(a)}(i)) = h_{R,i,u,v}(T_{v,u}^{(a)}(i))} = a_{i,u,v} \right ] \right |
\\
& \le \tfrac12 \delta (cK/m)^{100|\Pi|}\text{.}
\end{align*}


This allows us to bound the right-hand side of Eq.~\eqref{eq:delta-bias-simplification-1} by 
Eq.~\eqref{eq:delta-bias-simplification-2}
\begin{figure*}
\begin{align}
\nonumber
&\leq \sum_{a \in \Bad_{\mathcal{D}_R}} \left(\prod_{(u,v) \in E'}
\left(\Pr_{R \sim \mathcal{D}_R}\left[\bigwedge_{i:\text{no err on $(i,u,v)$}} \mathsf{1}_{h_{R,i,u,v}(T_{u,v}^{(a)}(i)) = h_{R,i,u,v}(T_{v,u}^{(a)}(i))} = a_{i,u,v}\right] 
	+ \delta (cK/m)^{100|\Pi|} \right)\right) \cdot Q(a) 
\\
&=  \sum_{a \in \Bad_{\mathcal{D}_R}} \left(\prod_{(u,v) \in E'}\left(\Pr_{R \sim\Unif}\left[\bigwedge_{i:\text{no err on $(i,u,v)$}} Z(R, i, u, v, a)\right] +\delta (cK/m)^{100|\Pi|} \right)\right) \cdot Q(a)\label{eq:delta-bias-simplification-2}
\end{align} 
%
\hrulefill
%
\vspace*{4pt}
\end{figure*}
where we use the definition of $Z(R, i, u, v, a)$ to avoid cumbersome notation. Note that in the last transition we replaced the distribution $\mathcal{D}_R$ with a uniform distribution~$\Unif$. This follows since, by the definition of $\mathcal{D}_R$, each of the seeds $R_{i,u,v}$ with $(u,v) \in E'$ is uniform and independent.



%
\begin{figure*}[!b]
%
\hrulefill
%
\vspace*{4pt}
%
\begin{align} 
%
&\leq  \sum_{a \in \Bad_{\mathcal{D}_R}} \prod_{(u,v) \in E'}\left(\left(1+2^{-|\Pi| \K / m}\right) \cdot \Pr_{R_{u,v} \sim \Unif}\left[\bigwedge_{i: \text{no err in $(u,v)$)}} Z(R,i,u,v,a)\right]\right) \cdot Q(a) \nonumber \\
&\leq  \left(1+2^{-|\Pi| \K / m}\right)^m \sum_{a \in \Bad_{\mathcal{D}_R}} \prod_{(u,v) \in E'}\left(\Pr_{R_{u,v} \sim \Unif}\left[\bigwedge_{\text{$i$: no err on $(i,u,v)$}}  Z(R, i, u, v, a) \right]\right) \cdot Q(a) 
%
\label{eq:delta-bias-simplification-3}
%
 \\
&\leq e \cdot \sum_{a \in \Bad_{\mathcal{D}_R}} \prod_{(u,v) \in E'}\left(\Pr_{R_{u,v} \sim \Unif}\left[\bigwedge_{\text{$i$: no err on $(i,u,v)$}}  Z(R, i, u, v, a) \right]\right) \cdot Q(a) \nonumber
\end{align}
\end{figure*}



We now wish to bound $\delta$ as a fraction of the probability of the event in Eq.~\eqref{eqn:event:i-no-err}.
\begin{claim} 
\label{clm:eq:delta-small}
We have that,
\(
\delta (cK/m)^{100|\Pi|} 
\leq 2^{-|\Pi| \K / m}  \times \min_{a_{u,v}: (u,v) \in E'}\Pr_{R_{u,v} \sim \Unif}\left[\bigwedge_{\text{$i$:no err on $(i,u,v)$}}  Z(R, i, u, v, a)\right].
\)
%
%
%
%
%
%
%
%
\end{claim}
\begin{proof}
Recall that, given a uniform seed, the hash collision probability is exactly $p = 2^{-\Theta(\K / m)}$ (Lemma~\ref{lem:unifHash}). 
Note that in the event of Eq.~\eqref{eqn:event:i-no-err}
%
we are AND-ing over at most $100|\Pi|$ iterations~$i$,
In each iteration $i$, since we use a uniform seed, the probability of $Z(R, i, u, v, a)$ on iterations $i$ with no error conditioned on the previous outcomes is at least $p$. To see this, note that the transcripts either agree or disagree. If the transcripts agree, then since $a$ is consistent, the probability is~$1$. If the transcripts disagree, then with probability~$p$ there is a collision, and with probability $1-p > p$ there is not. 
%
We can therefore write,
\begin{align*}
&\min_{a, (u,v) \in E'}\Pr_{R_{u,v} \sim \Unif}\left[\bigwedge_{\text{$i$:no err on $(i,u,v)$}} Z(R, i, u, v, a)\right] \\
&= \min_{a, (u,v) \in E'}\prod_{\text{$i$:no err on $(i,u,v)$}}\Pr_{R_{u,v} \sim \Unif}[Z(R, i, u, v, a)] \\
&\ge  p^{100|\Pi|} \\
&= 2^{-\Theta(|\Pi| \cdot \K/m)}.
\end{align*}
%
The claim now holds
 by recalling that $\delta =  2^{-\Theta(|\Pi| \cdot \K/m)}$, hence,
\(
\delta (cK/m)^{100|\Pi|} = 2^{-\Theta(|\Pi| \cdot \K/m)} 2^{O(|\Pi|\log (K/m))},
\)
 and taking the constant in the exponent of $\delta$ to be sufficiently large.
\end{proof}




%
With Claim~\ref{clm:eq:delta-small},
Eq.~\eqref{eq:delta-bias-simplification-2} can be now bounded, as depicted in  Eq.~\eqref{eq:delta-bias-simplification-3},
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
where in the last transition, we use the fact that $|\Pi|\K \geq m\log m$ to conclude that $(1+2^{-|\Pi| \K / m})^m \leq (1+\frac{1}{m})^m \le e$. 

We are almost done: if Eq.~\eqref{eq:delta-bias-simplification-3} had an AND over \emph{all} iterations $i$ instead of just the iterations with no error, we would be able to apply Proposition~\ref{prop:key} on this term to finish the proof of Lemma~\ref{lem:bound-dangerous-obliv-no-crs}. 
Note that
\begin{align*}
&\sum_{a \in \Bad_{\mathcal{D}_R}} \Pr_{R}[A=a] 
=  \sum_{a \in \Bad_{\mathcal{D}_R}} \Pr_R\left[\bigwedge_{i,(u,v) \in E} Z(R, i, u, v, a) \right] \displaybreak \\
&= \sum_{a \in \Bad_{\mathcal{D}_R}} \prod_{(u,v) \in E'}\Pr_{R_{u,v} \sim \Unif}\left[\bigwedge_{\text{$i$:no err on $(i,u,v)$}} \!\!\!\!\!  Z(R, i, u, v, a) \right] 
\\
&\qquad\qquad\qquad\qquad
 \times \Pr_{R_{u,v} \sim \Unif}\left[\bigwedge_{\text{$i$:err on $(i,u,v)$}} \!\!\! Z(R, i, u, v, a) \right] \\
 &\qquad\qquad\qquad\qquad
 \times Q(a)\text{.}
\end{align*}
where we use Proposition~\ref{prop:key} in the first transition and the fact that the $R_{i,u,v}$ are independently sampled uniform strings when $(u,v) \in E'$ in the second.

The extra term can be lower bounded as follows.
\begin{claim}\label{clm:LB:ierr}
For any $a\in \Bad_{\mathcal{D}_R}$,
\begin{equation}
 \prod_{(u,v) \in E'}\left(\Pr_{R_{u,v} \sim \Unif}\left[\bigwedge_{\text{$i$:err on $(i,u,v)$}}  Z(R, i, u, v, a) \right]\right) 
 \ge 
 p^{4\Err'}.
\label{eqn:i-err}
\end{equation}
\end{claim}
\begin{proof}
First, we recall that edges in $E'$ have the property that the parties share their random string correctly - hence, we have $R_{i,u,v} = R_{i,v,u}$ for all $(u,v) \in E'$ and iterations $i$.



We split $Z$ into two subevents $Z_1$ and $Z_2$ in the natural way, such that $Z = Z_1 \wedge Z_2$. Formally:
\begin{align}
\label{con:1}
&Z_1(R, i, u, v, a) \eqdef 
\big \{ \mathsf{1}_{h_{R,i,u,v}(T_{u,v}^{(a)}(i)) = \widetilde{h}_{R,i,u,v}(T_{v,u}^{(a)}(i))} = a_{i,u,v} \big \}  
\intertext{and} 
&Z_2(R, i, u, v, a) \eqdef 
\big \{ \mathsf{1}_{\widetilde{h}_{R,i,u,v}(T_{u,v}^{(a)}(i)) = h_{R,i,u,v}(T_{v,u}^{(a)}(i))} = a_{i,v,u} \big \},
\label{con:2}
\end{align}
where we also used the fact that $R_{i,u,v} = R_{i,v,u}$ in the above definitions. 


Since $a$ is consistent with respect to $\mathcal{D}_R$,  that is, $\Pr[A=a]>0$, then 
by Proposition~\ref{prop:key} there must exist $R^*$ such that 
$\bigwedge_{i,u,v} Z(R^*, i, u, v, a)$ holds. In other words, for this specific~$R^*$,
we have that for all $(i,u,v)$ such that $(u,v) \in E'$ and iteration~$i$, we have that $Z_1(R^*, i, u, v, a) = Z_2(R^*, i, u, v, a) = 1$. 
If $o_1$ and $o_2$ are the hash outputs on the link $(u,v)$ in iteration $i$ with randomness $R^*$ (i.e. $o_1 = h_{R^*,i,u,v}(T_{u,v}^{(a)})$ and $o_2 = h_{R^*,i,u,v}(T_{v,u}^{(a)})$), then if $a_{i,u,v}=1$, the noise exactly makes $\widetilde{h}_{R,i,u,v}(T_{v,u}^{(a)}(i))=o_1$, and otherwise it does not. Similarly, if $a_{i,v,u}=1$ then the noise makes $\widetilde{h}_{R,i,u,v}(T_{u,v}^{(a)}(i))=o_2$, and otherwise it does not. We will say that $o_1$ and $o_2$ make the event $Z$ (resp. $Z_1, Z_2$) \emph{occur}, when the iteration $i$, link $(u,v)$, and agreement pattern $a$ are understood from context.

Fix an iteration $i$, link $(u,v)$, and agreement pattern $a$. Assume $T_{u,v}^{(a)}=T_{v,u}^{(a)}$. Then, if there is no noise in the message $h_{R,i,u,v}(T_{v,u}^{(a)}(i))$ it must be that $a_{i,u,v}=1$, since we know that the hashes will match even if the random string used were $R_{i,u,v} = R^*_{i,u,v}$. In fact, \emph{any} seed $R_{i,u,v}$ makes the hashes match, and so since $a_{i,u,v} = 1$, we conclude that $\Pr_R[Z_1(R,i,u,v,a)]=1$. 

If there is noise in that message, then it must be that $a_{i,u,v}=0$ since for any seed $R_{i,u,v}$ (including $R^*_{i,u,v}$), the hashes will not match, since they matched before the noise and the noise makes one of the messages different. Once again, since this holds for all possible random strings $R_{i,u,v}$, we have that $\Pr_R[Z_1(R,i,u,v,a)]=1$ holds for this case as well.

Now assume that $T_{u,v}^{(a)} \ne T_{v,u}^{(a)}$. Furthermore, assume there is no noise in the message $h_{R,i,u,v}(T_{v,u}^{(a)}(i))$. If $a_{i,u,v}=1$, then, any seed~$R$ that causes a collision makes $Z_1(R,i,u,v,a)=1$. I.e.,
\begin{align*}
&\Pr_R[Z_1(R,i,u,v,a)] \\
&  = \Pr_R[ h_{R,i,u,v}(T_{u,v}^{(a)}(i)) = h_{R,i,v,u}(T_{v,u}^{(a)}(i))]  = p,
\end{align*}
where the last inequality uses the fact that $p$ is \emph{exactly} the collision probability of the inner product hash function we use (Lemma~\ref{lem:unifHash}).
If, on the other hand, $a_{i,u,v}=0$, then by a similar argument,
\begin{align*}
&\Pr_R[Z_1(R,i,u,v,a)] \\
&  = \Pr_R[ h_{R,i,u,v}(T_{u,v}^{(a)}(i)) \ne h_{R,i,u,v}(T_{v,u}^{(a)}(i))]  \\
& = 1- \Pr_R[ h_{R,i,u,v}(T_{u,v}^{(a)}(i)) = h_{R,i,u,v}(T_{v,u}^{(a)}(i))] \\
&= 1- p.
\end{align*}

Next let us assume that there was noise in the message $h_{R,i,u,v}(T_{u,v}^{(a)}(i))$. 
To be concrete, we will denote the additive noise by $x$.

If $a_{i,u,v}=1$, then, since $Z_1(R^*,i,u,v,a)=1$, 
we know that $o_1 = \widetilde{o_2} = o_2 + x$ (as vectors over GF(3)).
Then,
\begin{align*}
\Pr_R&[Z_1(R,i,u,v,a)]  \\
=& \Pr_R[  (h_{R,i,u,v}(T_{u,v}^{(a)}(i))= h_{R,i,u,v}(T_{v,u}^{(a)}(i)) +x].  \\
\intertext{Let us split into each index~$j$ and recall that each output bit of the hash is independent of the other output bits, since the parts of~$R$ that affect two different output bits are disjoint and thus independent.}
=&
\prod_{j: \, x_j=0}\Pr_R[  h_{R,i,u,v}(T_{u,v}^{(a)}(i))_j= h_{R,i,u,v}(T_{v,u}^{(a)}(i))_j] \times \\
&\prod_{j: \, x_j=1}\Pr_R[  h_{R,i,u,v}(T_{u,v}^{(a)}(i))_j=1 \wedge h_{R,i,u,v}(T_{v,u}^{(a)}(i))_j=0] \times\\
&\prod_{j: \, x_j=-1}\Pr_R[  h_{R,i,u,v}(T_{u,v}^{(a)}(i))_j=0 \wedge  h_{R,i,u,v}(T_{v,u}^{(a)}(i))_j=1]  \\
\ge&\, p^2\text{,}
\end{align*}
where the last transition is due to Lemma~\ref{lem:unifHash}.

If, on the other hand, $a_{i,u,v}=0$, then we can split into two cases. 
Let $E_{x}$ be the event that $\widetilde{h}_{R,i,u,v}(T_{v,u}^{(a)}(i))$ is not  not a binary string (i.e., it includes a silence).
Then, if $E_x$ occurs,
$\Pr_R[Z_1(R,i,u,v,a) \mid E_x] =1$, since $h_{R,i,u,v}(T_{u,v}^{(a)}(i))$ is a bitstring.
Otherwise, we can again write $h_{R,i,u,v}(T_{u,v}^{(a)}(i)) = h_{R,i,u,v}(T_{v,u}^{(a)}(i)) +x$ as an equation of vectors in~$GF(3)$, and
\begin{align*}
&\Pr_R[Z_1(R,i,u,v,a) \mid \overline{E_x}]  \\
&= \Pr_R[  h_{R,i,u,v}(T_{u,v}^{(a)}(i)) \ne \widetilde{h}_{R,i,u,v}(T_{v,u}^{(a)}(i))  \mid \overline{E_x}]  \\
& = 1- \Pr_R[  h_{R,i,u,v}(T_{u,v}^{(a)}(i)) = h_{R,i,u,v}(T_{v,u}^{(a)}(i)) +x  \mid \overline{E_x}] \\
 &= 1-\sum_y  \Pr_R\left[ 
 	\begin{multlined}
	 h_{R,i,u,v}(T_{u,v}^{(a)}(i)) = y  \\
	 \wedge h_{R,i,u,v}(T_{v,u}^{(a)}(i))  = y-x  
	  \end{multlined}
	  \ \middle \vert\  \overline{E_x}
	  \right] \\
&\ge 1 -\sum_y p^2 \\
&\ge 1-p\text{,}
\end{align*}
where the penultimate transition follows due to the strong 2-universality property of our inner product hash function (Lemma~\ref{lem:unifHash}). Note that $y$ should be restricted to binary strings (otherwise, the probability is 0), and that $y-x$ is over $GF(3)$, thus the inequality.


Hence, in all cases we have 
\(
\Pr_R[Z_1(R,i,u,v,a)]  \ge p^2.
\)
Similar arguments apply to $Z_2(R,i,u,v,a)$. Since both events are independent when the transcripts are different (they use  different seeds for the hashes, and the transcript is fixed by $a$ and the noise pattern), we get that for any appropriate $(i,v,u)$,
\[ 
\Pr_R[Z(R, i, u, v, a)] \geq p^4.
\]

Recall that the seeds $R_{i,u,v}$ are independent and uniform when $(u,v) \in E'$.
Since there are at most $\Err'$ triples $(i,u,v)$ in the main part such that an error occurs in $(i,u,v)$, we conclude that 
\[
\prod_{(u,v) \in E'} \Pr_{R_{u,v} \sim \Unif}\left[\bigwedge_{\text{$i$:err on $(i,u,v)$}}  Z(R, i, u, v, a) \right] \geq p^{4\Err'}.\]
\end{proof}
\begin{remark}[Remark on Fixing Adversaries]
In~\cite{GKR-1}, we proved that our scheme is resilient to both additive adversaries and \emph{fixing} adversaries. The latter type of adversary commits errors where it fixes the communication sent on a link in a given round. In the proof of Claim~\ref{clm:LB:ierr} we have assumed the adversary is additive; however, it can easily be verified that the claim also holds for fixing adversaries. The main idea is that, for any symbol $\widetilde{o_2}$ that the adversary puts on a link (which could also be silence), the probability that $h_{R,i,u,v}(T_{u,v}^{(a)}(i))= \widetilde{o_2}$ is exactly equal to $p$ if $\widetilde{o_2}$ is not silence, due to the uniform output distribution of the hash. If $\widetilde{o_2}$ \emph{is} silence, then the probability of agreement is 0, but this means that every consistent agreement pattern $a$ has $a_{i,u,v} = 0$, and the probability of this event over the hash randomness is 1. This is the only step of the proof which differs for fixing and additive adversaries.
\end{remark}


%
\begin{figure*}[!t]
\begin{equation}\label{eqn:large-eqn-1}
\begin{aligned}
 &\sum_{a \in \Bad_{\mathcal{D}_R}} \Pr_{S \sim \mathcal{D}_S}[A=a] \\
 &\leq e \cdot \sum_{a \in \Bad_{\mathcal{D}_R}} \prod_{(u,v) \in E'}\left(\Pr_{R_{u,v} \sim \Unif}\left[\bigwedge_{\text{$i$:no err on $(i,u,v)$}}  Z(R, i, u, v, a) \right]\right) \cdot Q(a) \\
&\overset{(1)}{\leq} e \cdot p^{-4\Err'} \cdot \sum_{a \in \Bad_{\mathcal{D}_R}} \prod_{(u,v) \in E'}\left(\Pr_{R_{u,v} \sim \Unif}\left[\bigwedge_{\text{$i$}}  Z(R, i, u, v, a) \right]\right) \cdot Q(a)
 \\
&\overset{(2)}{=} e \cdot p^{-4\Err'} \cdot \sum_{a \in \Bad_{\mathcal{D}_R}} \prod_{(u,v) \in E'}\left(\Pr_{R_{u,v} \sim \Unif}\left[\bigwedge_{\text{$i$}}  Z(R, i, u, v, a) \right]\right) \cdot \Pr_{S \sim \mathcal{D}_S}\left[\bigwedge_{i,(u,v) \in E \setminus E'} Z(S, i, u, v, a)\right] \\
&\overset{(3)}{=} e \cdot p^{-4\Err'} \cdot \sum_{a \in \Bad_{\mathcal{D}_R}} \prod_{(u,v) \in E'}\left(\Pr_{R_{u,v} \sim \Unif}\left[\bigwedge_{\text{$i$}}  Z(R, i, u, v, a) \right]\right) \cdot \Pr_{S \sim \mathcal{D}_R}\left[\bigwedge_{i,(u,v) \in E \setminus E'} Z(S, i, u, v, a)\right] \\
&\overset{(4)}{=} e \cdot p^{-4\Err'} \cdot  \sum_{a \in \Bad_{\mathcal{D}_R}} \Pr_{R \sim \mathcal{D}_R}[A=a]. 
\end{aligned}
\end{equation}
%
\hrulefill
%
\vspace*{4pt}
\end{figure*}
%




 Claim~\ref{clm:LB:ierr} along with Eq.~\eqref{eq:delta-bias-simplification-3} lead to 
 the derivation of Eq.~\eqref{eqn:large-eqn-1}.
%
%
%
%
%
%
%
%
Transition (1) is via  Claim~\ref{clm:LB:ierr}. 
Transition (2) is by the definition of~$Q$, Eq.~\eqref{eqn:q-def}. 
Transition (3) uses the fact that $\mathcal{D}_R$ and $\mathcal{D}_S$ are identical for $(u,v)\in E\setminus E'$. Transition (4) follows from Proposition~\ref{prop:key}.

Hence, we have proved the desired relation between $\sum_{a \in \Bad_{\mathcal{D}_R}} \Pr_{S \sim \mathcal{D}_S}[A=a]$ and between $\sum_{a \in \Bad_{\mathcal{D}_R}} \Pr_{R \sim \mathcal{D}_R}[A=a]$. %
We recall that this is equivalent to relating  
$\Pr_{S \sim \mathcal{D}_S}[D > k \cdot \Err']$ and $\Pr_{R \sim \mathcal{D}_R}[D > k \cdot \Err']$ by the same relation, which concludes the proof of Lemma~\ref{lem:bound-dangerous-obliv-no-crs}.
\end{proof}

We now show that even with arbitrary oblivious tampering of random strings on the edges $E \setminus E'$, the adversary cannot cause too many dangerous triples when the seeds $R_{u,v}$ are uniform for $(u,v) \in E'$. 
Let $X_{i,u,v}$ be an indicator random variable for the event that there is a hash collision between $u$ and $v$ in iteration $i$. Note that here we specifically mean a hash \emph{collision}, and not just any agreement: a hash collision occurs when the transcripts mismatch but the generated hashes match. 

Define $\psi_{u,v}$ as follows. 
\begin{algorithm}[H]
\caption{The process $\psi_{u,v}$}
\small
\begin{algorithmic}
\State $i \gets 1, \psi_{u,v}(1) \gets 0$
\ForAll{iterations $i$ from 1 to $100 |\Pi|$}
  \If {error occurs between $u$ and $v$\\ during iteration $i$, during any phase}
    \State $\psi_{u,v}(i+1) = \psi_{u,v}(i) + 6C_6$
  \ElsIf {$\psi_{u,v}(i) > 0$}
    \State $\psi_{u,v}(i+1) = \psi_{u,v}(i) + 6C_6 X_{i,u,v} - 5 (1 - X_{i,u,v})$
  \Else
    \State $\psi_{u,v}(i+1) = \psi_{u,v}(i)$
  \EndIf
\EndFor
\end{algorithmic}
\end{algorithm}
Let $\D$ denote the triples $(i,u,v)$ where $\psi_{u,v}(i) > 0$ and $(u,v) \in E'$. We proved in~\cite{GKR-1} that $\psi_{u,v} \geq \varphi_{u,v}$ for all iterations, which we recall now.
\begin{lemma}[Lemma 4.15 in~\cite{GKR-1}]
\label{lem:psi-lb-old}
For all iterations $i \in [100|\Pi|]$ and all edges $(u,v) \in E'$, we have that $\psi_{u,v}(i) \geq \varphi_{u,v}(i)$, where $\varphi_{u,v}(i)$ denotes the value of the potential $\varphi_{u,v}$ at the beginning of iteration $i$.
\end{lemma}
It follows from Lemma~\ref{lem:psi-lb-old} that $|\D| \geq D$. We provide a brief proof sketch that echoes the proof in~\cite{GKR-1}.
\begin{proof}[Proof sketch]
This follows from properties of $\varphi_{u,v}$, which are established in Lemma A.6 and Claim A.1 in~\cite{GKR-1}: $\varphi_{u,v}$ starts at 0, rises by at most $6C_6$ in any iteration, and falls by at least $5$ otherwise (we can take $C_6$ to be a multiple of 5 so there are no divisibility issues).

This establishes that, for iterations $i$ where $\psi_{u,v}(i) \geq \varphi_{u,v}(i) > 0$ at the start, $\psi_{u,v}(i+1) \geq \varphi_{u,v}(i+1)$. It still needs to be shown that $\psi_{u,v}(i+1) \geq \varphi_{u,v}(i+1)$ whenever $\psi_{u,v}(i) \geq \varphi_{u,v}(i) = 0$. This follows from \cref{prop:phi-nonnegative}, which states that the transcripts between $u$ and $v$ in iteration $i$ are consistent, so there cannot be a hash collision. So whenever $\varphi_{u,v}(i) = 0$, $\varphi_{u,v}(i+1)=0$ unless there is an error between $u$ and $v$ in iteration $i$. But in this case, $\varphi_{u,v}$ increases by at most $6C_6$, and $\psi_{u,v}$ will rise by $6C_6$, proving the lemma.
\end{proof}


We now proceed to upper bound $|\D|$ with high probability. Readers of~\cite{GKR-1} may notice that this is identical to what we do in Lemma~4.17 %
in~\cite{GKR-1}. Indeed, the only difference here 
is that we only consider the edges that are in $E'$, rather than all of $E$.
\begin{lemma}
\label{lem:bound-dangerous-obliv-2}
Suppose the adversary is oblivious, and let $\Err'$ be the number of errors committed during the main part. Let $p = 2^{-\Theta(\K / m)}$ be the hash collision probability of $h$, and assume that $p < \frac{1}{30C_6}$. Let $k$ be some real number such that $k \geq 10C_6$. Let $\D$ denote the set of triples $(i,u,v)$ such that $\psi_{u,v}(i) > 0$ and $(u,v) \in E'$. Then 
\[ 
\Pr_R[|\D| > k\cdot \Err' ] < p^{\Omega(k \cdot \Err') },
\]
where $R$ is defined as in Lemma~\ref{lem:bound-dangerous-obliv-no-crs}, and the $\Omega$ hides constants on the order of $1/C_6$.
\end{lemma}


\begin{proof}%
Consider an instance of the protocol after fixing the adversary's errors, and assuming uniformly random seeds for the hashes.
Assume $|\D|>k \cdot \Err'$ and let
$\wtD \subseteq \D$ denote the set of triples $(i,u,v)$ such that $\psi_{u,v}(i) > 0$ and $(u,v) \in E'$, and no error occurs between $u$ and $v$ in iteration $i$. Since the number of errors is $\Err'$, we get that $|\wtD| \geq (k - 1) \Err'$. Define 
\[
\psi \eqdef \sum_{(u,v) \in E'} \psi_{u,v}.
\]

We know that $\psi$ is always non-negative by design, since each of the $\psi_{u,v}$'s are non-negative. Consider $\psi(100 |\Pi|+1)$, that is, the value of $\psi$ immediately after the final $100 |\Pi|$-th iteration of \AlgCRS. 
%
Recall that $\psi_{u,v}$ goes up by $6C_6$ whenever there is an error or hash collision between $u$ and~$v$, and goes down by $5$ whenever there is no hash collision between $u$ and $v$ and $\psi_{u,v}$ was positive. This yields
\begin{multline}
\label{eq:d*-1}
 0 \leq  \psi(100 |\Pi| + 1) \leq \\
 6C_6 \cdot \Err' + \sum_{\mathclap{(i,u,v)\in \wtD}} (6C_6 X_{i,u,v} - 5(1-X_{i,u,v})),
\end{multline}


Rearranging, we note that 
\begin{align*} 
\sum_{(i,u,v) \in \wtD} X_{i,u,v} &\geq \frac{5|\wtD| - 6C_6 \cdot \Err'}{6C_6 + 5} \\
&\geq \frac{4}{6C_6 + 5} |\wtD|\text{,}
\end{align*}
where the last inequality follows from $|\wtD| \geq (k-1) \cdot \Err' \geq 6C_6 \cdot \Err'$.
So we can upper bound $\Pr_R[|\D| > k \Err']$ by upper bounding the probability that $\sum_{(i,u,v) \in \wtD} X_{i,u,v} \geq \frac{4}{6C_6 + 5} |\wtD|$.
Note that the events of hash collisions on the links $E'$ are independent, due to the fact that the adversary fixes their errors before the seeds are sampled.
Furthermore, they all happen with at most probability $p$. 
So, by a Chernoff bound, we get that 
\begin{multline}
\label{eq:chernoff}
\Pr\left[\frac{1}{|\wtD|}\sum_{(i,u,v) \in \wtD} X_{i,u,v} \geq \frac{4}{6C_6 + 5} \geq p + \frac{3}{6C_6+5}\right] \\
 \leq p^{\Omega(|\wtD|)} \leq p^{\Omega(k \cdot \Err')}
\end{multline}
For brevity we omit details on how to rigorously define random variables for which we can apply the Chernoff bound. For details on this, see the proof of Lemma~4.17 in~\cite{GKR-1}. The same proof applies verbatim here.
\end{proof}

\begin{corollary}[Corollary of Lemmas~\ref{lem:bound-dangerous-obliv-2} and \ref{lem:bound-dangerous-obliv-no-crs}]
\label{cor:bound-dangerous-obliv-no-crs}
Suppose $|\Pi|\K \geq m\log m$, and the adversary is oblivious and makes $\Err'$ errors in the main part. 
Let $k$ be a constant that is sufficiently larger than $\max\{ C_6, \frac{m}{\K }\log(p^{-1})\} $. 
Suppose that we run an instance of $\AlgCRS$ 
and denote the random string sampled by the protocol as~$S$. 
%
Then
\[ 
\Pr_S[D \geq k \cdot \Err'] \leq p^{\Omega(k \Err')} = \exp(-\Omega(k \cdot\Err' \cdot (\K / m))\text{.}
\]
\end{corollary}
\begin{proof}
We apply Lemma~\ref{lem:bound-dangerous-obliv-no-crs} and use the fact that $|\Pi|\K \geq m\log m$, we have that 
\begin{equation*}
\label{eq:cor-bound-dangerous-obliv-1}  
\Pr_S[D \geq k \cdot \Err'] \leq e \cdot p^{-4\Err'} \cdot  \Pr_R[D \geq k \cdot \Err'],
\end{equation*}
where $R$ is uniform for seeds on the edges in~$E'$. Recall that $|\D| \geq D$, and so applying Lemma~\ref{lem:bound-dangerous-obliv-2}
we get that
\begin{equation*}
\label{eq:cor-bound-dangerous-obliv-2}  
\Pr_S[D \geq k \cdot \Err'] \leq e \cdot p^{-4\Err'} \cdot p^{\Omega(k \Err')} = p^{\Omega(k \Err')}.\qedhere
\end{equation*}
\end{proof}





\subsubsection{Bounding the communication}
\label{sec:noCSR:comm-bound}

We continue to bound the communication in \AlgCRS. 
We start with an easy claim bounding the communication that occurs during the randomness exchange.
\begin{claim}
\label{claim:randomness-exchange-comm}
Assume that $|\Pi|\K \geq m\log m$. Then the communication in the randomness exchange (Algorithm~\ref{alg:randomness-exchange}) is $\Theta(\K |\Pi|)$. 
\end{claim}
\begin{proof}
Since $\delta = 2^{-\Theta(|\Pi|\K/m)}$ (Algorithm~\ref{alg:initialize-state-2}),
every link needs to exchange during this part a seed $L\in\{0,1\}^r$ of length
\begin{align*}
r &=  \Theta \left( \log(1/\delta) + \log \ell \right) \\
&= \Theta(|\Pi|\K/m)) +  \Theta(\log (|\Pi|^2 \K^2/m)) \\
& = \Theta\left (|\Pi| \frac{\K}{m}\right).
\end{align*}
where in the last line we use the fact that $\log(\K) = \Theta(\log m)$ for all settings of $\K$ that we use (either $m$ or $m\log m$), and that $|\Pi| \K / m \geq \log m$.


Each such seed is encoded via an error correcting code with a constant rate, hence, each such codeword takes $\Theta(|\Pi|\K/m))$ bits.
Since there are $m$ links in the network, the claim holds.
\end{proof}








Next we prove that the communication cannot get too high without a large number of errors. Note that some links have arbitrary, potentially disagreeing, random strings, and hence the corresponding parties might have hash-collisions in all iterations. 
While this can make the communication very large, our goal is to show that the communication cannot become \emph{too} large without having many dangerous triples (where again, dangerous triples only count on edges $(u,v) \in E'$). Once we establish this fact, we will bound the probability of having a large amount of dangerous triples.

Towards this end, we first recall that Lemma~\ref{lem:main-communication-old} connects the number of errors and hash collisions in a specific iteration to the potential increase and the communication that these errors and collisions might result in the same iteration. 

We now prove the connection between the large communication and large amount of dangerous rounds (assuming the noise level is within the allowed threshold).
In the following proofs, we denote the number of errors in the main part of the protocol as~$\Err'$, and the communication in this part as~$\CC'$, and let $D$ and $E'$ be the same as defined in Lemma~\ref{lem:bound-dangerous-obliv-no-crs}. 

\begin{lemma}
\label{lem:cc-bound-2}
Fix $\gamma \geq 2$ , and a sufficiently small $\eps'$. 
If $\CC' \geq 100 \gamma \alpha |\Pi| \K (1 + |E \setminus E'|)$ and $0< \Err' \leq \frac{\eps' \CC'}{\K}$, 
then
$$D \ge \beta \cdot \Err',$$ 
where $\beta \geq  \frac{1}{3\alpha \eps'}$ and $\alpha$ is the constant %
from Lemma~\ref{lem:main-communication-old}.
Further, if $\Err'>0$, then $\beta \ge \frac{33\gamma |\Pi| (1+ |E \setminus E'|)}{\Err'}$, and if $\Err'=0$ then $D=0$.
\end{lemma}
\begin{proof}


By Lemma~\ref{lem:main-communication-old}, we can bound
\begin{equation} 
\label{eqn:cc-bound-no-crs}
\CC' \leq \alpha\K(100|\Pi| + \EHC)\text{.}
\end{equation}
A ``hash collision'' (the HC in $\EHC$) occurs when two hashes that are passed on an edge match, but the transcripts do not match. Note that on any edge $(u,v) \in E \setminus E'$, the seeds may not have even been shared correctly! We bound the number of ``hash collisions'' on edges like this trivially, by $100|\Pi|$.  Note that if $u$ and $v$ have different seeds, their hash outputs may disagree even when their transcripts are the same. While this is problematic for simulating the protocol correctly, these sorts of ``fake'' hash misses do not increase the communication, since this stops parties from talking rather than making them talk too much (unlike hash collisions, which can make parties talk excessively, as seen in 
%
Lemma~4.8 in~\cite{GKR-1}).  %

Since $\Err' \leq \frac{\eps'}{\K} \cdot \CC'$ %
and noting that the number of hash collisions on links in $E'$ is upper bounded by the number of dangerous triples $D$, we can rewrite Eq.~\eqref{eqn:cc-bound-no-crs} as 
\begin{align} 
\CC' &\leq \alpha \K \left(100 |\Pi| + \frac{\CC' \cdot \eps'}{\K} + D + HC_{E \setminus E'}\right) \nonumber \\
&\leq  \alpha \K \left(100 |\Pi| + \frac{\CC' \cdot \eps'}{\K} + D + 100|\Pi|\cdot|E \setminus E'|\right) \text{.} \label{eqn:cc-bound-no-crs-expanded}
\end{align}
Rearranging and using the assumption that $\CC' \geq 100\gamma \alpha |\Pi| \K (1 + |E \setminus E'|)$ and $\gamma \geq 2$, and assuming sufficiently small $\eps'$ so that $\alpha\eps'<1/6$, we get that 
\begin{align*}
D &\geq \frac{(1 - \alpha \eps')\CC' - 100 |\Pi| \alpha \K (1 + |E \setminus E'|)}{\alpha \K} \\
&\geq \frac{(1 - \alpha \eps'  - \gamma^{-1})\CC'}{\alpha \K} \\
&\geq \frac{\CC'}{3\alpha\K}  \\
&\geq  \frac{1}{3\alpha \eps'}\Err' \text{.} \numberthis
\end{align*}
Thus, it holds that  $D\ge \beta \Err'$ for $\beta$ that is at least $1/3\alpha\eps'$. 

If $\Err'>0$, then from the  penultimate line and the fact that  
$\CC' \geq 100 \gamma \alpha |\Pi| \K (1+|E \setminus E'|)$ we also get that $\beta \ge \frac{33\gamma |\Pi| (1+ |E \setminus E'|)}{\Err'} $. 

Finally, note that if $\Err' = 0$, then there are no errors on the link in $E'$ in the main part of the protocol. Since the parties agree on seeds in $E'$, this means that every two parties are always in agreement and there will be no dangerous triples at all, $D=0$. 
%
 \end{proof}

Now we can prove our main communication bound of the section. 
\begin{lemma}
\label{lem:main-communication-no-crs}
Assume that $|\Pi| \K \geq m\log m$. 
Fix $\gamma \geq 2$, and a sufficiently small $\eps'$.
The probability that 
$\CC' \geq 100 \gamma \alpha |\Pi| \K (1 + |E \setminus E'|)$ and $\Err' \leq \frac{\eps'}{\K} \cdot \CC'$ is at most 
\[ 
p^{\Omega(\gamma |\Pi| \cdot (1 + |E \setminus E'|))},
\] 
where $\alpha$ is the constant multiplying the communication in Lemma \ref{lem:main-communication-old}. 
\end{lemma}
\begin{proof}
Suppose that $\CC' \geq 100 \gamma \alpha |\Pi| \K (1 + |E \setminus E'|)$ and $\Err' \leq \frac{\eps'}{\K}\cdot \CC'$. 

If $\Err'=0$ then Eq.~\eqref{eqn:cc-bound-no-crs-expanded} bounds $\CC'$ by 
$\alpha \K \left(100 |\Pi| + \Err' + D + 100|\Pi|\cdot|E \setminus E'|\right)$ and since $D=0$ by Lemma~\ref{lem:cc-bound-2} the statement holds.

Otherwise, by applying Lemma~\ref{lem:cc-bound-2}, we have that $D \geq \beta\cdot \Err'$ with 
 $\beta \geq \frac{1}{3\alpha \eps'}$. We can assume the constant $\eps'$ is small enough so that $\beta$ is large enough to apply
Corollary~\ref{cor:bound-dangerous-obliv-no-crs} to get that the probability of this is at most 
\(p^{\Omega(\beta \Err')}.\)
Since $\beta \geq \frac{33\gamma |\Pi| (1+ |E \setminus E'|)}{\Err'{\strut}}$, we conclude that the probability of this event is at most 
\(p^{\Omega(\gamma |\Pi| \cdot (1 + |E \setminus E'|))}.\)
\end{proof}


%

\subsubsection{Proof of Theorem~\ref{thm:oblivious-adv-no-crs}}
\label{sec:thm:oblivious-adv-no-crs:proof}
Recall that we have $\K = m$ in \AlgCRS,
%
and so we will set $\K = m$ throughout this proof. We split the proof into three steps. First, we show that the probability that $|E \setminus E'| \geq 1$ and $\Err \leq \frac{\eps}{m} \CC$ is at most $\exp(-\Omega(|\Pi|))$. Then, we set $E' = E$ and show that the probability that $\Err \leq \frac{\eps}{m} \CC$ and $\CC > \Theta(|\Pi| m)$ is also exponentially small. Finally, we show that the probability that $\Err \leq \frac{\eps}{m} \CC$, $\CC \leq \Theta(|\Pi| m)$, and $D \geq \omega(\eps |\Pi|)$ is also exponentially small. This covers the space of bad events for our protocol; outside of these events, it can be shown that the protocol is simulated correctly, by following the proof of Theorem 4.1 in~\cite{GKR-1}. 

Denote the number of errors in the main part of the protocol as~$\Err'$, and the communication in the main part as~$\CC'$. 

\begin{claim}
For a sufficiently small constant $\eps>0$,
\[
\Pr\left [\left( \Err \leq \frac{\eps}{m}\CC \right) \wedge (|E \setminus E'| \geq 1)\right ] < \exp(-\Omega(|\Pi|)).
\]
\end{claim}
\begin{proof}
Note that if $|E \setminus E'| \geq 1$, then the adversary must have committed $\Omega(|E \setminus E'| \cdot |\Pi|)$ errors in the randomness exchange phase. This holds since we encode each random strings with an error-correcting code with length $r=\Theta(|\Pi|)$ (Claim~\ref{claim:randomness-exchange-comm}) and constant distance. The code having constant distance means that in order to corrupt even a single codeword, the adversary must make at least $\Theta(|\Pi|)$ errors.
But since $\Err \leq \frac{\eps}{m}\CC$, such an attack is within the adversary's budget only if $\CC \geq \frac{m}{\eps}|\Pi|\cdot|E \setminus E'|$. 

Note that the communication in the randomness exchange phase is at most $\Theta(|\Pi| m)$, since there are $m$ links and strings of length $\Theta(|\Pi|)$ are sent on each. Hence, for a sufficiently small constant $\eps$, the amount of communication in the main part of the protocol must be at least
\[
\CC' \geq \Theta \left(\frac{m}{\eps}|\Pi|\cdot|E \setminus E'|\right) \geq 200 \alpha |\Pi| m (1 + |E \setminus E'|),
\]
where we use the assumption that $|E \setminus E'| \geq 1$ and $\alpha$ is the constant in Lemma~\ref{lem:main-communication-old}. 
 
 By Claim~\ref{claim:effective-noise}, the error in the main part satisfies 
  $\Err' \leq \frac{\eps'}{m} \CC'$  for $\eps' = \Theta(\eps)$.
%
So we can apply Lemma~\ref{lem:main-communication-no-crs} with $\gamma=2$ and allowed noise rate (for the main part) of~$\eps' / m$, and get that the probability that $\CC' \geq 200 \alpha |\Pi| m (1 + |E \setminus E'|)$ is at most $\exp(-\Omega(|\Pi| \cdot (1 + |E \setminus E'|))) \leq \exp(-\Omega(|\Pi|))$, as stated.
\end{proof}

Given the above claim, we know that the adversary cannot corrupt even a single seed and keep its attack within the allowed budget. Hence, we can assume from this point on that~$E' = E$, and that all the seeds are $\delta$-biased strings chosen by the parties.
%
Under these conditions, Lemma~\ref{lem:main-communication-no-crs} gives us that   
\begin{multline*}
\Pr \left [(\CC' \geq 200 \alpha |\Pi| m)  \wedge \left(\Err' \leq \frac{\eps'}{m} \CC' \right) \right ] \\
< \exp(-\Omega(|\Pi|)).
\end{multline*}


Now further suppose that the communication in the main part satisfies $\CC' \leq 200 \alpha |\Pi| m$ and that $\Err' \leq \frac{\eps'}{m}\CC'$. This implies that the number of errors the adversary commits is at most $200 \alpha \eps' |\Pi|$. Combining this with Corollary~\ref{cor:bound-dangerous-obliv-no-crs}, we see that the probability that the adversary can cause the number of dangerous triples exceed $k \eps' |\Pi|$ in this case is at most $\exp(-\Omega(k \eps' |\Pi|))$, even when the parties share $\delta$-biased randomness, where  $k \geq 10C_6$. Hence,
\begin{corollary}
\label{cor:remove-crs-ehc}
For a real number $k$ such that $k \geq 10C_6$, we have that  
\[
\Pr[ \EHC > (k+1)(200 \alpha \eps') |\Pi|] < \exp(-\Omega(k \eps' |\Pi|)).
\]
\end{corollary}

To conclude, if we limit the adversary to make at most $\Err \leq \frac{\eps}{m} \CC$ corruptions,
then
the probability that the adversary is able to tamper with any of the of the randomness exchanges, cause more than $\Theta(|\Pi|m)$ communication throughout the protocol, or cause the number of errors and hash collisions to exceed~$\Theta(k \eps' |\Pi|)$, is at most $\exp(-\Omega(k \eps' |\Pi|))$, where we have freedom to set $k$ to be as large as we would like.
 
Regardless of the seed being used, 
Lemma~\ref{lem:main-communication-old} shows that  \AlgCRS concludes with $\phi \geq 100 |\Pi| m$. 
Then, as long as none of the above bad events happen, 
we can take $\eps$ (and therefore also~$\eps'$) to be sufficiently small, which (by applying Corollary~\ref{cor:remove-crs-ehc} with appropriately selected $k$) makes $\EHC$ at most $|\Pi| / C_7$ with probability at least $1 - \exp(|\Pi|)$. Finally, we appeal to Claim~\ref{claim:final-claim}, a reformulation of Claim~4.19 from~\cite{GKR-1}, %
to conclude that \AlgCRS correctly simulates~$\Pi$.
\begin{claim}[\cite{GKR-1}]
\label{claim:final-claim}
Suppose that $\phi$ is defined as in Eq.~\eqref{eqn:potential}, that $\phi \geq 100|\Pi| \K$, and that
$\EHC \leq \eps^* |\Pi|$ for a sufficiently small constant $\eps^* > 0$ that does \emph{not} go to~$0$ as $\eps$ goes to~$0$.
Then the underlying protocol $\Pi$ has been simulated correctly.
\end{claim}
To conclude the proof, we note that $\EHC$ is bounded by $\eps^* |\Pi|$ with probability $1 - \exp(-\Omega(|\Pi|))$ for \AlgCRS 
follows from Corollary~\ref{cor:remove-crs-ehc} by taking $\eps'$ to be sufficiently small with respect to $\eps^*$, where the 
$\Omega$ hides a factor of the constant $\eps^*$ (but not $\eps$ or $\eps'$). 
For more details, see the proof of 
%
Theorem~4.1 in~\cite{GKR-1};
the proof follows identically in this case.
%



